Pisces: Private and Compliable Cryptocurrency Exchange

Cryptocurrency exchange platforms such as Coinbase, Binance, enable users to purchase and sell cryptocurrencies conveniently just like trading stocks/commodities. However, because of the nature of blockchain, when a user withdraws coins (i.e., transfers coins to an external on-chain account), all future transactions can be learned by the platform. This is in sharp contrast to conventional stock exchange where all external activities of users are always hidden from the platform. Since the platform knows highly sensitive user private information such as passport number, bank information etc, linking all (on-chain) transactions raises a serious privacy concern about the potential disastrous data breach in those cryptocurrency exchange platforms. In this paper, we propose a cryptocurrency exchange that restores user anonymity for the first time. To our surprise, the seemingly well-studied privacy/anonymity problem has several new challenges in this setting. Since the public blockchain and internal transaction activities naturally provide many non-trivial leakages to the platform, internal privacy is not only useful in the usual sense but also becomes necessary for regaining the basic anonymity of user transactions. We also ensure that the user cannot double spend, and the user has to properly report accumulated profit for tax purposes, even in the private setting. We give a careful modeling and efficient construction of the system that achieves constant computation and communication overhead (with only simple cryptographic tools and rigorous security analysis); we also implement our system and evaluate its practical performance.

==> 1intro.tex <==

\section{Introduction}

Just like stocks and other commodities, people buy or sell cryptocurrencies on exchange platforms, mostly, on centralized platforms such as Coinbase, which are essentially marketplaces for cryptocurrencies. There, customers can pay fiat money like U.S dollars to get some coin, e.g, Bitcoin, or transfer their coin in the platform to an external account ({\em withdrawal}) \footnote{Or transfer coins into accounts in the platform from an external account ({\em deposit}), then sell for fiat money; and {\em exchange} one coin, e.g., BTC, to get some other coin, e.g., ETH. See Fig.\ref{overview}, and Sec.\ref{syntax} for details.}. 
%
Despite the promise of decentralized exchange, those centralized trading platforms still play a major role for usability and even regulatory reasons. For example, the annual trading volume of Binance was up to 9580 billion USD in 2021~\cite{BinanceStatistics}, and Coinbase also had 1640 billion USD in 2021 \cite{CoinbaseStatistics}. 

Like conventional stock exchanges, these exchange platforms must comply with regulations including Know Your Customer (KYC). They require businesses to verify the identity of their clients. Essentially, when a client/user registers an account at the exchange platform, he is normally required to provide a real-world identification document, such as passport, or a stamped envelope with address, for the platform to verify. Also for trading purposes, bank information is also given. 

%The client (called user) has an account maintaining all kinds of cryptocurrencies it owns and the exchange platform (called platform) holds them in escrow. 
%Each user has an account containing all kinds of cryptocurrencies he owns and the platform holds them in escrow. 

%In the exchange platform supporting multiple cryptocurrencies, the users buy, sell, withdraw or exchange cryptocurrencies and the platform modifies the balance state of their accounts according to their requests. 
%Especially, on the withdraw request, the platform generates on-chain transaction that sends cryptocurrency to the user's designated electronic address on the blockchain.



%who are in compliance with the KYC, AML requirements and tax rules. 
%When users buying, selling, exchanging or withdrawing cryptocurrencies, the platform knows their identities. 
%Especially, when they require the platform to send cryptocurrency to their electronic wallets, the wallet addresses are linked to their identities. 
%It would violate user's privacy of future transactions.
%When the user registers himself, he shows the real-world identity, like E-mail address, phone number, passport, etc, abiding KYC and AML.




\iffalse
\paragraph{\bf{Bank transfer}}
In the real world, users transfer money with real name bank accounts under the supervision.
It is the legal requirement to prevent money laundry or financial crimes.
People withdraw cash from bank. 
Cash is widely acceptable and offline cash transactions cannot be traced. 
So users need not worrying the privacy violation.
However, things become different when it comes to the payments on the public blockchain where the transactions are transparent for everyone.
%Once they can be linked to user's identity, even the pseudonyms anonymity cannot be guaranteed.
\fi

\iffalse
\paragraph{\bf{Blockchain payment}}
%\noindent\textbf{Pseudonym anonymity}
For the payments in the public blockchain, anyone can link sender and receiver as well as trace back the origin of coins.
%, breaking the unlinkability and untraceability properties.
%One of the features of Bitcoin 
This feature is called pseudonym anonymity:
users are not required to provide real identities but use pseudonyms. 
So it is explicitly seen that some entities transact with each other, but no one can link those on-chain payments with the real identities. 
%The transactions are recorded and made public, but they are linked only with electronic addresses instead of real-world identities.
For example, Bitcoin is the most widely known distributed, peer-to-peer payment network.
When people pay with their Bitcoins, the purchase behavior cannot be traced specifically to them.%\\
%Generally speaking, the aim of anonymization is to prevent attackers from discovering the relationship between bitcoin wallet addresses and the real user identity information through the Bitcoin network and the blockchain.
\fi



\ignore{%%%%%%%%%%%%%
 


\noindent\textbf{Exchange platforms}  
%\paragraph{\bf{Cryptocurrency exchange platforms}}
%\paragraph{\bf{Exchange platforms}}
Mining Bitcoin is a heavy work.
Most users prefer to buy Bitcoins with fiat money 
%They may interact with individual miner, but the fairness is not guaranteed.  So more and more users choose purchase 
from Coinbase or other centralized cryptocurrency exchange platforms.


Firstly, the user registers and creates an account in the platform. 
When the user registers himself, he shows the real-world identity, like E-mail address, phone number, passport, etc, abiding KYC and AML.
With an account in the exchange platform, the user conducts the following operations: %\\
\iffalse
\textbullet\ Deposit: The user deposits assets into the exchange platform. They can be fiat money or cryptocurrencies. The platform credits the respective assets in his account.\\
\textbullet\ Exchange: The user exchanges one kind of asset to another one. For example, exchanging fiat money to cryptocurrency can be seemed as buying and the opposite direction is selling. \\
\textbullet\ Withdraw: The user withdraws assets and lets the platform sends them to his bank account or wallet address in blockchain. \\
\textbullet\ Request: The user requests the platform to sign his annual profit for reporting tax to some authority like IRS.
\fi
%\iffalse
\setlist{nolistsep}
\begin{itemize}[noitemsep,leftmargin=*]
	\item Deposit: The user deposits assets into the exchange platform. They can be fiat money or cryptocurrencies. The platform credits the respective assets in his account.
	\item Exchange: The user exchanges one kind of asset to another one. For example, exchanging fiat money to cryptocurrency can be seemed as buying and the opposite direction is selling.
	\item Withdraw: The user withdraws assets and lets the platform sends them to his bank account or wallet address in blockchain.
	\item Request: The user requests the platform to sign his annual profit for reporting tax to some authority like IRS.
\end{itemize}
%\fi
}%%%%%%%%%%%%%%




\iffalse
\begin{itemize}
	\item Buy: The user transfers fiat money to the exchange platform from his bank account. The platform credits the cryptocurrency in its platform account.
	\item Sell: The user sells its cryptocurrency to the platform and gets fiat money to its bank account.
	\item Exchange: The user exchanges one kind of cryptocurrency to another one.
	\item Withdraw: The user withdraws cryptocurrencies and lets the platform sends them to his electronic wallet.
	\item Request: The user requests the platform to sign the number of its annual profit for reporting tax to some authority like IRS.
\end{itemize}
\fi
%When client spends bitcoins, he obtains income corresponding to the bitcoin price at that time, and he should pay tax on this kind of income yearly.
	

\iffalse
\paragraph{\bf{Privacy in exchange platform}}
The exchange platform can be seemed as the bridge between the real world and the cryptocurrency world.
It knows both the identities of its users in the real world and the cryptocurrency addresses of its receivers on the blockchain.
When the user buys and withdraws cryptocurrency, the exchange platform generates a transaction on the blockchain and the user plays the role of receiver.
So the exchange platform can link user with its cryptocurrency addresses easily and even all future transactions made from these address. 
It means the platform knows users' future on-chain spending behaviors which is a severe destruction of their privacy.

To handle with this issue, the intuitive idea is hiding user's identity or the address during withdrawing so that the platform cannot link them. 

%When users pay for the cryptocurrency, their payment methods reveal their identities, so they should not get the cryptocurrency immediately. 
%Here we treat the number of the cryptocurrency as an attribute of user's account, denoted by $v$. 
%It gets credited when user purchases some cryptocurrency and it gets deducted if user spends some of them.



\paragraph{\bf{Accountability in exchange platform}}
There are many kinds of assets in the exchange platform. Their
prices fluctuate over time. 
Users exchange them and make a profit from the difference between the buying and selling prices.  
They should declare such profit when filing taxes.
Based on the suggested tax policy of Coinbase, transactions that result in a tax are called taxable events.
Taxable events as capital gains include selling cryptocurrency for cash, converting one cryptocurrency to another and spending cryptocurrency on goods and services (withdrawing cryptocurrency). 
(``taxable events happen when you realize losses or gains, meaning you've sold your cryptocurrency by either selling for cash, converting to another cryptocurrency, or spending it on a good or service. 
The gains are unrealized if you still own the original shares." )

Privacy is a double-edged sword.  
Such private exchange system preserves user's privacy, which may also protect their illegal behaviors from being detected, such as money laundering or tax evasion.
Some malicious user may claim it did not make any profit. 
In case of the private exchange platform where users' operations are unlinkable, it is not easy to check whether it is cheating.
Therefore, we should pay attention on the accountability of users even in the private exchange system to make sure they behave legally.
Such accountability needs to be treated carefully to avoid affecting honest user's privacy.
\fi
%Here the \textbf{accountability} does not mean restricting users' behaviors such as limiting transaction amount or transaction frequency, since it also disables their legal and normal operations.  (...), They are just required to provide compliance information periodically or as dispute solution.

\iffalse
\paragraph{\bf{Periodical report}} 
The user needs to provide some compliance information periodically, for example, the annual profit as his tax basis. The compliance information can be seemed as an attribute of user's account and it is updated during each operation. 
But it should not be a link among honest user's operations which violates privacy. 

 

\noindent\textbf{Our solution}
In the exchange platform, there are many kinds of assets.
Their prices fluctuate over time.
Users exchange them and make a profit which is the difference between the buying and selling prices. (bid and offer prices)

Every user has an account in this platform.
It contains all values of the assets that he owns and his compliance information.  
They are recorded in a token issued by the platform and users obtains their tokens  when they join. 
(The platform knows its every customer due to the KYC requirement.)
Each time when the user obtains some amount of one asset through deposit or exchange, it gets a record for that new added asset which contains its metadata, such as the type, the value, the buying price, etc.
When the user spends some asset via exchange or withdraw, the value of record gets deducted and the compliance information is updated.


\noindent\textbf{Buy and sell} 
When users pay for the cryptocurrency with fiat money, the payment method, like bank account, naturally leaks user's account, so we introduce an attribute in the token denoting the fiat money and split the buying operation into two steps: first deposit fiat money into his platform account, then exchange fiat money to cryptocurrency. 
Selling is operated in a reverse direction that exchanging cryptocurrency to fiat money then withdrawing to the bank account.
Therefore, the buying and selling can be represented by depositing, exchanging and withdrawing. 


\noindent\textbf{Compliance information}
The compliance information is recorded in the token and it is computed from some compliance function. 
The function is public and it takes the latest compliance information and current operation as inputs.  
Let $\bf{cp}$ denotes the user's current compliance information, then for each successful operation it is updated to $f(\mathsf{operation}, \textbf{cp}, k)$ where $\mathsf{operation}\in\{\mathsf{exchange},\mathsf{withdraw},\mathsf{request}\}$.
Except the request operation, the compliance information is unlinkable to any user. 
In each operation, the user computes his new compliance information $f(\mathsf{operation}, \textbf{cp}, k)$ and proves the correctness. 
Once the exchange is convinced, it issues the new token with the updated value and compliance information. 
In the later construction, we use annual cumulative profit as the compliance information.
Users report it in tax file every year. 

Based on the suggested tax policy of Coinbase, transactions that result in a tax are called taxable events.
Taxable events as capital gains include selling crypto for cash, converting one crypto to another and spending crypto on goods and services (withdrawing crypto). 

``taxable events happen when you realize losses or gains, meaning you've sold your crypto by either selling for cash, converting to another crypto, or spending it on a good or service. 
The gains are unrealized if you still own the original shares." 
\fi

%%%%%%%%%%%%%%%%%%%%%%%



%\tian{just note: privacy in the exchange is special, even the basic anonymity without compliance rules out many other primitives like payment, payment channel hub, give a basic construction, then show it can be enhanced from the following three aspects: full anonymity (exchange privacy has independent interest), comply with the regulation (tax filing, AML, etc), efficiency especially for private exchange; then the overview is corresponding to these points }

%\tian{introduce our initial attempt: cut the link between the user's identity with his address, existing constructions are not enough}

 
\noindent{\bf Serious privacy threats.} Despite provided convenience, those centralized cryptocurrency exchange platforms cause a much more serious concern on potential privacy breaches. 

As we have witnessed, many data breach instances exist \cite{DataBreaches}. A more worrisome issue in the exchange setting is that exchange can be seen as a bridge between the real world and the cryptocurrency world, which amplify the impacts of potential privacy breach (in exchange, of user records including identities and accounts). Users may {\em deposit} coins into the platform from,  or {\em withdraw} coins (transfer out of the platform) to,  his personal account on a blockchain. %\yanan{a brief introduction of exchange mechanism to understand why the platform could learn link identity and on-chain address:} 

%Note that all the coins within the centralized exchange are actually hosted by the platform, who is the real payee and payer of the on-chain transaction in {\em deposit} and {\em withdrawal}, respectively.

Since most of the blockchains are transparent (except very few number of chains such as Zcash \cite{zcash}) and publicly accessible (e.g., Bitcoin, Ethereum), the platform can essentially extract all transaction history knowing the real identity of a user. In the former case, the platform immediately links the real identity to his incoming addresses, and trace back all previous transactions on-chain; while even worse in the latter case, the platform, knowing the real identity of a user, and knows exactly which account/address of the cryptocurrency the user requested to withdraw (transfer to), and all future transactions. For instance, the platform could easily deduce that a user Alice bought a Tesla car with Bitcoin, as she withdrew them from the platform and then transferred them to Tesla's Bitcoin account (which could be public knowledge). 

%In this way, the centralized platform immediately ``destroyes'' the pseudonymous property of blockchain
  

\ignore{%%%%%%
It sells cryptocurrencies to users and holds their assets in escrow. 
Note that the user's account in the platform binds to his real identity due to the requirement of KYC and AML. 
The platform also knows their cryptocurrency addresses on the blockchain when they request to withdraw cryptocurrencies to the designated wallet addresses. 




the platform knows users' future spending behaviors and destruct their privacy.
The blockchain just shows that ``somebody'' pays Tesla with the amount of Bitcoins, but Coinbase knows exactly that the payer is Alice.
}%%%%%%

It follows that existing centralized cryptocurrency exchange immediately ``destroys'' the pseudonym protection of blockchains, and the platform could obtain a large amount of information that is not supposed to be learned, e.g., the purchase/transaction histories of clients {\em outside of} the platform. This is even worse than conventional stock/commodity exchange where privacy may be breached within the system, but user information outside of the system is not revealed. 

%\subsection{Anonymity and privacy in cryptocurrency exchange}
%\noindent{\bf \em Identifying a unique problem about privacy in exchange.} 
We would like to design a cryptocurrency exchange system that at least restores user anonymity/privacy so that external records are not directly linked to the real identity. 
%In this section, we will break down the design goal step by step to demonstrate the necessity of a systematic study

%In the following, we break down the design goal step by step, and demonstrate it deserves further study as using existing solutions directly for private payment or adaptively for reconstructing the exchange system is not satisfying in terms of anonymity and other usability issues.



%Interestingly, as we will discuss very soon, it becomes essentially necessary that we need the privacy preserving property also {\em within} the platform. 


%%%%%%%%%%%
%\tian{Our goal (no compliance now): Exchange to all kinds of assets; Variable amount in exchange and withdraw; Proper anonymity.}
%%%%%%%%%%%%%%
%\tian{Limitation of existing anonymous constructions: One asset: E-cash, Monero, Zcash, Zether; Fix value: A2L, LDSP; Limited anonymity: A2L, BlindHub}


 
\noindent{\bf Insufficiency of external anonymity mechanisms.} 
%One basic idea is to cut the link between transactions within the exchange system (which links to real user identity) and external records. Since only the withdrawal operation (an onchain-payment from platform to an external address) is directly related to external records,  one may propose to focus on withdrawal to explore how to cut the link. 
%We know that a withdrawal operation consists of an on-chain payment (exactly a payment via blockchain) from the platform to the user and a within-exchange payment from the real identity user to the platform. %If the blockchain e.g., Echash and Monero is anonymous, 
The first potential method is keeping the existing exchange unchanged, and cutting the link between the exchange and external blockchain by
making on-chain payments/transfers (for coin deposits and withdrawals) on every blockchain anonymous, 
%The ideal case is that each on-chain payment is anonymous; 
%say the main task is to design an on-chain payment system 
so that nobody %(including the exchange platform)
can link the payer and the payee. Unfortunately, all those external anonymity solutions are insufficient.

First, fully anonymous on-chain payments such as Zcash only support its own native coins, while in most exchange platforms, Bitcoin, Ethereum and many other crypto tokens are the main objects of exchange, and cannot be supported. 

%To the platform cannot get the link between the user's real identity and the receiving account. In reality, it is challenging. 
%Concretely, on the one hand, existing blockchains achieve different degrees of anonymity. For example, most blockchains such as Bitcoin and Ethereum only provide pseudonym anonymity, while Zcash provides pseudonym anonymity and hides the payment sender, receiver, and amount.  So it is complicated for the exchange platform supporting all kinds of cryptocurrencies to enable consistent anonymous withdrawal no matter what cryptocurrency is withdrawn. Especially when the withdrawn cryptocurrency is only pseudonym anonymous, 

More exotic solutions like anonymous layer-2 payment solutions ~\cite{heilman_tumblebit_2017, glaeser2022foundations, qin2022blindhub, ng_ldsp_2021} and private smart contract enabled private payment solutions~\cite{bunz2020zether,diamond2021manyzether} also exist. 
One may wonder whether we can let the platform be the payer in those solutions during coin withdrawal. 
%\footnote{One naive attempt is withdrawing coins from the exchange and using the above private payment solutions for later on-chain payments. But such plain withdrawal already leaks information to relate the withdrawal on-chain address and user identity.}
%[A2L,BitTumbler,Blindhub]. 
%
%On the other hand, even the platform uses customized payment solutions for each kind of cryptocurrency, the existing anonymous payment solutions are not good enough, as they provide weak anonymity or introduce costs to hurt usability. 
%
%The private layer-2 solutions~\cite{heilman_tumblebit_2017, glaeser2022foundations, qin2022blindhub, ng_ldsp_2021} 
%
However, existing solutions mainly consider $k$-anonymity (where $k$ is the number of active users in an epoch) against the hub in~\cite{heilman_tumblebit_2017, glaeser2022foundations, qin2022blindhub} and the leader in~\cite{ng_ldsp_2021} and other outsiders, {\em not against the payer himself}. In our case, the platform is the payer and knows exactly the payee address during a coin withdrawal. 
%%\yanan{supply analyzing the attempt proposed by reviewers: withdraw in a plain way and do  private on-chain payments}

Recent works of \cite{tairia2l2021,glaeser2022foundations} even considered anonymous ($k$-anonymity) payment hub against payers, assuming fixed denomination. Besides that $k$ is usually small, the withdraw transactions in exchange platform can hardly be of a fixed amount. When two users withdraw different amount of coins, the platform again can trivially tell them apart.



%total amount of hub/leader customers. 
%The unlinkability to payees against payers is more challenging as payers know the exact transaction amount which could be quite different from others, and the case is worse if payees only have one transaction. Then the anonymity set only includes payees with same amount of withdrawal, which could be much less than $k$. %[A2L,BitTumbler]


%Some works \cite{heilman_tumblebit_2017, glaeser2022foundations, ng_ldsp_2021} require the fixed denomination which is an anonymity and usability trade-off. If the denomination is too small to be composed of any total amount, the anonymity is still restricted to a small number of payees transacting the same special total amount of coins. If the denomination is large, then it hurts the usability as many small amounts of withdrawal are not supported. The smart contract enabled private payment solutions \cite{bunz2020zether,diamond2021manyzether} provide privacy against outsiders except payers and payees. But the platform as the payer knows exactly the payees' addresses. Besides, they rely much on the smart contract which requires the underlying blockchain like Ethereum supports running Turing-complete scripts, and are not suitable for many blockchains.%Concretely, we take Bitcoin as an example and the anonymous payment hub has $k$ customers. Users withdraw Bitcoin via the anonymous payment hub where payers are unlinkable to payees among k users for each insider and outsider even including the payer and payee. Since the platform knows the exact withdrawn amount, when payees purely finish the withdrawal operation and close the channel, the special amount for each payee. Ideally, the user could be anyone of $k$ customers except the platform. Assuming users only conduct the withdrawal transaction and then close the payment channel after successful withdrawal, then the balance variants are equivalent to the withdrawal amount, which is known to the platform and could reduce the anonymity set depending on the amount. In [A2L, BitTumbler], 

 
\noindent{\bf Unexplored anonymity within exchange platform.} The above analysis hints that relying on external anonymity mechanism alone is insufficient, we need to further strengthen the anonymity protection {\em within} the platform. Anonymity issues are classical topics that have been extensively studied in different settings, including in cryptocurrencies; yet, we will demonstrate that large body of those works are not applicable to our setting of exchange system.

%briefly recall the related works, try to adapt their design framework for the exchange system, and analyze the corresponding drawbacks.

%The other method is to reconstruct the existing plain exchange mechanism to enable anonymous withdrawal. 


%Privacy/anonymity are classical topics that have been studied for a long time.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%. Privacy preserving centralized exchange platform is desired. However, privacy is intuitively contradictory with compliance, which makes private yet accountable centralized exchange platform more tricky.

%\noindent{\bf Privacy} \

%So the exchange platform can link user with its cryptocurrency addresses easily and even all future transactions made from these address. 


\iffalse
Besides, we observe that the platform always knows the names and amounts of cryptocurrencies the user withdraws. 
This information can be used for narrowing down the anonymity set of users.
Someone handles this issue by simply setting fixed nominations for the withdrawn asset. 
For example, restricting that every user can only withdraw 1 BTC each time which is inconvenient. 
We are more interested in how to live with the leakage and achieve the best anonymity level without applying the above restriction.
\fi

\iffalse
In the real world, users transfer money with real name bank accounts under the supervision.
It is the legal requirement to prevent money laundry or financial crimes.
People can also withdraw cash from bank. 
Cash is widely acceptable and offline cash transactions would not be traced. 
So users need not worrying the privacy violation.
However, the transactions on the public blockchain are transparent for everyone.
Once they can be linked to user's identity, even the pseudonyms anonymity cannot be guaranteed.
At first, the platform holds users' assets in escrow.
When the user withdraws bitcoins, the platform links his account with the bitcoin address, 
so even the pseudonyms anonymity cannot be guaranteed.
\fi 

\iffalse
Considering a scenario where a cryptocurrency exchange platform, like Coinbase, sells cryptocurrencies to its clients and holds users' assets in escrow. 
The client's account in the platform binds to his real identity.
When he requests the platform to send cryptocurrencies to his own electronic wallet, it is able to link the account with the address which violates user's privacy in the cryptocurrency world.
%If a client pays to the provider for the bitcoin online, e.g., through bank transfer, credit card, PayPal, the provider is able to link the client's payment information to the address of the transacted bitcoin, where the payment information is associated with the client's real identity.
Besides, the \textit{inside privacy} is also important for users.
We observe that the platform always knows the names and amounts of cryptocurrencies the user withdraws, 
if it knows the names and amounts of cryptocurrencies the user owns or exchanges, 
this information can be used for narrowing down the anonymity set of users. 
%via the withdrawn asset itself. 
Someone solve this issue by simply setting fixed nomination for withdrawn asset.
For example, restricting that every user can withdraw 1 BTC each time.
However, it is inconvenient for the users.
We are interested in that to which privacy level can be reached at best without applying the above restriction.
\fi
	





%: Private yet compliable with leakage}
%Each user has an account in the exchange platform, and the company knows their real world identities due to the KYC policy.
%Users can buy, sell, exchange in the platform and more important, withdraw cryptocurrency to their wallet addresses. 



%or even money laundering 
%Some of them could claim they did not make any profit. 


%, 

%
%We aim for the following goal in this paper:
%, and it is unlinkable with any other transaction.
%functionality: partial withdrawal, pay tax on yearly income
%\vspace{-2mm}	

%\begin{center}
%	{\em To protect users' privacy {\em  outside the platform}, i.e., breaking the link once the coin is moved out, while at the same time, to ensure the platform could still fulfill its duties on KYC or other compliance requirement.}
%\end{center}

% 	
\ignore{%%%%%%%
\noindent{\bf Who and how obtain the compliance related info.} 
Users are required to reveal their correct compliance information to some authority periodically, like reporting tax to IRS. 
Otherwise, they would be detected and punished. 
Such report needs the authentication of the platform to make sure the compliance information is correct. 
%To make sure the correctness, the user needs the authentication of platform on that information. The platform also helps the authority to identify who does not request to prevent tax evasion.		
%When requesting authentication, the user must convince the platform that the information is true, otherwise the platform refuses it.
Furthermore, the user must request authentication periodically, otherwise he would be identified and cannot exchange or withdraw later, which means his assets would be frozen in the platform. 
%In another word, in the view of the platform, users' pseudonym in the bitcoin world should be independent with their real identities.
}%%%%%%%

% 	
%\noindent{\bf Compliance requirements} \ 


%But when it is outside the platform, it would be desirable that for a withdraw transaction, the exchange cannot link it with any account.
%Hence, in the view of the exchange, users' pseudonym in the bitcoin world is independent with their real identities.

%\noindent\textbf{Warm up} 	
\iffalse
\tian{do we need the rough idea as warm up?}

To protect user's privacy, a rough idea is introducing a third party as an intermediary who sends cryptocurrency to users directly.
Users interact with the platform for buying or exchanging cryptocurrencies with their accounts.
When they withdraw cryptocurrencies from the platform, the cryptocurrencies are sent to a third party.
Then the intermediary forwards cryptocurrencies to users' wallet addresses.
Here the difficulty is that users need to hide the wallet addresses and cryptocurrency values from the platform but show them to the intermediary. 
Besides, there is an inherent issue of this method.
The third party must be independent with the platform, which means we need additional assumption on the third party. 
Otherwise, they can collude and link users with their wallet addresses trivially.
%Secondly, users' transactions inside the platform (buying, selling and exchanging) are public for the platform.

Can we protect user's privacy using a better method? 
In other words, making all kinds of users' operations unlinkable without introducing any new party or additional assumption.
\fi



%Therefore, we should pay attention on the compliance of users even in the private exchange system to make sure they behave legally. 

%\tian{highlight the unique setting and challenges: model, compliance (conceptually different with other setting) and construction (efficient design is non-trivial, existing schemes cannot imply)} 

%\tian{why not UC model? inefficient construction} 



%\medskip
%\noindent\textbf{Challenges.} 

\iffalse
\yanan{- Private payment solutions only target on a single blockchain. So in the exchange marketplace, all kinds of cryptocurrencies based on different blockchains are supposed to be considered and analyzed separately to check how to leverage private payment solutions to enable the private platform, which is costly work: Firstly, only limited kinds of cryptocurrencies are private, which can be used directly, e.g., Zcash, Monero. Secondly, there are several works[14][23] on enabling anonymous payment but the achieved anonymity and privacy are restricted. Detailed the privacy drawback. Thirdly, some layer-2 payment solutions also achieve privacy, but the restriction is that the transaction amount is limited to single unit, which is inconvenient and even has the probability bias for owner of the extreme large amount of asset. What is CBDC????  

- For Atomic swap, seems no private solution for the transacting two parties? need further check. 
%- DEX. It has different goals from private exchange marketplace. DEX focuses on the content privacy but does not protect one party from the counterparty. In CEX, the platform is one party who knows the exact information of the counterparty. 
}
\fi


%\tian{central bank digital currency: UTT, Platypus}

\iffalse
\tian{cross-chain atomic swap: there are some works on the privacy-preserving cross-chain atomic swap\cite{deshpande2020privateswap}, but its privacy depends on the confidentiality and anonymity properties of the underlying blockchains. If the swap protocol involves transparent blockchain, like Bitcoin chain, it cannot protect privacy of transactions.}
\fi
%\tian{discuss payment, swap and DEX}


\iffalse
Privacy/anonymity are classical topics that have been studied for a long time. Many works have been proposed including untraceable e-cash \cite{chaum1988untraceable}, and recent ones of decentralized anonymous payment \cite{zerocash,monero}, anonymous layer-2 payment \cite{tairia2l2021,ng_ldsp_2021} and CBDC \cite{tomescu2022utt,Platypus}. 
%In payment setting, 
They provide anonymity of sender and receiver and secrecy of the payment amount.
But they only supports one kind of asset and the private payment systems are built on a single private closed blockchain \cite{monero, zcash}, smart contract \cite{bunz2020zether,diamond2021manyzether}. %or layer-2 solutions \cite{tairia2l2021,ng_ldsp_2021,qin2022blindhub}.
It cannot handle the exchange between different kinds of cryptocurrencies especially for some public cryptocurrencies.
\fi

%As briefly discussed above, 
First, not only anonymous payment hub solutions cannot be directly applicable, even the techniques
%cannot be applied directly as an external anonymity mechanism; moreover, the techniques of them 
(e.g., viewing the exchange platform as the hub instead, while each user can be both a payer and payee) are not sufficient either for the {\em ``internal''} anonymity. The key difference, again, lies in the functionality difference of payment hubs (and other payment related solutions in general) and exchange platforms. 

Usually, in an anonymous payment hub, payer-payee exchange some information first, and then each runs some form of (blockchain facilitated) 
 fair exchange protocol with the hub. For anonymity, they would require a bunch of payers and payees to have some on-chain {\em setup} first with the hub, and $k$ active payments, so that the link between each pair of payer-payee can be hidden among those $k$ transactions; otherwise, each individual incoming transaction can be recognized by the hub. But in an exchange platform, there is no other entity for such setup, each individual request would be independent from the view of the platform: when user A, B purchase some BTCs from the exchange platform, 
 %naively applying techniques from the anonymous payment hub, 
 these purchase requests can trivially be distinguished by the platform (i.e., $k=1$).
% \tian{why? payer-payee issue or k-anonymity issue? oh, I see, although the hub (platform) does not know A exchanges with whom, it does know it is A is buying BTC, so the anonymity in the hub setting is not applicable in the exchange platform}
 %, e.g., knowing whether two requests from the same user.  

 Another issue (not covered in the payment solutions) in anonymous exchange is that every exchange transaction between a user and the platform contains two highly correlated parts: the transaction from user to platform and that from platform to user. The amounts are based on the exchange rate, e.g., A pays 1 BTC, for 15 ETHs. While in (anonymous) payment solutions, any two transactions can be completely independent, e.g., A pays 10 BTCs to B (e.g. platform here), while B pays 1 ETH to A.
 %\tian{While (anonymous) payment solutions do not guarantee this property and two transactions can be completely independent. //cannot get information from the eg example}

%In the former, they require $k$ senders all initiate transactions/payments 
There are also some works on private Decentralized EXchange (DEX for short) \cite{bowe2020zexe, Baum2021P2DEXExchange} where users exchange cryptocurrencies with each other. % directly or with smart contract.
%However, its privacy very different from our setting.
The privacy model in DEX is different from that of our centralized setting.
It %focuses on trade anonymity and trade confidentiality and 
keeps the transaction information secret {\em except} for the trading parties.
Again, in our setting, the platform is one of the trading parties who can learn the information of the other trivially.
%In the former, the transaction is one direction, in the sense that   
%Payment channel hub (PCH) is a set of payment channels.
%Each user establishes a payment channel with a central tumbler then they pay each other via it as an intermediary.  Anonymous PCH achieves the payment unlinkability between the sending transactions and receiving transactions, which is described as an interaction multi-graph \cite{heilman_tumblebit_2017}. 


%While such unlinkability has one drawback: it is limited to active users and the tumbler knows the number of user's transactions. If a sender is more active (sending more transactions), it is more likely to link it to a receiver. This is unavoidable as the design does not hide the senders' and receivers' activities, just mix the link. However, users' activities could leak information. We hope to protect users so that active and inactive users have the same possibility to be linked to a withdrawal transaction in our exchange system.

%\yanan{place where for atomic swap? it supports cross-cryptocurrency exchange, Can we take as one party the platform with different cryptocurrencies, and users exchange with the platform for different cryptocurrencies?  atomic swap pays much effort how to ensure fairness. If the privacy relies on the underlying blockchain, }
Atomic swap across different ledgers supports the exchange between different cryptocurrencies.
%, which is similar to a centralized multi-cryptocurrency exchange system. % in supporting multiple cryptocurrencies.
While atomic swap pays much effort on ensuring fairness, the only privacy-preserving atomic swap work \cite{deshpande2020privateswap} reduces
%There are some works on the privacy-preserving cross-chain atomic swap\cite{deshpande2020privateswap},  more cites??, but its privacy depends  
the confidentiality and anonymity properties to the underlying blockchains. 
If the swap protocol involves cryptocurrencies on transparent blockchains, like Bitcoin and Ethereum, these two transactions can be linked easily via their amounts. 
%For more detailed comparisons, we defer to Appendix \ref{rwk}. \tian{no appendix}
%It is unsuitable for anonymous exchange system.
%since their amounts are relevant according to the exchange rate.
%So it is easy to link these two transactions in the ledgers.
%
%\red{
There is only one private  fiat-to-Bitcoin exchange \cite{yi2019new}. 
%To prevent linkability by the input UTXO, 
During withdraws, the client chooses one UTXO and mixes it among $k$ transactions. 
To prevent linkability by the transaction amount, it requires each withdrawal to be fixed for 1 BTC. 
%So it also only achieves $k$-anonymity. 
And if two clients choose the same BTC, only one of them would get paid.%} 
%Besides the inconvenience of the fixed amount and security restriction of $k$-anonymity, the design is not compliable with regulations without leaking privacy.
%\yanan{move back this paragraph from related works in appendix}

%\tian{fiat-to-cryptocurrency: fixed amount and k-anonymity}

It follows that the natural question of anonymous cryptocurrency exchange is still open.
%\noindent\textbf{DEX}



%\tian{discuss PCH}

%\noindent\textbf{PCH}

%The PCH defines unlinkability in terms of an interaction multi-graph \cite{heilman_tumblebit_2017}. The star topology of PCH is very similar to the exchange scenario where the user sends one kind of asset to the exchange platform and receives another kind from it. Regarding the exchange user as the sender and receiver at the same time and the platform as the hub, PCH's unlinkability seems related to our goal that cutting the link between two accounts. Nevertheless, it is not suitable to be used to design a private exchange system due to the  operation restrictions and limited privacy: PCH relies on the payment channel which is only valid before the expiration time, and the fixed lock fund restricts the exchange amount. Some constructions require the off-chain transaction amount is a fixed denomination \cite{tairia2l2021,glaeser2022foundations} or be variable but concealed \cite{qin2022blindhub}.  The anonymity level of PCH depends on the number of active users and their exchange times in an epoch. Withdrawal requires closing the channel which displays its changed amount.  If a user just exchanges once, his two channels can be linked easily via the changed amounts.


\ignore{%%%%%%%%%%%%
Payment channel hub (PCH) is a set of payment channels.
Each user establishes a payment channel with a central tumbler then they pay each other via it as an intermediary. 
The PCH defines unlinkability in terms of an interaction multi-graph \cite{heilman_tumblebit_2017}. 
\iffalse
It is a mapping of transactions from a set of senders to a set of receivers in an epoch.
An interaction graph is called compatible if it explains the view of tumbler.
The unlinkability requires that all compatible interaction graphs are equal and the anonymity set depends on the number of compatible interaction graphs in the epoch.
Since the payment amount can be used to link the sender and receiver trivially, the unlinkability requires the amount to be fixed \cite{heilman_tumblebit_2017,tairia2l2021,glaeser2022foundations} or concealed \cite{qin2022blindhub}.
\fi
The star topology of PCH is very similar to the exchange scenario where the user sends one kind of asset to the exchange platform and receives another kind from it. 
%And there are some works adding anonymity on the PCH to prevent the tumbler from linking the sender and receiver.
Regarding the exchange user as the sender and receiver at the same time and the platform as the hub, PCH's unlinkability seems related to our goal that cutting the link between two accounts.
Nevertheless, it is not suitable to be used to design a private exchange system due to the  operation restrictions and limited privacy:
PCH relies on the payment channel which is only valid before the expiration time, and the fixed lock fund restricts the exchange amount.
Some constructions require the off-chain transaction amount is a fixed denomination \cite{tairia2l2021,glaeser2022foundations} or be variable but concealed \cite{qin2022blindhub}. 
%is a recent work that supports variable amounts.
The anonymity level of PCH depends on the number of active users and their exchange times in an epoch.
%It assumes that there are many active users and each of them transacts many times during the epoch.
Withdrawal requires closing the channel %and open a new channel for the next withdrawal.
which displays its changed amount. 
If a user just exchanges once, his two channels can be linked easily via the changed amounts.
For a more detailed comparison, we defer to Appendix \ref{rwk}.
}%%%%%%%%%%%%

\iffalse
(i) PCH requires the establishment of payment channels on the blockchains by the tumbler and users.
It means each exchange needs the deployment of two channels in two blockchains. 
The channel is only valid before the expiration time, so the establishment work should be done repeatedly to make sure that they can exchange freely.
The fund locked in the channel is fixed and the user cannot transact more than that locked amount. So the exchange amount is limited by the money locked in the channel rather than the money that the user owns.
Even if the user has a huge amount of BTC, he cannot exchange them into ETH more than the amount locked in the Ethereum channel.

(ii) The anonymity set of PCH is just the active users in an epoch.
Some constructions require the off-chain transaction amount is a fixed denomination \cite{tairia2l2021,glaeser2022foundations} which is inconvenient.
BlindHub \cite{qin2022blindhub} is a recent work that supports variable amounts.
But it still assumes that there are many active users and each of them transacts many times during the epoch.
If the sender just sends once and the receiver just receives once before closing the channel, the changed amounts of their channels would link them easily.

(iii) The exchange system consists of deposit, exchange and withdraw operations where the deposit and withdrawal amount must be public and variable.
We consider the anonymity in the whole system. The interaction graph model is not enough since it only focuses the payments in one epoch and only supports the \textit{k}-anonymity of active users. 
It drives us to define a more strong model of interaction indistinguishability.
\fi

\iffalse
In the other hand, all above primitives do not support fiat money transactions and they are generally deployed in the decentralized setting like smart contract. 
They are unaffected by the KYC requirement and do not consider other accountability requirement.
\fi




\medskip
%\subsection{Our contributions}
\noindent{\bf Further challenges.} Besides the issues mentioned above not covered in existing studies, the anonymous cryptocurrency exchange setting has several other features that bring about more challenges: since the exchange system is always connected with external blockchain (e.g., via the {\em deposit} and {\em withdrawal} of coins), it automatically leaks highly non-trivial information (e.g., 3 BTCs has been deposited, and 2.9 BTCs has been withdrawn/transferred out 2 minutes later) such that how to best deal with them requires care.
%One simple analogy we can see is the setting of encrypted search, e.g., order revealing encryption. When some non-trivial leakage is allowed to enable certain search functionality, it often turns out that the consequence is much more disastrous, sometimes making the security completely vacuum \cite{naveed2015inference}. 
%Ignoring its privacy would leak many information of users in other systems, especially for transparent blockchains.
%\tian{would the analogy be helpful for understanding? maybe others are not familiar with encrypted search}


\iffalse
PCH is also connected with the blockchain, but it only focuses the payments in one epoch and its unlinkability in the interaction graph model\cite{heilman_tumblebit_2017} only provides the \textit{k}-anonymity of active users. 
It drives us to define a stronger model.
\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\tian{We design the basic construction using anonymous credential, how can we say role out e-cash? Seems UTT can cover the basic scheme, but not the private exchange (full anonymity) and profit computation (compliance)}

%We define withdraw anonymity and give a basic construction. %using anonymous credential.
%Although this basic scheme is efficient and satisfies some kind of stronger withdraw anonymity (unlinkable among all eligible users including inactive ones), it is still far from the needs of the real world, since the achieved anonymity is not enough for the unique exchange scenario with complex leakage profile. Moreover, the basic construction does not capture the real compliance rules.
%We explain it as follows.


% 
%\tian{just note: our goal is enhanced from the following three aspects: stronger anonymity, compliance and maintaining the efficiency}

 \noindent{\em The right anonymity/privacy goal.}\ 
From a first look, 
we may just handle the withdrawal operation and define a basic, direct anonymity notion, that breaks the link between the receiving account and user identity, and leave other operations unchanged for efficiency. 
%Note that this is modeling issues, which is different with only leveraging external anonymity payment solutions.
%we may define a basic anonymity notion by requiring  any withdrawal transaction is indistinguishable for two different users if both of them are able to withdraw successfully. Indeed, we have a simple construction.
%
A bit more formally, given two different users and a specified withdraw transaction, we can require that it is infeasible to distinguish which one conducts the withdrawal if {\em both} of them are eligible. % Indeed, we can have a simple construction.
%In this way, we may only need to handle anonymous withdraw, and leave other operations as now for efficiency. construction.
% for this purpose.
However, if we examine the  {\em anonymity set} of the withdrawal, it only consists of users who have enough amount of the specified coin, which could be few. %while there is no guarantee on anonymity size. 
For example, for some unpopular assets, maybe only a very small number of users own such kinds of coins; or one user may hold a significantly larger amount of the coin than others. When a large-volume withdrawal of such token is taken place, it is easy for the platform to identify the user.
%the size of the anonymity set is  very small. 
%Such a narrow anonymity set cannot provide sufficient protection, especially for holders of not-so-popular assets.

%probably most users in the exchange system can own it if they want, 


%only one or two. %   When there is a withdrawal with a large amount from some whale account, maybe only one or two users have enough assets and the platform knows who they are. 

%Note that modeling the withdraw anonymity is already involved. 
%The above simple example hints that basic anonymity is weak. 
We then turn to consider stronger anonymity. One may suggest to gradually strengthening anonymity by allowing fewer unnecessary leakages (keeping some internal transaction data {\em private} such as amount) and leave seemingly safe information such as coin names as now (to avoid potentially complex solutions for protecting such info). Unfortunately, many of remaining transaction metadata, together with the inherent leakages such as 3 BTCs have been withdrawn by someone to an external address, can still reduce anonymity set. %(we will demonstrate with detailed examples later in Sec. \ref{WithdrawAnonymitySection}). 
%it is repeated with the end of this paragraph
It is hard to have a reasonably stronger anonymity without full internal transaction privacy (excluding the inherent leakage during withdraw/deposit), as it is unclear what is the actual consequence of each specific leakage.
For these reasons, we choose a definition that insists the system does not leak anything more than necessary to the exchange platform (essentially requiring privacy). We will explain more in Sec. \ref{WithdrawAnonymitySection}.

%completely hiding the internal transaction privacy 

%``clearly defining'' plausible leakage, 
%as it is unclear what is the actual consequence of each specific leakage \footnote{There were works on private (decentralized) exchanges, or payments \cite{yi2019new,Baum2021P2DEXExchange,chu_manta_nodate}, but to them, everything is essentially happening within the system, thus no subtle issues in modeling, as there is no external ``side channel''.}.  

%which could capture all the unnecessary leakages to maximize the anonymity set. Unnecessary leakage means some leakage in the system which can be prevented if taking measures, such as the user identity, amount, and asset kind of an exchange transaction.  

%Interestingly, we observe that all the unnecessary leakages could reduce the anonymity set once leaked, 

%On the other hand, the exchange system also has some leakages that are unavoidable due to the existing external environment and assumptions, including the time and frequency of each operation, the amount and asset kind of each withdrawal (i.e., withdraw 3 BTCs to address A) etc. %the amount and asset kind of each deposit, 
%and the identity of the fiat money deposit. %These leakages could provide an external ``side channel'' to threaten anonymity. 
%However, it is quite unclear how we may rule out those trivial cases due to the unavoidable leakages case by case.


%Specifically, inspired by Zcash~\cite{zerocash} on the private ledger, we define full anonymity called interaction indistinguishability. Intuitively, it requires any two exchange systems with supported operations to be indistinguishable as long as their necessary leakage profiles are the same.
%   The first step is to identify all the unnecessary leakages in the exchange system.    via additionally hiding the users' asset states, e.g., kinds and balances, inside the platform involving all possible operations besides the withdrawal. The fiat money deposit is unavoidably public to the platform, which is a trivial leakage that should be excluded. 

\ignore{
The above simple example hints that we need to consider reasonably strong anonymity via hiding the users' asset states, e.g., names and balances.
%The above simple example hints that we need to consider additional confidentiality requirement that prevents the platform from knowing the user's asset state, e.g., balances.  
But the deposited asset is also public which implies the user must conduct exchange transactions after each deposit to hide his asset state. What's worse, even the transaction time, e.g., when there is only one single withdrawal request from a user, no technique can break the link between the receiving account and request (which contains real user identity). Actually, it turns out to be unclear how we may rule out all those trivial cases or allow certain leakages to the platform; and more importantly, it is completely unclear what is the actual consequence of any specific leakage. \footnote{There were some previous works on private (decentralized) exchanges, or payments \cite{yi2019new,Baum2021P2DEXExchange,chu_manta_nodate}, but to them, everything is essentially happening within the system, thus no external ``side channel''.} 
It follows that to consider a reasonably strong anonymity, we have to consider anonymity and privacy {\em simultaneously} even {\em inside} the platform.
}
%Therefore, the classic anonymity and confidentiality experiments are not suitable for this setting due to the public information. 

%However, given a public special withdrawal,

%Let us see a naive attempt using the classic anonymity experiment. 



\ignore{%%%%%%%%
In the payment case, the transaction amount is kept confidential so no one knows who have enough balance to generate the transaction so the anonymity is large.


In anonymous payment system, the confidentiality of transaction amount is regarded as the necessary step for anonymity.
Unfortunately, it cannot be true in the withdrawal.
But does it mean it is impossible to preserving anonymity for withdrawal?
If there is any hope, what is the best anonymity level that it can achieve and how to model it?
}%%%%%%%%%





\noindent{\it Preserving major compliance functionalities.} We also need to preserve all the critical functionalities that are currently provided by centralized exchange platforms, including compliance such as generating tax reports for users and checking sufficient reserve for the platform. \footnote{There are some related works in  accountable privacy (e.g., PGC \cite{chen2020pgc}, UTT \cite{tomescu2022utt}, Platypus \cite{Platypus}, etc),
but they only focus on the payment with a single kind of asset and enforce limits on one transaction amount or account balance or sum of all sent or received values. 
%(Enforcing limits on transaction value and sum of all sent values are two general regulatory rules.)
Note that these compliance requirements cannot cover the profit computation which uses the specific buying price without linking to that transaction.}


There are many types of assets/coins in an exchange system, %and each of them is with a price as an extra attribute.
and their prices fluctuate over time. 
Users gain a profit by capitalizing on the price difference between buying and selling.
%Users make a profit from the difference between the buying and selling prices.
It is often mandatory for users to pay taxes on their {\em accumulated} profits over time. 
%The profit in exchange or withdraw is computed based on the buying prices from past transactions and it is {\em accumulated} overtime as the final tax filing value.
%Specifically, when users trade their assets, they can just use part of it. 
At each year end, users obtain a tax report from the platform so that they can report their annual profit, e.g., to Internal Revenue Service for tax filing. %\footnote{Internal Revenue Service, the revenue service for the United States federal government, which is responsible for collecting U.S. federal taxes and administering the Internal Revenue Code, the main body of the federal statutory tax law.}   
For example, based on the suggested tax policy of Coinbase \cite{coinbasetax}, transactions that result in a tax are called taxable events. Taxable events as capital gains include selling cryptocurrency for cash, converting one cryptocurrency to another, and spending cryptocurrency on goods and services (e.g., withdrawing cryptocurrency).%\footnote{As shown in \cite{coinbasetax}: ``taxable events happen when you realize losses or gains, meaning you've sold your cryptocurrency by either selling for cash, converting to another cryptocurrency, or spending it on a good or service. The gains are unrealized if you still own the original shares." }
%


In the current transparent exchange system, the platform records the whole transaction history for each account and extract easily their taxable events. 
%tian
The platform can also check the reserve easily as it knows the asset details of each account. 
This ensures that the platform possesses sufficient assets to meet the withdrawal requests of users.

However, in the anonymous setting (now also requires privacy), the platform has no idea about the asset detail of each account. 
It cannot prove solvency in the same way as before. 
Furthermore, the platform knows neither the actual profit nor the relationship between these transactions with any user. 
Without careful designs to calculate accumulated profit (without violating privacy/anonymity), some users could always claim they made no profit. 



\iffalse
We aim for the following goal in this paper:
\begin{center}
	{\em To protect users' privacy {\em  outside the platform}, i.e., breaking the link once the coin is moved out; while at the same time, to ensure the platform could still fulfill its duties on KYC or other compliance requirements.}
\end{center}
\fi


%%%%%%%%%%%
% \noindent{\em Private yet compliable exchange.} 
%Besides the privacy, the compliance requirement (e.g., generating tax report) in the exchange setting also cannot be ignored, which brings new challenges.
% to make sure it is correct without affecting the privacy. 






%But we consider some more general cases in which updating compliance information may require some past transactions just like computing the profit from buying price.


%In the exchange setting, there are a lot of kinds of assets. 
  

 \noindent{\em Striving for practical performance.} 
%Theoretical feasibility could be reachable without considering efficiency, e.g., with large communication (e.g., proof sizes due to straightforward application of NIZKs), or large computation (e.g., due to simple use of SNARK). 
%Under a proper model and the special compliance requirement, it is another issue to design an efficient exchange system with many kinds of assets.
Privacy preserving constructions normally use zero-knowledge proofs. 
Although the deposit and withdrawal assets are public, the exchange details (e.g., 1 BTC for 15 ETHs) should be hidden and proven in zero-knowledge that the transaction is valid and the prices 
%sof the new exchanged asset 
are recorded correctly.
In theory, zkSNARK \cite{bitansky2013succinct} may enable succinct proof size and verification time.
But the proof generation incur heavy computation for users.
$\Sigma$-protocols may also be useful, but hiding the exchanged asset types in all $n$ kinds assets usually requires communication/computation cost growing at least {\em linear} in $n$. For a practical design, we need to reduce the communication and computation overhead to be as small as possible (e.g., ideally {\em constant} cost).
%An intuitive idea is that: the user generates $n$ commitments and proves that only the $i$-th committed value is 1 and all others are 0s,
%then multiplying them with respective public prices and adding them together, so the result is a commitment on the price of the $i$-th asset.
%They can be proved with logarithmic proof size using one-out-of-many proof, and the generation and verification time are still (super)linear with $n$.
%Firstly, the user needs to send $n$ commitments to the platform for its verification.
%So the communication cost is linear in $n$.


%For a practical design, we need to reduce the communication and computation overhead to be as small as possible (e.g., ideally {\em constant} cost). Unfortunately, existing anonymous constructions \cite{zerocash,bunz2020zether,diamond2021manyzether,tairia2l2021,ng_ldsp_2021,Bl2019UpdatableSystems,chen2020pgc,Platypus,tomescu2022utt} cannot be used because their models are either too restricted or their functionalities are too limited. 
%and similar to our basic anonymity.
%For example, Zerocash \cite{zerocash} uses the heavy zkSNARK \cite{bitansky2013succinct} and anonymous Zether \cite{bunz2020zether,diamond2021manyzether} restricts each user can only generate one transaction in a given epoch since all users' account states are maintained in a public ledger. 
\iffalse
A$^2$L \cite{tairia2l2021} and LDSP \cite{ng_ldsp_2021} only support payment with fixed coin denomination. 
%Incentive system\cite{Bl2019UpdatableSystems} does not support exchange or any regulation rules.
PGC \cite{chen2020pgc}, Platypus \cite{Platypus} and UTT \cite{tomescu2022utt} support accountable payment, but they only focus the compliance rules on one transaction amount or sum of all sent or received values and cannot cover the exchange and profit making setting.
\fi
%For more detailed comparisons, we defer to Appendix~\ref{rwk}. \yanan{check a bit any works not mentioned in the main body and add a brief review. Or just integrate to the previous paragraph}

\iffalse	
As the price of bitcoin soaring, trading bitcoin makes huge profits.
With the improvement of the regulatory system, it is mandatory for users to pay taxes on their profits.
In the current transparent system, the platform records all the income of each account from their spending (exchange or withdrawal) operations.
It directly links every spending operation with user's account which also leaks the identity of the owner of bitcoins.
	
In the privacy-preserving setting, the exchange has no idea about the relationship between withdrawal operations with any user.
How can the platform or user maintain privacy and the basic compliance information, e.g., the profit of each account at the same time?
%Since the client needs to sum up his incomes of withdrawing some specific bitcoins.
\fi	


\iffalse
\noindent\textbf{Challenges}
In a payment system, the transaction confidentiality is usually seemed as the stepping stone of anonymity.
However, it is far from guaranteed in an exchange system where the withdrawal transaction surely leaks some information, such as the name and amount of the asset. 
It weakens the user anonymity. 
In this case, how can we live with the leakage? 
What is the ideal anonymity and how can we achieve it? 

At the same time, suppose the withdraw anonymity is achieved, how to make sure the users are accountable?
They are required to comply with some regulation rules by providing the compliance information to some authority. 
Maybe it is not hard to check each individual transaction since the withdrawal is public. 
But things become complex when the compliance information is related with the user's past transactions and it does not violate the anonymity of withdrawals.
\fi
	

\vspace{-0.2cm}

\subsection{Our contributions}

%\paragraph{\bf{Model}}
\noindent\textbf{Modeling.}
We for the first time formally define the private and compliable cryptocurrency exchange.
%In an exchange platform, basically the user cannot exchange or withdraw more asset that he actually owns.
%To comply with some regulation rules, the user should provide his compliance information correctly.
%Surprisingly, there is little work on it especially for discussing the withdrawal anonymity.
We give a basic version of anonymity first as a warm up, which only cares about the withdrawal operation.
As we briefly discussed above, hiding only part of transaction data may not give a reasonably strong anonymity. 
%the withdrawn asset and exchange activities within the exchange system may be used to narrow down the anonymity set which is not covered by this experiment. 
%Those leakage information hinders us from defining a proper model.
%To enhance the anonymity by including more users to enlarge the anonymity set, 
%We have tried some modeling methods to enlarge the anonymity set.
In the end, we define the security model insisting that the exchange leaks essentially no information to the platform. In this way, we obtain the best possible anonymity (given that public withdrawal is always there). We also carefully define {\em soundness} properties such as {\em overdraft prevention}, and {\em compliance}. For details, we refer to Sec. \ref{model}.
%\ref{WithdrawAnonymitySection}. 
% we find the interaction indistinguishability is a proper model inspired by the ledger indistinguishability of Zerocash \cite{zerocash}.
%in which the leakage information are publicly consistent in different interaction records.

 

%\paragraph{\bf{Construction}}
\noindent\textbf{Constructions.} 
%The basic anonymity can be achieved by single-use anonymous credentials for each withdrawal. But its anonymity set is restricted and does not satisfy the compliance rule rigorously.
%The platform maintains the records of each user's withdrawals to ensure the correctness of the compliance information he requests to sign.
We first give a very simple construction satisfying the basic withdraw anonymity, and showcase its limitations. 
We then design the first private and compliable exchange system which is provably secure in the full private model.
Users are hidden in a large anonymity set, and they cannot withdraw more asset than they own, or report false compliance information.
To obtain full anonymity, user's information are concealed as much as possible in each transaction,
including user identities 
%in all kinds of transactions 
and the exchanged assets details. Soundness properties are ensured via efficient NIZK proofs specially designed for our purposes.
%But for compliance such as generating the tax report, we have to also rely on the user to generate and prove.
Note that proving correctness of a exchange request usually leads to a proof whose size is linear to the total number of asset types; instead, we propose an efficient construction with {\em constant} cost in both communication and computation which is independent with the number of asset types and users in the system.
%proof size for each kind of transaction and the generation and verification time are also independent with the number of asset kinds and users in the system.
%In the meantime, the compliance information (e.g., accumulated profit overtime) is recorded privately and correctly as per the transactions.
%which can support tax filing and extended compliance functions.


%If the compliance information is still recorded separately, the user may just provide partial of them. 
%We need some more advanced tools to deal with the private and anonymous exchange. 
%So we define a new primitive: oblivious updatable anonymous credential.
%On the one hand, we need to make sure the reported compliance information is correct with respect to the user's all operations.
%On the other hand, the records involved in each operation should be hidden.
%It updates the compliance information and hides which record is involved. 
%It also hides the exchange content from the platform.
%It means the records are used privately without restriction but their compliance information can be put together in a publicly verifiable way.

 
\noindent{\bf{Performance evaluations.}}
We implement and evaluate our $\mathsf{\name}$  system and test the cost breakdown in each operations, and compare with those in plain exchange (without anonymity). Considering the presence of TLS communication, our overhead is minimal. We also compare with other relevant systems\footnote{\label{ucs}There is a concept of updatable anonymous credential~\cite{Bl2019UpdatableSystems}, that share similar theoretical structure of proving properties of attributes in anonymous credential; however, their main application to incentive systems supports only limited functionalities and the achieved anonymity is weak, see Sec.~\ref{IncentiveSystem}. We have to design more complicated compliance functions.} for further evidence. See Sec.~\ref{sec:eval} for details.
%\tian{add some concrete evidence here to show that our private version comes with just modest cost }


%in particular, join, deposit only take less than 10ms, while the computation time of exchange on user side takes  26ms(+22ms), which is practical, especially in presence of TLS communication. Here the bracked part 22ms denotes the pre-computing cost while waiting for platform dealing the last request.
%
 %and platform side varies in 6\textasciitilde 88ms, 
% Compared with plain deposit, exchange, and withdrawal procedures in existing centralized exchange systems, the communication overhead of each procedure in \name\ varies in only 3\textasciitilde 12kb.% \qiang{slightly more precise, communication is for one sell, purchase, or transfer, or any of them, what is original communication?}
%{add evaluations}, compare with other works, operation time, other evaluation? transaction size, throughput (xx tx per second), latency

%\vspace{-0.2cm}


\section{Technical overview}
%\tian{high level overview; simple example; achieve full anonymous; add compliance; efficient private exchange}
%
We first provide a high-level overview of the technique. Typically, there are two main parties involved: the platform and the user. However, in certain cases such as tax filing, there may also be an external authority involved. 

 \noindent{\em Workflow of exchange system.}
First, the user provides the real identity to the platform during registration.
Then the user interacts with the platform to deposit, exchange (e.g., 1 BTC for 15 ETHs) and withdraw asset. 
For compliance, the user generates his compliance report, gets it certified by the platform and reports to an authority. 
The platform also generates information to check its own solvency.

%\yanan{seems here we only consider client compliance. Shall we mention platform compliance such as solvency?}

%\tian{yes, will change this figure}
%\yanan{we tune the system data flow a bit to cover solvency.}
%So he files his compliance information and requests the platform to sign on it. 
%gets an anonymous credential issued by the platform which is called the \textit{registration record}. 
%\footnote{\tian{ a little early to put here? there is no registration record in basic and privacy only}}
%It contains an identifier, her identity, the accumulated costs and gains.
%%%%We use individual credentials to represent the Alice's assets which is called the \textit{asset record}.
%%%%%%It contains an identifier, her identity, the kind, amount and price of this asset. With these records, the user interacts with the platform in the system. 
We use Fig \ref{overview} to visualize these (simplified) procedures.
%Figure \ref{overview} shows how the interaction proceeds in the system. 
%There are four steps.
%%%%The user interacts with the platform: join the system, deposit asset, exchange asset, withdraw asset and request signature of compliance information. 
Each interactive protocol can be expressed by \ding{192} \ding{193} \ding{194} steps.  
%When an interaction finishes, the user obtains new records. 
%representing his assets and compliance information.
%At the end of request procedure, 
The user sends compliance report to the authority who verifies it in step \ding{195}.
The platform checks in step \ding{196} whether its internal state satisfies the platform compliance rule.
%{We use Fig \ref{flow}(b) to visualize the records evolution.} 
%in the interaction for each kind of transaction.}
%The whole system satisfies the following properties.


\begin{figure}[!htbp] 
\centering 
\includegraphics[width=0.45\linewidth, height= 0.3\linewidth]{overview_check1.png} 
%%%\captionsetup{font={small,rm,stretch=0.8}}
%, justification=raggedright}
\caption{Overview of exchange system: \ding{192} \textit{Transaction request}; %: user generates the transaction using his records;
%$\mathrm{user\ generates\ the\ transaction\ using}$ $\mathrm{ his\ records;}$ 
\ding{193} \textit{Transaction processing}: platform verifies the transaction and process it; \ding{194} \textit{Transaction completion}: user completes the transaction; \ding{195} \textit{Compliance verification}: authority verifies the compliance report of the user; \ding{196} \textit{Compliance check}: platform checks internal state with the platform compliance rule} 
\vspace{-0.2cm}
\label{overview} 
\end{figure}


%As mentioned before, we aim to design a practical private exchange system that provides the best privacy protection and supports the current complex compliance rules. 

%\qiang{Add some technical challenges}

%There are three parties: the exchange platform (which we called platform to avoid confusing it with the exchange transaction), the user (client of the platform) and the authority who is only in charge of verifying the compliance information.  
%In the current transparent exchange system, each user has an account in the platform that is linked with its real identity.
%The platform simply modifies the state of users' accounts based on their transactions (at the backend). 
%To protect users' privacy, we require the platform cannot link their real identities with the wallet addresses in the withdrawal transactions.

%\tian{model challenge: anonymity and compliance, our model sketch}
%It requires careful 

%The exchange system is special in two folds: public withdrawn assets and involved compliance rules.
%Due to the withdrawn asset issue, the classic anonymity experiment only provides limited anonymity set for users.
 
\ignore{%%%%%%%%%%%% overview about models
\noindent{\bf Security models}. As we discussed above, a reasonably strong anonymity requires hiding user's identity and transaction details as much as possible. To translate this intuition into a proper model, we define  {\em interaction indistinguishability} that prevents the platform from knowing anything non-trivial from the interactions with users than that has to be public. To emulate the interactions supporting usual functionalities for deposit, exchange, etc, we carefully define a set of oracles. These oracles are duplicated to create two identical environments that remain consistently aligned with the public information throughout the experiment. The challenger determines which set of oracles to use when responding to the left queries in the pairwise interactions. It is infeasible for the adversary to distinguish which oracle set it interacts with is answering the left ones of pair-wise queries, so the platform cannot get more information from interactions. 
%Each oracle has two versions defined by the challenger, both of which are consistent w.r.t the public information. For each query, it is answered from one version of each oracle. It is infeasible for the adversary to distinguish which oracle set it interacts with, so the platform cannot get more information of users. 
%We then argue that such a model is essentially {\em best possible} anonymity. 
Directly defining {\em overdraft prevention} and {\em compliance} presents challenges in this privacy setting. We carefully generalize the idea of {\em proof of knowledge} to capture those soundness properties.
%we particularly consider for tax filing purpose that the reported accumulated profit is correct. 
For details, please refer to Sec. \ref{model}. %and \ref{WithdrawAnonymitySection}.
}%%%%%%%%%%


%More importantly, in our setting, the adversary is allowed to have access to usual functionalities as the platform. We define multiple oracles carefully to simulate the interactions between adversary/platform and honest users for deposit, exchange etc. 

%Each query is answered from one pair: $(Q, Q')$ and they are forwarded to different oracle sets by the challenger.
%They are public consistent to simulate the minimum public information exposed in the system. 



%Inspired by the ledger indistinguishability of Zerocash \cite{zerocash} which tries to capture no information will leaked from the public ledger, we propose the interaction indistinguishability experiment that prevents the platform from knowing any more non-trivial information than that has to be public. 


%simply combining the classic anonymity and confidentiality experiments is not sufficient and some models are too strong to fit the real world setting.


%\tian{construction challenge: just e-cash is not enough, zksnark is too heavy, our design in high level, it is efficient even with a lot of kinds of assets}
\ignore{%%%%%%
 As we elaborated above, simple ideas either do not provide sufficient privacy guarantee or have efficiency issues. 
In a high level, % structure of our system %is a careful combination of the e-cash design with the account model.
%The user obtains a registration record issued by the platform which binds with his identity and maintains his compliance information from each transaction. The user deposits assets into the platform and gets asset records issued, then he consumes them in exchange or withdrawal transactions.
%is similar to the e-cash system where the bank issues coins (a credential on some fixed denomination values) to the user blindly. Here, 
the platform blindly issues credentials that include attributes like the asset type/name, asset amount, current price, accumulated profit, and even user id for compliance. 
However, certain attributes and their positions need to be hidden from the platform and proven to satisfy claimed properties in transactions. To achieve this, we employ commitment schemes along with efficient zero-knowledge proofs. %credentials are issued separately for different asset types 
%Some attributes should be hidden from the platform, and be proven to satisfy claimed property in the transactions, using commitment with efficient zero-knowledge proofs. 
To enable constant size record and transactions for efficiency considerations, we carefully design efficient proofs for relevant statements to optimize performance. 
%We illustrate our design idea step by step below.
}%%%%%%%%%
 \noindent{\bf Constructions.}  Based on the workflow above, we illustrate the design idea of our efficient system $\mathsf{\name}$\/ step by step.

%First, let us describe the simple {\em data flow of exchange system}.



%from basic anonymity to full anonymity to compliance and finally to efficiency.

 \noindent {\em Basic anonymity.} As a warm-up,  %we first look at basic withdraw anonymity. 
%We %can get basic (but limited) anonymity by using 
%use a blind signature (a one-time anonymous credential) and zero-knowledge range proof. 
%The deposit and exchange transactions are transparent to the platform. 
%For withdrawal, 
to just break the link between outgoing transaction (withdraw) and the history within the platform, we can introduce a preparation step. There, users ask for %one or multiple 
{\em one-time} anonymous credentials (as tokens) with amounts hidden to the platform (simply via a ``partially'' blind signature) that later can be used to do withdrawal. Users also submit a committed record containing asset details of the token for compliance purposes.  Now, the user balance becomes hidden, and users should prove that 
%that each hidden amount is positive and the sum of all hidden amounts is not larger than the balance, 
the sum of all hidden amounts is valid depending on his previous balance via zero-knowledge range proof. 
%At the same time, 
When withdraw, users could directly reveal such one-time credential (a valid signature on a random identifier and transaction etc), which easily prevents double-spending. Since now user balance is also hidden, all future operations including exchange, withdraw preparation will involve (efficient) zero-knowledge proofs of validity. 

%One-time credential ensures no double-spending. 

%After withdrawal preparation, the user's balance of the involved asset is hidden. As a result, users are required to prove in zero-knowledge that the asset balance is enough in the following exchange operations.
%This is also important for proving the validity of the accumulated state that will be used and verified by external parties for tax purposes. 

%But we do not use coins with fixed denomination which shows benefits with constant record size and transaction size.
%Our construction uses standard commitment scheme, blind signatures and efficient $\Sigma$-protocol as building blocks.
%It is provably secure in our full anonymity model and satisfies the compliance rules and is practical enough for real world.


\ignore{%%%%%
an intuitive idea is using the e-cash design: the platform issues coins blindly with fixed denominations for the user when they request to withdraw assets and deducts the same amount from his account.
In a withdraw transaction, the user consumes those coins by revealing their serial numbers with valid signatures from the platform. 
Although this method prevents the platform from linking the withdrawal transactions with the user's identity, it is still far from our expected since it only provides limited anonymity set. 
In other hand, we can instantiate using zkSNARK with succinct proof size and verification time. 
But the proof generation is a heavy work for users with resource-constrained devices.
}%%%%%



%\vspace{-1cm}




\iffalse
Firstly, it is impractical to maintain so many coins and take them as inputs in exchange or withdraw transactions.
Second, the anonymity set is not large enough.
The platform knows the account state of each user and the withdrawn asset, so it can narrow down the anonymity set to the users who have been deducted more asset than that in the withdrawal.   
Third, the compliance information is not exact.
After requesting, the user can withdraw assets at any time in an unlinkable way.
So it is hard to trace the real withdraw prices and verify the correctness of the reported profit without affecting their privacy. 
\fi

\iffalse
\begin{figure}[!htbp] 
\centering 
\includegraphics[width=1\linewidth, height= 0.3\linewidth]{plain.png} 
\captionsetup{font={small,rm,stretch=0.9}, justification=raggedright}
\caption{Exchange system with real name account}%: \ding{192} \textit{Transaction generation with records}: user generates the transaction using his records;
%$\mathrm{user\ generates\ the\ transaction\ using}$ $\mathrm{ his\ records;}$ \ding{193} \textit{Records issuance}: platform verifies the transaction and issues new records; \ding{194} \textit{Records completion}: user completes his new records; \ding{195} \textit{Compliance verification}: authority verifies the user's compliance information} 
\vspace{-0.4cm}
\label{plain} 
\end{figure}
\fi

%\tian{basic: one-time use anonymous credential/blind signature+range proof; full: blind signature + range proof+relation proofs on old and new commitments (for compliance, we need keep transaction records, but add and use transaction record in one credential leaks the position and transaction times which violates the privacy; private exchange needs heavy proofs); private and compliance: blind signature+range proof+relation proof, use separate transaction records and additional platform's signatures on prices.}

\ignore{
\noindent\textbf{Simple exchange example.} \
Here we describe the workflow in the exchange system via a simple example.
%When Alice joins the system, she gets a registration record maintaining her compliance information.
%As shown in the Fig \ref{plain}, 
Alice deposits 1000 USD in her account. %, she gets an asset record for it.
Then she exchanges 800 USD to 0.5 BTC with price 1600. 
%In this phase, 
%the old USD asset record is spent and 
%she gets a new USD record with amount 200 and a new BTC record with amount 0.5 and price 1600.
Afterward, she 
%spends the BTC record to 
withdraws 0.3 BTC when its price is 2000. 
%She gets a new BTC record with an amount 0.2 with the same price and 
For investing 0.3 BTC, the cost is 480 USD and the gain is 600 USD, which are added to her compliance information.
For tax filing, Alice files her accumulated cost and gain and requests the platform to sign on them. 
Then she shows them to the IRS authority. 
%During the above procedures, the spent records are cannot be used anymore.
%Depositing fiat money reveals the user's identity since the platform knows her bank account.
In this example, the platform always knows that it is Alice who is withdrawing. Then the platform could link her to the receiving bitcoin address, and trace future transactions related to this address easily.
%It can link her Bitcoin addresses and future transactions easily.

\noindent\textbf{Basic anonymity.} \ 
In the basic version, Alice interacts with the platform in real name when registers, deposits and exchanges.
When she wants to withdraw some asset, she requests the platform issue a credential for it which can be achieved via blind signatures.
She generates a commitment on an identifier and the number of the to be withdrawn asset and proves in zero-knowledge that she has sufficient asset for this withdrawal.
Once the platform is convinced, it signs on the commitment blindly.
Alice unblinds it and gets a valid signature on the identifier and asset information.
Afterwards, she can withdraw by showing the above message-signature pair.
The platform only knows that this is a user who has enough such assets and has requested but cannot link it to anyone of them.
}



%\tian{explain the full construction by splitting to full anonymity, compliance, efficient exchange three parts}


 \noindent{\em Full anonymity.} 
Additional protection on the exchanges and deposits is needed. Especially, the exchanges should not only be anonymous but also keep {\em asset type} and {\em amount} private. %Besides using anonymous credentials,
%Pure anonymity might be achievable with anonymous credentials. But 
Each exchange transaction requires the value of exchange-in and exchange-out to be equal. To calculate the value, users need to show the used prices (now committed) are two of all current prices and correspond to the two exchanged assets. Further zero-knowledge proofs on membership and equality will be leveraged. But doing them efficiently requires care and will be explained soon in {\em practical considerations}.   

\ignore{\yanan{annotate}
In the full anonymity design, 
Alice obtains an anonymous credential when she registers, then she uses it to interact with the platform anonymously all the way.  %and request it to issue new ones according to her transactions.  
The credential contains the following messages: an identifier, her identity and balance of all names of assets her owns which were initialized as zeros.
In the following transactions, Alice proves that she owns a valid credential and requests the platform to issue a new one on the same message except a fresh identifier and correctly modified balance numbers according to the transaction.
Especially, the exchanged assets should be concealed different from the deposit and withdraw. %which means the positions and changed numbers of the modified balances.
}
\iffalse
\setlist{nolistsep}
\begin{itemize}[noitemsep,leftmargin=*]
    \item When deposits 1000 USD, the USD balance gets credited by 1000.
    \item When exchanges 800 USD to 0.5 BTC, the USD balance is deducted by 800 and the BTC balance gets credited by 0.5. 
    These names and amounts are concealed.
    Alice proves that she has enough asset to deduct and the credited amount is correct with respect to the exchange price.
    \item When withdraws 0.3 BTC, the balance of the BTC gets deducted by 0.3 and she proves the remaining balance is non-negative.
\end{itemize}
\fi


\iffalse
\begin{itemize}
    \item When deposits 1000 USD, the balance of the deposited asset gets credited with the correct amount.
    \item When exchanges, the balance of one asset gets deducted and the balance of one another gets credited, and the names and amounts of these two assets are concealed.
    Alice proves that she has enough asset to deduct and the credited amount is correct with respect to the exchange price.
    \item When withdraws, the balance of the withdrawn asset gets deducted with the amount in the transaction and its remaining balance is non-negative.
\end{itemize}
\fi

\ignore{
Although this method makes all transactions unlinkable (and achieves the full anonymity?), it requires heavy cost for hiding the exchanged asset and is not friendly to the compliance requirement.
Firstly, the private exchange requires proving that the changed balances are correct and fair without leaking their positions.
It usually needs the user to commit on $n$ changed values and prove that only two of them are non-zero and their values are equal according to the public prices.
It implies that the communication cost is at least linear in $n$.
Secondly, it stores the balance of each asset in one credential and treats them as fungible properties.
However, in the exchange setting, the asset binds with a buying price when Alice gets it from deposit or exchange.
It prevents the asset from being accumulated even they are the same name of asset.
%It is used to compute the profit to meet the compliance requirement.
%She needs to compute the profit of each transaction and accumulate them for tax filing.
If we just use such one single credential and append the new asset with price on it, the position naturally leaks the user's transaction times and hiding the changed position is heavy work as we discussed before. 
}
%%%%%%%%%If we just append the transaction records into one credential, the number of transact is restricted and the position of price record leaks extra information such as the number of user's past transactions.

%%%%In first step, when Alice interacts with the platform, she just proves that she is a registered user without showing who she is.
%%%%It can be achieved via anonymous credential.

 
\noindent{\em Supporting compliance.}
The above full anonymity construction is over-simplified, as we have not considered compliance issues. For example, since each user can have multiple credentials, he could give one credential with, say 10 Bitcoins, as a gift to any person, who may not even registered with the platform. 
Then the gift receiver could use the credential to do the anonymous trading with the platform without revealing his real-world identity, which is not compliant even with the basic KYC regulation. Moreover, we would support common compliance goals without hurting anonymity/privacy. 
In particular, we use tax filing as an example of client-compliance. %for our study. 

First, all transactions from the same user should be bind together (without revealing the content) to derive accumulated profit; we thus let each user maintain {one} long-term {\em registration credential} that contains two attributes ``cost'' and ``gain'' to record the buying cost, and selling gain for exchange-out and withdraw transactions (the taxable transactions in e.g., Coinbase). Such a credential is issued when user registered to the system, and will be updated properly after each transaction. To conveniently update it, transaction metadata would also be recorded in a secure way, e.g., each coin type, buying/selling price and amount, etc (as in current exchange platform such as Coinbase). Each transaction corresponds to two one-time {\em asset credentials} w.r.t the exchanged assets which contain the corresponding trading prices and amounts.%to derive 
%An attribute on each {\em asset credential} to store the buying price of the corresponding asset. 

When users request to exchange or withdraw, they need to provide proof of ownership for a valid asset credential with sufficient amounts, a valid registration credential, evidence of fair exchange, and accurate records of updated costs and gains. However, when generating the compliance report, revealing this information directly to the platform would compromise user privacy. For instance, if a user has a substantial profit, it increases the likelihood of being linked to previous large-scale withdrawals. To address it, we employ a workaround by having the platform blindly sign (thus providing validity proof) to generate the report without revealing sensitive information.

%they prove owning a valid asset credential with enough amounts, a valid registration credential, fair exchange, and correct record of ({\em updated}) cost and gain.
%\footnote{As in Footnote.\ref{ucs}, there exists the concept of updatable anonymous credential via general zero-knowledge proofs, but we need to design concrete update functions efficiently.} 
%
%When generating the compliance report, directly revealing information to the platform violates user's privacy. For example, if a user has a large profit, the chances he may be linked with some previous large-size withdraw increases. We get around this by letting the platform blindly sign (providing validity proof) to generate the report.%, and only let external tax authority to check the %, which in turn hurts withdraw anonymity.
%The accumulated profit may leak non-trivial information. For example, a 
%it could rule out sleepy users who did not exchange or withdraw in the past year indicated by the empty compliance information.
%Thus, in our design, users just show its identity and commitment of the profit information to the platform and prove the correctness.
%that it is same with the value in his latest registration record.
%If the platform accepts the proof, it signs blindly.
%After that, the user shows the profit with the platform's unblinded signature to the authority in the tax filing. 






%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
%While all transactions are unlinkable, Alice needs to maintain the compliance information covering all of them.
It is achieved by computing each transaction's compliance information and accumulating them in her registration record. 
Computing an individual compliance information relies on the asset's buying price and current price.  
To comply with the regulation rules, the compliance-related information is included in the asset record.
It is used to compute the cost and gain of each exchange and withdraw transaction (the amount of consumed asset times its buying price and selling price respectively.)  
The accumulated costs and gains are the compliance information shown to the authority for tax filing.
%%%Then they are added on the compliance information of his registration record. 
%is computed correctly based on the old registration record and the current profit.
When filing, the user hides the compliance information but proves that it comes from his \textit{latest} registration record to make sure that it is correct.


In first step, when Alice interacts with the platform, she just proves that she is a registered user without showing who she is.
It can be achieved via anonymous credential.
When Alice joins the system, she gets a registration record issued by the platform.
%maintaining her compliance information.

%Depositing USD is public and the bank account can be linked to Alice due to the KYC requirement, but spending such asset should not be linked to her further.
%To keep anonymous, we follow the e-cash design and generalize it to fit our expressive compliance requirement.

When Alice deposits or exchanges assets, she proves in zero-knowledge the ownership of a registration record. 
The platform issues asset records containing her identity same as that in the registration record and the asset information, such as its name, quantity and trading price.
During exchanging or withdrawing, the user interacts with the platform anonymously by proving the ownership of {\em valid} registration and asset records in zero-knowledge.
It cannot link this with any user or other transactions.
Especially for an exchange transaction, the asset names and amounts are concealed. %and the user proves the validity.

In the filing transaction, directly showing the compliance information to the platform violates user's privacy, which in turn hurts withdraw anonymity.
Since it rules out the sleepy users who did not exchange or withdraw in the past year indicated by the compliance information.
Thus, in our design, Alice just shows her identity and commitments of the profit information to the platform and proves its correctness.
%that it is same with the value in his latest registration record.
If the platform accepts the proof, it signs blindly.
After that, the user shows the profit with the platform's unblinded signature to the authority in the tax filing. 


\fi


\iffalse
The asset contains the following information: user secret key \textit{usk}, identifier \textit{aid}, asset name \textit{i}, amount $k_i$ and compliance-related information $\mathsf{acp}_i$.
To issue the asset record, the platform signs the commitment of them.
When exchanging or withdrawing, Alice proves in zero-knowledge that she owns a valid asset and requests the platform to issue a new record for the same asset with a new identifier and updated amount.
In the exchange, a new asset record with a different asset name is generated which is also hidden from the platform.
Therefore, the platform cannot link any two of the transactions which provides the best possible anonymity set for the withdrawal.

%\iffalse
The deposited and withdrawn assets must be public since the platform is the receiver and sender.
But the exchanged assets inside the platform can be concealed, and the user could also hide his identity when interacts with the platform except depositing fiat money from bank account.
To obtain the best privacy, Alice should hide her information as much as possible. 
%%%%It requires that the platform has no idea about the user's records during the interaction.

%We illustrate it as follows.

%\noindent\textbf{Private interaction.} \ 

When the user joins the system, he provides his real identity and gets a registration record from the platform containing his identity and compliance information.
Thereafter he uses this record to interact with the platform and perform the deposit, exchange, withdraw and signature request transactions.
\fi


%\noindent\textit{Overdraft prevention.} \ 
%Note that each record binds with a unique identifier to prevent double-spending. 
%It is chosen by the user randomly and revealed when it is used. 
%These used records are invalidated and the platform issues new records.


%In withdrawal transactions, the new asset contains the information same with the old one except that the value is deducted by respective amount and a fresh identifier. 
%In exchange transactions, one asset record is used and two new asset records would be issued. One is same with the old except the value gets deducted. The other one denotes the exchanged asset and contains corresponding information. The exchange should be fair which means the value of deducted asset equals to the value of new exchanged. 



\noindent\textit{Practical considerations.} With above considerations, the users and platform have to engage in multiple non-interactive zero-knowledge proofs, some of which may be heavy if not done properly. Particularly, for each exchange transaction (e.g., user wants to buy 1 BTC using 15 ETHs), the user takes his ETH asset certificate, proves in zero-knowledge that the asset type belongs to $[n]$ via a membership proof (as asset type needs to be kept private); and proves the used prices (committed in the new asset certificates) are exactly
the current prices of the exchange-in and exchange-out assets, which also need membership proofs. To facilitate such a proof, one idea is to let the user to commit to a vector $\vec{v}$ with $n$ dimension, and prove that $\vec{v}$ is a vector of bits and contains only one entry (corresponding to his asset certificate) as $1$. Then homomorphically evaluating the linear combinations may get commitments of price$\times$amount of BTC, and ETH respectively, the user can further prove the resulting committed values are equal. The proof size is already at least $O(n)$, and computation cost even more. Recent work of one-out-of-many proof or many-of-many proof may reduce the proof size to logarithmic in $n$ but the computation cost of proof generation and verification is still (super)linear in $n$ \cite{Groth2015, diamond2021manyzether}. 

%Naively applying the best membership proofs via an ``AND'' logic still yields (super)linear communication and computation cost ($O(n\log n)$).

%This proof is the heaviest part as involving .

%Firstly, the user proves the name $i$ of the new asset belongs to $[n]$ via a membership proof (the exchanged assets need to be hidden in all $n$ types. %which involve one membership proof). % which does ( super ) linear computation cost $O(n\log n)$ with the total assets names $n$.
%To guarantee exchange equality, the user should prove the used prices are exactly
%the current prices of the exchange-in and exchange-out assets, which also need membership proofs. 
% with super linear computation cost $nlogn$.
%Then the user stores the price in the asset record which needs additional nontrivial work.

\iffalse
An intuitive idea is that: the user generates $n$ commitments and proves that only the $i$-th committed value is 1 and all others are 0s.
Then multiplying them with respective public prices and adding them together, so the result is a commitment on the price of the $i$-th asset.
They can be proved with logarithmic proof size using one-out-of-many proof, and the generation and verification time are still (super)linear with $n$.
Besides the proofs, the user also needs to send $n$ commitments to the platform for its verification.
So the overall communication cost is linear with $n$.
\fi

Instead, we let the platform generate signatures on each asset name and the price and make them public, called \textit{price credential}.
To capture the price fluctuation and avoid users using out-of-date price credentials, each price credential contains the timestamp of the latest price update. In the exchange transaction, the user proves that the new exchanged asset record contains the name and price and she knows the valid signature on them and the latest timestamp. %, and the exchange is fair according to these prices.
It can be verified by the platform's {\em single} public key, and we can bring down the communication and computation cost to be constant. For details, please refer to Sec. \ref{Pricecredential}.

 \noindent\textbf{Extensions and open questions.} 
For client-compliance, there are many other regulation rules such as limiting the transaction frequency, transaction amounts, all sending or receiving amounts and scrutinizing the receiver addresses in case of financing terrorism. Our techniques can be extended very easily to also support those. See Sec. \ref{construction} for more discussions.
%tian
%Except considering the compliance for users, it is essential for the platform to adhere to regulations. 
%This includes proving its solvency, ensuring that the platform possesses sufficient assets to meet the withdrawal requests of users.


%{\color{red} 
\noindent\textit{Solvency issues.} There are also many platform-compliance requirements. One notable one is the solvency problem that the platform should be able to check it has sufficient reserve. Now, transaction details are hidden in privacy-preserving exchange, which may increase the risk of solvency issues, and users may exchange/withdraw a large amount of certain cryptocurrency privately that exceeds the platform's reserve, thus causing a potential ``bank run''. According to the Basel Accords \cite{Basel} for the banking industry (we also use it as the platform-compliance rule in Sec. \ref{compliance-rule}), it usually requires the banks to  (i) provide sufficient liquidity (e.g., keep enough asset to cover the total withdraws of last month), and (ii) keep a sufficient minimal reserve (e.g., 0-10\% of the total assets held by all users in the platform, in the form of a major currency such as USD~\cite{IMFForeignExchangeReserve}; in our setting, Bitcoin). We show that our Pisces system with full anonymity also satisfies the first platform-compliance requirement. As the platform is still aware of the total amount of incoming/outgoing Bitcoins (and any other cryptocurrency tokens), thus the needed information could still be derived. 

For maintaining a minimal reserve, there might be some practical mitigation, e.g., actively monitoring the total withdrawal amount/pattern for each coin, limiting the exchange and withdrawal amount/frequency, etc, or involving a third-party auditor (similar to the tax authority to keep the aggregated information to manage risks). Those can be supported by extending our design. But a more rigorous solution remains open. Also, there could be even more strict and complicated rules that may require the platform to keep sufficient reserve and liquidity for every single type of coins \cite{BinanceProofofReserve}; or require the platform to generate publicly verifiable proofs of solvency. 

We remark that with our basic anonymity, the platform knows all the holdings of each account (except the link between the inside and external onchain accounts), thus can still derive all needed information for both requirements and the more strict rules.  

However, a more systematic investigation of solvency issues in the fully anonymous setting (e.g., allowing the platform to gain extra side information for solvency purposes) may again have further impact on the anonymity.

%
%We take the requirements of Basel Accords \cite{Basel} 
%It is compatible with our full anonymity setting.


%
As a first step studying privacy in exchange system with efficient compliance support, there are many interesting questions and challenges to explore (e.g., supporting broader compliance rules). 
For a more systematic investigation, we leave them as interesting open problems.
%}
%When he withdraws all that cryptocurrency, the platform cannot afford to pay. 
%\yanan{promise extension.} 


%we believe it is a wonderful open question to explore a more rigorous sophisticated solution.

%We only consider calculating profit and tax filing in our design since they are more complex than others and our construction supports other requirements straightforwardly.
%We just give some sketches due to the page limitation.



%To achieve the basic KYC goal, we introduce a secret attribute (also user secret key, usk for short) to identify registered users uniquely in each credential. And users are issued a credential about usk when they join the system (register). To avoid linking to real identity and previous transactions, users should prove knowledge of the secret key in zero-knowledge. And the credential can only be used when users know the usk embedded in the credential, which means that if one owner gives one credential as a gift, then leaks the secret and lose control of other credentials.  \qiang{above two paras unsure}



\iffalse
The user conducts the following operations: deposit, exchange and withdraw. 
They can achieve the function of buy, sell, exchange and withdraw.
In order to buy cryptocurrency, the user deposits fiat money in his account, then request the platform exchanging fiat money to some cryptocurrency.
If it wants to sell cryptocurrency, he uses similar method by exchanging it to fiat money, then withdraws fiat money to its bank account.
It can also withdraw cryptocurrency to his electronic wallet.
\fi


\iffalse	
\{The user shows $id, upk$ and profit of his latest unspent token, and generates the zero-knowledge proof of the correctness. The issuer checks this information and proof. If it is true, the issuer helps the user to update his token with a new $id$ and marks it as a token that has been revealed profit. It leaks no other information of user except that he has already revealed his profit.
\}

\subsubsection*{Security}

privacy

no privacy: Coinbase knows who selects which bitcoin and traces it on blockchain.
Given an unspent bitcoin sent by Coinbase, it knows the real identity of the current owner.

Unlinkability:
(pseudonym anonymity) exchange only knows someone is withdrawing bitcoin to an address but it does not know the client's real identity.
This is the highest level of anonymity that bitcoin can provide.
Ideally, the company knows each client's real identity, but on the withdraw request, it cannot infer any information of the client except that he has enough money.
Formally speaking, the exchange cannot link withdraw request with any other operations.

double-spending

In the privacy-preserving setting, the client can partially withdraw and sell bitcoin by proving that he has enough money and these requests cannot be linked to his account.
The company does not know the balance of each account.
The client may withdraw all his bitcoin to different address in two requests and it is a double spending.

\fi
	

%To preserve user's privacy, we propose an anonymous exchange scheme leveraging anonymous token from updatable anonymous credentials (UACS)\cite{Blomer2019UpdatableSystems}. 




\iffalse
It is maintained in their account tokens.
When the user exchanges or withdraws cryptocurrency, this information is also updated.
Later, the user requests the platform to sign on his accumulated profit blindly with proof of correctness. 
Thus, it fulfills the compliance requirement without breaking the unlinkability of past transactions.
\fi

\iffalse
\subsection{Related works}

\qiang{extract some part to move earlier to show why our setting is different with all previous private exchanges}

\tian{compare with the accountable work with some auditor, we can extend to that setting easily using an additional encryption layer and zero-knowledge proofs?}

There are some previous works on private exchanges.
However, they suffer from inconvenient usage, transaction linkability and lack of consideration of compliance issues.
A private fiat-to-Bitcoin exchange scheme is proposed in \cite{yi2019new}. 
The user buys cryptocurrency with fixed denomination from an exchange platform who cannot recognize the linkage between his identity and the Bitcoin address. 
%But each purchase binds with fixed domination like 1 Bitcoin which is inconvenient for users. 
%%There are some works on {private exchange} in the decentralized setting like P2DEX \cite{Baum2021P2DEXExchange} and Manta \cite{chu_manta_nodate}, but they do not consider the compliance issue. The users do not need to provide their real identities or comply with any regulation rules.
P2DEX \cite{Baum2021P2DEXExchange} is a privacy preserving exchange system for cryptocurrency tokens cross different blockchains. 
It preserves order privacy to avoid front-running attack and ensuring users never lose tokens.
It focuses in the transaction confidentiality rather than user anonymity.
Manta \cite{chu_manta_nodate} is a decentralized anonymous exchange scheme based on AMM.
It converts some base coins to private coins via a mint mechanism, then achieves anonymous exchange by trading private coins without compliance guarantee.

Besides the private exchange, there are some other related works in accountable privacy.
But they only focus in the payment system and enforce limits on transaction value and sum of all sent or received values.
%(Enforcing limits on transaction value and sum of all sent values are two general regulatory rules.)
Note that this compliance information update only involves the current transaction value. 
But we consider some more general cases in which updating compliance information may require any past transactions and take the profit computation as an example.
Each profit is computed based on the buying prices from past transactions and it is accumulated with the past profits as the final value.

\noindent{\bf Fiat to cryptocurrency (F2C) exchange.} \ 
In general, the centralized F2C exchange platform does not consider user's privacy, like Coinbase, Binance.
They collect user's personal information when they register to meet the KYC requirement.
However, the user's accounts are transparent for the platform.
It knows their asset profile, i.e., which names and how many assets they own.
In the case of cryptocurrency, it would also know how the user spend their cryptocurrency which violates user's privacy outsides the platform.

A privacy-preserving  fiat-to-Bitcoin exchange scheme is proposed in \cite{yi2019new}. 
The user purchases a fixed amount of cryptocurrency from an exchange platform by fiat money but the platform cannot recognize the linkage between its real identity and its Bitcoin address. 
%It is not possible to have atomic swap since a fiat money transaction is needed.
They use a blind signature to receive Bitcoin from the platform while hiding the output address of that transaction. 
Eventually, this transaction will be put onto the Bitcoin blockchain which reveals the output address, the transaction amount and the UTXO used by the platform at that time.

To prevent the linkability by the transaction amount, the amount of withdrawn cryptocurrency is fixed for all transactions. 
For example, let all transactions worth 1 Bitcoin.
To prevent the linkability by the input UTXO, %it cannot be selected by the platform.  
%For each request from the client,
%If the UTXO is chosen by the exchange platform, it can identify it when the client post the transaction (input UTXO, output address) on the blockchain and link the client's address with his identity via that UTXO.
it should be chosen by the client.
But two clients may choose the same UTXO and the conflict leads to only one of them would receive the bitcoin.
Besides, it is not accountable. 
The users do not need to provide any compliance information, otherwise their privacy cannot be preserved. 

%[\textbf{buy with cash}] 
There are also some service for purchasing cryptocurrencies with cash, e.g. Bitcoin ATM. 
Users receive Bitcoins anonymously since the cash is untraceable, but such service is not secure or can be used for crime.[https://www.cnbc.com/2021/11/09/bitcoin-atms-criminals-target-cryptocurrency-transactions.html]

%\paragraph{
\noindent\textbf{Decentralized exchange platform (DEX).}   
There are some work on decentralized exchange where users exchange cryptocurrencies with each other directly or with smart contract.
However, it is very different from our setting.
It does not support fiat money transactions and they are generally deployed in the decentralized setting like smart contract that is unaffected by the KYC requirement.
Users are free to join the DEX without providing their real identities as long as they have cryptocurrencies.
It is hard to directly enforce compliance requirement on it since the enrollment does not require real-world identities. 
Uniswap \cite{uniswap} implements an ordinary constant product automated market maker (AMM) with smart contract. 
It is an algorithm for trading two fungible tokens on the same chain.
Another alternative technique is to leverage trusted execution environments (TEE), e.g. Intel SGX \cite{sgx}. 
%Teechain [47] and Teechan [48] synchronize payments across channels using TEEs. 
%TEE enable expressive and off-chain smart contracts on restricted Bitcoin-based blockchain [49]. 
For example, Tesseract \cite{bentov_tesseract_2019} proposes a scalable cryptocurrency exchange using TEE that supports cross-chain exchange.

There are also some works on the {private exchange} in the decentralized setting like P2DEX \cite{Baum2021P2DEXExchange} and Manta \cite{chu_manta_nodate}, but they do not consider any compliance issue.
P2DEX \cite{Baum2021P2DEXExchange} is a privacy preserving exchange system for cryptocurrency tokens cross different blockchains while preserving order privacy to avoid front-running attack and ensuring users never lose tokens.
They use MPC for privately matching exchange orders and deploy smart contract to reimburse affected clients with the collateral deposit from the cheating server.
Manta \cite{chu_manta_nodate} is a decentralized anonymous exchange scheme based on AMM.
Firstly, they design a mint mechanism to convert base coins to private coins. Then they achieve the decentralized anonymous exchange by trading private coins anonymously.

%\paragraph{\bf Accountable privacy.}
\noindent\textbf{Accountable privacy.} 
There are some works in studying to achieve privacy-preserving and accountability at the same time.

(Bifurcated anonymous signatures allow to bifurcate into absolute anonymity and identity escrow at the signing time, where computing signatures is associated with a predicate P. 
Whether a signature is traceable by an authority or not depends on the content that being signed and the user's identity. 
\tian{is it related?})
%Since users know the predicate and its value before signing, they know beforehand when they will be subject to tracing and they can make an educated decision as to whether they can afford to sign a specific message or not.

Androulaki et al present a privacy-preserving token payment system for permissioned blockchains that with auditing.
The content of transactions is concealed and only some authorized parties can inspect them.

Untraceable transactions (UTT) is a Ecash-like payment system. 
It provides accountable privacy by implementing anonymous budgets.
Senders can generate payments anonymously within a limited amount of money per month. 
After that, their transactions have to be public to the authority.


%\paragraph{\bf Private cryptocurrencies.}
\noindent\textbf{Private cryptocurrencies.} 
There are two popular types of transaction models in today’s blockchain networks. The first method is called the UTXO (Unspent Transaction Output) model (e.g. Bitcoin), and the other is account model (e.g. Ethereum). 


To keep the sender anonymous in the UTXO model, one can either hide him in a subset of other users (called anonymity set in Monero \cite{monero}) or store all outputs in a Merkle tree (like in Zcash \cite{zcash,zerocash}) so that one can prove the knowledge of an output by providing a zero-knowledge proof of a Merkle opening using zkSNARKs or other techniques. 


For account-based currencies, it is difficult to hide the sender or receiver, since the change of balance is obvious and indicates who are involved into the transaction. 
Thus, it seems necessary to change every user’s account balance in some anonymity set. However, it may render other users’ transactions invalid. 
The anonymous version of Zether \cite{Bunz2019} handles this issue by restricting users generate only one transaction in a specific time period.

 
\noindent{\bf Private layer 2 solutions.}
%TumblerBit, Coinjoin, Coinmixer.
%These solutions need introducing some third party and users need to wait long enough and pay additional fees for the service.
In the off-chain setting, many solutions have been proposed. 
They perform as opt-in tools that enhance privacy for existing cryptocurrencies.
They aim to prevent an adversary from linking a payment from a particular payer to a particular payee.


Bolt \cite{green_bolt_2017} is an anonymous payment channel was introduced by Green and Miers.
It aims to offer privacy-preserving payment channels such that multiple payments on a single channel are unlinkable to each other. 
Assuming the funded cryptocurrency is anonymous (e.g. Zerocash), the payments in Bolt are also anonymous.


TumbleBit \cite{heilman_tumblebit_2017} is a unidirectional payment channel hub (PCH) relying on an untrusted intermediary called Tumbler and Hashed Timelock Contracts (HTLCs). 
The Tumbler issues anonymous payments that users can cash-out to Bitcoins. 
Every payment made via TumbleBit is backed by Bitcoins and nobody can link any pair of them. 
It is also guaranteed that the Tumbler can neither violate anonymity, nor steal bitcoins, nor issue payments to itself.


Anonymous atomic locks (A2L) is introduced in \cite{tairi_2_2021} where the authors propose a payment channel hub (PCH) upon it. 
This PCH is a three-party protocol for conditional transactions, where the intermediary (called hub) pays the receiver only if the latter solves a puzzle with the help of the sender.
It means the hub has been paid by the sender.
Due to the puzzle is randomizable, the sender and receiver in a payment cannot be linked by the hub.


LDSP \cite{ng_ldsp_2021} is a layer-2 cryptocurrency payment system that supports payer privacy.
It is designed in the setting of shopping with cryptocurrency where the payer is customer and the receiver is merchant.
There is also an untrusted entity called leader who is in charge of issuing coins for customers and merchants.
Customers can transfer coins off-chain with low-latency.
Since the coins are issued in a blind way, the leader cannot link the spent coin with any customer.
On the other hand, the merchants will receive the coins.

There are also some off-chain works such as Plasma \cite{Poon2017Plasma:Contracts}, NOCUST [21], ZK-Rollup \cite{gluchowski_zk_nodate}. 
They aim to improve the scalability of blockchain by moving the expensive computation and redundant data off-chain via an untrusted operator.
In order to build privacy on these scaling solutions, PriBank \cite{galbraith_pribank_2022} is proposed with an efficient Commit-and-Prove NIZK protocol for quadratic arithmetic program.
The users’ balances and transaction values are kept private from other entities except the operator. 
The operator is not trusted to execute honestly but is trusted for confidentiality.






\iffalse
Unlinkable HTLC [117], is a cryptographic primitive that ensures that a HTLC in a payment path is built upon a different and unrelated hash value. 
Rayo and Fulgor achieve the same functionality as HTLC but prevent linkability of payments.

Unlike Rayo and Fulgor, AMHL protocol embeds the synchronization condition within a public key, improving upon Rayo and Fulgor on efficiency and privacy (i.e. the synchronization condition does not explictly appears on the transaction).
\fi


\noindent\textbf{Exchange platform compliance.} 
%\paragraph{\bf Exchange platform compliance.} 
Provisions \cite{Benedikt2003ProVISION} is a privacy-preserving proof of solvency whereby an exchange does not have to disclose its Bitcoin addresses; total holdings or liabilities; or any information about its customers.
The proof of solvency means the exchange platform proves it has enough cryptocurrencies to settle each customer’s account.
A proof of solvency consists of two components. In the first, the proof of liabilities, the exchange commits to the total quantity of bitcoin it owes to all of its users. 
In the second, the proof of assets, the exchange commits to the total value of bitcoin it has signing authority over. If the latter committed value is greater than or equal to the former, the exchange is considered solvent.

%It is out of scope of/orthogonal to our work.
\fi


%\subsection{Paper organization}
%\paragraph{\bf Paper organization}

\ignore{%%%%%
\noindent\textbf{Paper organization.} In the next section, we introduce the notations and some basic cryptographic primitives.
In Section 3, we formalize the syntax of a private exchange system with compliance and its security model.
In Section 4, we first give a basic model of withdraw anonymity with a construction and discuss their shortage for warm up.
%from single-use anonymous credential, but its anonymity set is limited and the compliance information only relates to the activities of real name account, then we discuss the difficulty of defining stronger anonymity: failed definition and artificial modification.
Then we define the full anonymity model with enlarged anonymity set.
%where the capable users are indistinguishable from the incapable users. 
%(2) to achieve it and better/perfect compliance, we need more advanced tools: uac with fairness proof. (3) 
In Section 5, we give a construction where the compliance information is profit and prove its security.
In the end, we provide the performance evaluations.
}%%%%%

\iffalse
\paragraph{\bf Efficiency considerations.} 	
{All the ZK proofs can be efficiently instantiated, in particular, we can use the randomizable signature scheme by Pointcheval and Sanders \cite{Pointcheval2016ShortSignatures} and Schnorr zero-knowledge proofs. }
	
{The user hides his secret message using Pederson commitment and generates the Schnorr style's proof of knowledge. The issuer produces the PS signature on the commitment which can be converted to a signature on the original message by the user. The message and the signature form user's token.
		
In the Deposit operation, the user needs to prove that he has a valid token by proving the ownership of such a message-signature pair without showing them. This can be done by randomizing this PS signature and prove the knowledge of the message with Schnorr's method.
In the exchange or withdraw operation, the user additionally shows his token's $id$ to prove this token is unspent. He also needs to prove $v\geq k$ by generating a range proof on $v$.
When the user reveals his compliance information, he also generates the proof of correctness. Here we use the Schnorr zero-knowledge proof too.}

\fi


==> 5fullcopy.tex <==
\section{Private and Compliable Exchange System}
\label{construction_system}
%\vspace{-0.3cm}
%\tian{briefly describe the overflow, then explain how these records issued and used unlinkably } 

In this section, we present the generic construction of the private and compliable exchange system $\Pi_{\mathsf{\name}}$ that achieves full anonymity, overdraft prevention, and compliance, and we provide formal proofs of its security.
Before that, we give concrete compliance rules that our system aims to comply with for both clients and the platform. % the clients and platform that our system aims to comply.
Following that, we introduce the concept of price credentials and illustrate the high-level idea about the construction.%It works as the specific data structure for asset price so that our scheme can be instantiated via efficient zero-knowledge proofs. \yanan{price credential is not very clear? It is issued by the platform on the current price of an asset and some metadata, which are organized with a specific data structure. So that users could anonymously and privately convince the platform the used price is correct.} %(\textbf{recall intro to highlight})
%At a high-level, our system is a combination of the e-cash design with the account model.
%


\noindent{\em Concrete compliance rules.} \label{compliance-rule}
\tian{define F,G compliance here}
%It is achieved via commitment, blind signature, and zero-knowledge proof.
For F-client-compliance, we take the tax report as an example of rule F, called tax-report-client-compliance. It requires clients to report the accumulated investment profit (gain minus cost) yearly. Concretely, the taxable profit is calculated and accumulated when clients sell their assets via exchange and withdraw transactions. %each exchange and withdraw transaction occurring during the tax period is a taxable transaction. 
The profit equals the selling value of exchange-out or withdrawn assets minus its buying cost.  Our idea to achieve tax-report-client-compliance is recording the buying price of flow-in assets to the unspent asset credential in the deposit and exchange transactions, calculating the profit when selling assets to the platform in exchange and withdraw transactions, and accumulating the profit to the user registration credential as the taxable profit. Considering the privacy setting, some operations such as calculating profit, recording the price of exchange transactions, etc, will be conducted in a zero-knowledge way, detailed in construction~\ref{construction}.
% %Note that the asset binds with additional compliance property. 
% The compliance-related information of an asset is its buying price when the user obtains it from deposit or exchange, denoted by $\mathit{acp}=px_i$. The user computes the cost and gain of each exchange and withdraw transaction as the buying value $px_i\cdot k_i$ and selling value $\overline{px}_i\cdot k_i$, where $\overline{px}_i$ is the asset $i$'s current (selling) price. Then he reports the accumulated cost $\mathit{cp}_1=\sum \mathit{px_i}\cdot\mathit{k_i}$ and gain $\mathit{cp}_1=\sum \overline{px}_i\cdot\mathit{k_i}$ to the authority at the end of the financial year.
% %We say that a system has tax-report-client-compliance property if all users have to report the correct accumulated cost and gain.

%tian revise
For G-platform-compliance, we refer to the rules of Basel Accords \cite{Basel}, a series of banking regulations established by representatives from major global financial centers. 
It mandates that banks maintain a minimal reserve (10\% of total assets, MR for short), and an appropriate liquidity coverage ratio (LCR), which is to hold sufficient cash and liquid assets to cover fund outflows for 30 days. 
The total reserve value can be decided based on the public net inflow of all assets and converted to amounts of BTCs.  
The platform always knows clearly the inflows/outflows for each coin including fiat money transfers (as the platform receives or transfers them out). 
Thus this MR-LCR-platform-compliance is compatible with our fully anonymous setting.






\noindent\textit{{About price credential and price fluctuation.}}\label{Pricecredential} 
To achieve efficient private exchange with compliance, we introduce {price credentials}.
Each price credential is signed by the platform on the current time, the coin kind, and the corresponding current price. To tackle price fluctuation without leaking coin information, the platform keeps signing the latest prices for all coins at the same timestamp.
%In the exchange transaction, the user proves that the new exchanged asset record contains the kind and price and he knows the price credential (valid signature) on them with the latest timestamp and the exchange is fair according to these prices and amounts. In this way, the platform maintains the latest price credentials for all users, and the user only needs to prove using a single latest price credential, which breaks down the communication and computation cost to constant and is more efficient than the case that the user commits all latest prices and prove using one of them via a membership proof taking linear computation and sublinear communication cost. 
In the exchange transaction, the user proves that the newly exchanged asset record contains the type and price, and they know a valid signature on these values from the latest timestamp's price credential. The user also ensures that the exchange is fair based on these prices and quantities. This approach allows the platform to maintain the latest price credentials for all users, while the user only needs to prove using a single latest price credential. This significantly reduces communication and computation costs to a constant, making it more efficient compared to committing all the latest prices and proving using a membership proof, which entails linear computation and sublinear communication costs.
%It can be verified by the platform’s single public key, and we bring down the communication and computation cost to be constant.
%so that platform cannot get coin information from the timestamp.


%\tian{move high-level illustration in Appendix X back to Sec VI.}

\noindent\textit{{High-level idea.}}
Before giving the formal algorithms, let us illustrate the high-level construction idea with five concrete transaction examples in the following. 
The platform only knows some public information, like all registered users and their bank accounts, the kind and amount of deposited and withdrawn assets, as shown in Fig.\ref{view}. 

%We use Fig. \ref{view} to present the platform's view during the above interactions. 
%In summary, the platform only knows some public information, like all registered users and their bank accounts, deposited and withdrawn assets.

\begin{figure}[!htbp] 
\centering 
\includegraphics[width=1.05\linewidth, height= 0.35\linewidth]{view.png} 
%%%\captionsetup{font={small,rm,stretch=0.9}} %justification=raggedright}
\caption{Platform's view in the exchange system}
%: it only knows the public information, like all registered users and their bank accounts, deposited and withdrawn assets}
%\vspace{-0.4cm}
\label{view} 
\end{figure}

%\medskip
%\noindent{\bf Concrete example.} Here we give a concrete example for illustration.
\setlist{nolistsep}
\begin{itemize}[noitemsep,leftmargin=*]
    \item When deposit 1000 USD, the bank account leaks Alice's identity. Then Alice gets
    %needs to get a receipt of 1000 USD from the platform for spending later. Technically, the receipt is 
    an asset credential or signature generated by the platform.  
    %If it only includes 1000 USD, the platform can sign the plain message directly. 
    %But the signed message should include more attributes 
    To avoid double-spending and be compliant with regulations, the signed message should include more attributes besides the asset details. 
    One attribute is a unique identifier of the credential so that it can only use once. The compliance requires that assets can only be spent by the owner registered within the system. To ensure that only Alice could use the credential later, another signed attribute is Alice's private key bonded with her registered public key. These two attributes should be hidden from the platform to keep the user anonymous, so the platform signs a blind signature. %The attributes are hidden. %via commitment. 
    Alice is required to prove in zero-knowledge that the blinded private key is equal to that in her registration credential.
    To meet tax-report-client-compliance, the profit of selling assets in exchange and withdraw transactions need to be recorded in the registration credential. This necessitates including the exact cost of the assets when they were purchased in deposit and exchange transactions. As a result, we introduce the buying price as an additional attribute in asset credentials when users buy assets, including both deposited and exchanged-in assets.% which needs the exact cost when the assets were bought in the deposit and exchange transactions. 
    %Here we take tax reporting as the main client-compliance regulation. The profit of each transaction should be recorded for users. 
    %We add the buying price as one more attribute of asset credentials when users buy assets including deposited assets and exchanged-in assets. 
    %For the same purpose, Alice could prove the blind private key is consistent with her registration credential. 
%    \item when deposit 10 BTC, the only difference from a fiat deposit is that the platform does not know Bob's identity or his registered public key. Bob is required to prove that he owns a valid registration credential where the private key attribute is equal to the blind private key to be signed as the asset credential. 
    %\item When exchanges 800 USD to 0.5 BTC, Alice requests the platform to issue new registration record with accumulated cost and gain, and two new asset records for the remaining 200 USD and 0.5 BTC where these kinds and amounts are concealed. 
    \item When exchanges 800 USD to 0.5 BTC, Alice shows an asset credential with enough USD which will be revoked and requests the platform to issue two new asset credentials for the remaining USD and 0.5 BTC where these kinds and amounts are concealed. The request is hidden via commitment and the platform signs in a blind way on condition that Alice generates a range proof to show enough USD, and several equality proofs to show  credentials share the same private key, the remaining quantity of USD equals the original minus the deducted, the price of the exchanged-in asset (BTC) equals its current price in the latest price credential, %~\ref{Pricecredential}, 
    and the total exchange value (quantity times price) is equal. 
    
    We give each asset one separate asset credential for practicality especially with compliance. Intuitively, if all assets are in one credential their attributes would increase linearly with the asset kinds. When taking compliance into consideration, it would be worse since each transaction for each asset should be recorded which means the number of the credential attributes keeps increasing like transaction records. It is practical to separate each transaction asset, then the question is it is hard to collect all transactions to calculate the total profit. We solve it by accumulating profit for each selling transaction involving exchanged-out assets and withdrawn assets, and recording it on users' exclusive credentials the registration credential as two attributes: accumulated cost and accumulated gain. Concretely, Alice shows the registration credential which will be revoked, and requests the platform to issue a new registration credential on a new index, updated cost, and gain on condition that the updated cost and gain are consistent with real cost (quantity times buying price) and gain (quantity times selling price). Fiat money is stable so we set its price as 1. 
    %Even though there is no profit from selling the bought fiat money, 
    We treat fiat money in the same way as coins so that the platform does not know whether the exchange involves fiat money. 
    
    %new registration record with accumulated cost and gain, and two new asset records for the remaining 200 USD and 0.5 BTC She proves that 
    %(i) she owns a valid registration record and an (old) asset record with the same identity; 
    %(ii) one of the new asset record shares the same user identity, asset kind and price with the old asset record and its amount is non-negative; 
    %(iii) the other new asset record has the same user identity and new asset kind, non-negative amount and correct price corresponding to new asset kind; 
    %(iv) the sum of the values of two new assets is equal to the value of that old asset;
    %(v) the new registration record has the same identity and the cost and gain are credited correctly.
    
    %by the amount of the exchanged asset times its past buying price and current price respectively.
    %the balance of USD is deducted by 800 and the balance of BTC gets credited by 0.5. 
    %These kinds and amounts are concealed.
    %Alice proves that she has enough asset to deduct and the credited amount is correct with respect to the exchange price.
    
    %\item When withdraws 0.3 BTC, Alice requests the platform to issue a new registration record with accumulated cost and gain, and a new asset record for the remaining 0.2 BTC, only hiding the amount. She proves that 
    %(i) she owns a valid registration record and a BTC asset record with the same identity; 
    %(ii) the new BTC record shares the same identity and price with the old one and its amount is non-negative; 
    %(iii) the new registration record has the same identity, and the cost and gain are accumulated correctly.
    %by the value of the withdrawn BTC with respect to its past buying price and current price. 
    \item When withdraw 0.3 BTC, it is similar to the exchange operation, except for the exchanged-in asset. Alice also verifies the receipt of the withdrawn BTC on the blockchain.%Additionally, Alice checks she has really received the withdrawn BTC on the chain .
    %\item When files her profit: all cost 480 and all gain 600,  Alice commits to these values and requests the platform to
    %sign on them with her identity and issue a new registration record. She proves that (i) she owns a valid registration record with values equal to those in the commitment; (ii) the new registration record contains the same identity with zero values. 
    \item When file profit: all cost 480 and all gain 600,  Alice shows a valid registration credential with her identity, and requests an updated registration credential with a new index, reset cost 0  and reset gain 0, and a file credential used to show to the regulatory authority. The file credential should contain Alice's real identity, the correct cost and gain, and some regulatory auxiliary information. Since the cost and gain are hidden from the platform to avoid information leakage, Alice should prove the committed cost and gain are equal to the ones in her registration credential, and the platform signs blindly. Alice will deblind it and submit the message signature pair to the authority for tax report.
    %they are equal to those in her latest registration record and request the platform to sign on them with her identity
\end{itemize}

%\fi




\vspace{-0.2cm}	
\subsection{An efficient $\mathsf{\name}$\ construction}
\label{construction}
In this section, we give an efficient $\mathsf{\name}$ construction from additive homomorphic commitment, blind signature and zero-knowledge proof\footnote{Note that these primitives are also used for updatable anonymous credentials and an incentive system in \cite{blomer_updatable_2019}. As we explain in detail in App.\ref{IncentiveSystem}, they do not support the exchange operation and compliance rule in our setting.}. 
A concrete and efficient instantiation is presented in section~\ref{instantiaction}. 
Let $\mathsf{Com}$ be an additively homomorphic commitment scheme, $\Pi_{\mathrm{bs}}=(\mathsf{KeyGen}$,$\mathsf{Com}$, $ \langle\mathsf{BlindSign}, \mathsf{BlindRcv}\rangle,\mathsf{Vrfy})$ be a blind signature scheme and $\mathsf{ZKAoK}$ is the underlying proof system. 
The platform maintains the registered user set $\mathsf{UPK}$ and the identifier set $\mathsf{ID}$ which are initially empty.
Formal construction is in Fig~\ref{scheme}.

\begin{figure*}[!htbp] 
\centering 
\includegraphics[width=1\linewidth, height= 1.2\linewidth,frame]{pages.pdf} 
%%\captionsetup{font={small,rm,stretch=0.9}} %justification=raggedright}
\caption{Our efficient construction of Pisces}
%: it only knows the public information, like all registered users and their bank accounts, deposited and withdrawn assets}
%\vspace{-0.4cm}
\label{scheme} 
\end{figure*}

%%%%%%%%%%%%%%%%%scheme%%%%%%%%%%%%%
\iffalse
%\newpage
%a
%\newpage

%(\mathsf{KeyGen}_{\mathrm{bs}}, \mathsf{Commit}_{\mathrm{bs}}, \mathsf{BlindSign}_{\mathrm{bs}}, \mathsf{BlindRcv}_{\mathrm{bs}}$, $\mathsf{Vrfy}_{\mathrm{bs}})$ be a blind signature scheme.

\iffalse
Let $\Pi_{\textrm{ouac}}=(\mathsf{Setup}_{\mathrm{ouac}},\mathsf{IssuerKeyGen}_{\mathrm{ouac}},
\langle\mathsf{Issue}_{\mathrm{ouac}},\mathsf{Receive}_{\mathrm{ouac}}\rangle,\langle\mathsf{Update}_{\mathrm{ouac}},\newline\mathsf{UpdRcv}_{\mathrm{ouac}}\rangle,\langle\mathsf{ShowPrv}_{\mathrm{ouac}},\mathsf{ShowVrfy}_{\mathrm{ouac}}\rangle)$ be an oblivious updatable anonymous credential system scheme.
$\Pi_{\mathrm{bs}}=(\mathsf{KeyGen}_{\mathrm{bs}}, \mathsf{Commit}_{\mathrm{bs}}, \mathsf{BlindSign}_{\mathrm{bs}}, \mathsf{BlindRcv}_{\mathrm{bs}}, \mathsf{Vrfy}_{\mathrm{bs}})$ is a blind signature scheme. 

\fi

%$\Pi_{\mathrm{sig}}=(\mathsf{KeyGen}_{\mathrm{sig}}, \mathsf{Sign}_{\mathrm{sig}}, \mathsf{Vrfy}_{\mathrm{sig}})$ is a digital signature scheme.


%\iffalse
	
%\medskip
%\noindent\textbf{Note}: Here we note that Sell and Withdraw operations are similar except that the user provides bank account and bitcoin address accordingly. So in the protocol description, we merge them into a single Spend operation. 
	
	
%\medskip
%Let $\Pi_{\textrm{bs}}=(\mathsf{KeyGen}_{\mathrm{bs}}, \mathsf{Commit}_{\mathrm{bs}}, \mathsf{BlindSign}_{\mathrm{bs}},\mathsf{BlindRcv}_{\mathrm{bs}},\mathsf{Vrfy}_{\mathrm{bs}})$ be a blind signature scheme. \\
\setlist{nolistsep}
\begin{itemize}[noitemsep,leftmargin=*]
    \item \noindent $\mathsf{Setup}(1^\lambda)\rightarrow epp$: This algorithm is to generate exchange system public parameters $epp$ that contains the blind signature public parameter $pp$ and the total assets kinds $n$ where $i\in[n]$ denotes the $i$-th asset. 
    It specifies the maximum balance $v_{max}$ of each kind of assets, where $v_{max}=p-1$ 
    %when we assume that the attribute space $\mathbb{A}=\mathbb{Z}_p$ 
    for some super-poly $p$.
    It also includes the public price tokens $\mathsf{px}(i)$ for each asset \textit{i}. %that would be used in each record. 
    %the $\mathsf{UAC}$ credential public parameter from $\textit{cp}p\leftarrow \mathsf{Setup}_{\mathrm{uac}}(1^\lambda)$. 
    

%$epp$ also contains the compliance function $f(\mathsf{operation}, \textit{token}, \textit{record}, \textit{tx})$ for different operations, where $\mathsf{operation}\in\{\mathsf{Exchange},\mathsf{Withdraw},\mathsf{File}\}$, 
%\textit{token} and \textit{record} denote the involved $\mathsf{UAC}$ tokens, and \textit{tx} denotes the transaction information.



    \item \noindent$\mathsf{PKeyGen}(epp)\rightarrow (pk,sk)$:
    The platform  generates a key pair $(pk, sk) \leftarrow \mathsf{KeyGen}(1^{\lambda})$, and initializes the registered user set $\mathsf{UPK}=\emptyset$, the identifier set $\mathsf{ID}=\emptyset$. 

    \item \noindent$\mathsf{UserKeyGen}(epp)\rightarrow (upk,usk)$:
    The user generates a key pair $(upk, usk)$   %$\leftarrow \mathsf{KeyGen}(epp)$, which is simply an encryption key pair, i.e., $usk \leftarrow \mathsf{KeyGen}_{enc}(epp)$ and 
    where $upk=\mathsf{ComputePK}(epp,usk)$. 
    %which is used to identify the user.

\iffalse
\item \noindent$\mathsf{RdReg} \leftarrow\langle\mathsf{Join}(epp,pk,usk,\mathsf{ReqJoi}), \mathsf{Issue}(epp,pk,sk)\rangle\rightarrow b$: 
The user sends its join request $\mathsf{ReqJoi}=(Join, upk)$ to the platform. 
The platform checks: if $upk\in\mathsf{UPK}$, outputs $b=0$ and aborts. 
Otherwise, the two parties run
$ \textit{cred}\leftarrow\mathsf{Receive}_{\mathrm{uac}}(\textit{cp}p,pk,\psi,\alpha)\leftrightarrow \mathsf{Issue}_{\mathrm{uac}}(\textit{cp}p,pk,\psi,sk)\rightarrow b$.
The hidden parameter $\alpha=(usk, id)$ where the identifier \textit{id} is chosen randomly from $\mathbb{Z}_p$, and the update function $\psi$ is 
$$\psi(\bot,\alpha) = \begin{cases}
(usk, id, \textit{cp}_1, \textit{cp}_2), \ \mathrm{if} \ \psi_{chk}  \\
\bot, \ \mathrm{otherwise} \\
\end{cases}$$
where $\psi_{chk}$ is true if and only if
\begin{itemize}
    \item The user's secret in the attributes/credential is matched with the user's public key, i.e., $upk=\mathsf{ComputePK}(epp, usk)$;
    \item there is an identifier $id$ in the attributes/credential;
    \item the compliance information is initialized as $\textit{cp}_1=0, \textit{cp}_2=0$.
\end{itemize}

If $b=1$, the platform adds $upk$ to the set $\mathsf{UPK}$, and the user outputs  $\mathsf{RdReg}=(usk,id,\textit{cp}_1, \textit{cp}_2,cred)$ consists of its initial compliance information ${\textit{cp}}_1=\textit{cp}_2={0}$ and a credential \textit{cred} on the attributes $(usk, id, {\textit{cp}}_1, \textit{cp}_2)$. 
%This \textit{token} is set to be the user's register record $Rd_{reg}$.

\tian{no uac, just blind signature and nizk}
\fi

\item \noindent$\mathsf{RdReg} \leftarrow\langle\mathsf{Join}(epp,pk,usk,\mathsf{ReqJoi}), \mathsf{Issue}(epp,pk,sk)\rangle$ $\rightarrow b$: 
The user's join request is $\mathsf{ReqJoi}=(\textit{join}, upk)$. 
He chooses randomness $rid, r\sample\mathbb{Z}_P$ and produces the commitment $com=\mathsf{Com}(usk, rid, \textit{cp}_1, \textit{cp}_2; r)$ with the zero-knowledge proof $\pi$: %proving that:
\setlist{nolistsep}
\begin{itemize}[noitemsep,leftmargin=*]
    \item %the $usk$ in $com$ is matched with the user's public key, i.e., 
    $upk=\mathsf{ComputePK}(epp, usk)$;
    \item there is an identifier $rid$ in $com$;
    \item %the compliance information is initialized as 
    $com$ contains
    $(\textit{cp}_1, \textit{cp}_2)=(0,0)$.
\end{itemize}

\iffalse
%\begin{itemize}
%    \item 
\noindent $\mathbf{-}$ The $usk$ in $com$ is matched with the user's public key, i.e., $upk=\mathsf{ComputePK}(epp, usk)$;\\
%    \item 
\noindent $-$ there is an identifier $id$ in $com$;\\
%    \item 
\noindent $-$ the compliance information is initialized as $\textit{cp}_1=0, \textit{cp}_2=0$.
%\end{itemize}
\fi

The user sends $(\mathsf{ReqJoi}, com, \pi)$ to the platform. 
It checks: if $upk\in\mathsf{UPK}$ or the proof $\pi$ is invalid, outputs $b=0$ and aborts. 
Otherwise, the platform adds $upk$ to $\mathsf{UPK}$, and replies with $\hat{\sigma}_{\textit{reg}}\leftarrow\mathsf{BlindSig}(pp, pk, sk,com)$. 
The user unblinds $\hat{\sigma}_{\textit{reg}}$ and gets 
$\sigma_{\textit{reg}}\leftarrow\mathsf{BlindRcv}(pp,pk,\hat{\sigma},r)$ and outputs  $\mathsf{RdReg}=(usk,rid,\textit{cp}_1, \textit{cp}_2,$ $\sigma_{\textit{reg}})$ if $\mathsf{Vrfy}(pp, pk, (usk,rid,\textit{cp}_1, \textit{cp}_2),$ $ \sigma_{\textit{reg}})=1$. 
%consists of its initial compliance information ${\textit{cp}}_1=\textit{cp}_2={0}$ and a signature $\sigma$ on $(usk, id, {\textit{cp}}_1, \textit{cp}_2)$. 



\iffalse

\item \noindent$Rd_{dep}\leftarrow\langle\mathsf{Deposit}(epp,pk,upk,usk,\{Rd\},\mathsf{ReqDep}), \mathsf{Credit}(epp,pk,sk)\rangle\rightarrow b$: 
The user sends a deposit request $req_{dep} = (Deposit, i, k_i, px_i)$ on asset $i$ with amount $k_i$, and price $px_i$.  
The input record set $\{Rd\}$ only has his register record $\mathsf{RdReg}=(usk, rid, \textit{cp}_1, \textit{cp}_2, \sigma_{reg})$. 

The platform checks that the amount of the received asset $i$ is equal to $k_i$ and $px_i$ is the current price according to the $epp$. 
If the check does not pass, the platform outputs $b=0$ and aborts. 
Then the two parties run\\ $\mathsf{RdAsset}_i\leftarrow\mathsf{Receive}_{\mathrm{uacs}}(\textit{cp}p,pk,\psi,\alpha)\leftrightarrow \mathsf{Issue}_{\mathrm{uacs}}(\textit{cp}p,pk,\psi,sk)\rightarrow b$.

The deposit asset information is public.
The hidden parameter $\alpha=(usk, aid)$.
$$\psi(\bot,\alpha) = \begin{cases}
(usk, aid, i, k_i, px_i), \ \mathrm{if} \ \psi_{chk}  \\
\bot, \ \mathrm{otherwise} \\
\end{cases}$$
$\psi_{chk}$ is true if and only if
\begin{itemize}
    \item there is a new identifier $aid$ in the new record;
    \item the new record contains the correct deposit information including the kind $i$, amount $k_i$ and price $px_i$;
    \item the new record contains the same $usk$ as that in the $\mathsf{RdReg}$.
\end{itemize}
If the platform outputs $b=0$, the deposit operation fails. 
Otherwise, the user outputs the $Rd_{dep} = \mathsf{RdAsset}_i$. 

\tian{do we need update RdReg in deposit? and add year number in RdReg}
\yanan{If the registration record $\mathsf{RdReg}$ is shown in the deposit, the $rid$ will be invalid later. why not update the $\mathsf{RdReg}$? Or the registration record $\mathsf{RdReg}$ is not shown in the deposit?  }
%The platform adds $aid$ to the set $\mathsf{ID}$.

\fi

\item %\noindent%$\mathsf{RdDep}
\noindent$\{Rd\}'\leftarrow\langle\mathsf{Deposit}(epp,pk,upk,usk,\{Rd\},\mathsf{ReqDep}),$ $ \mathsf{Credit}(epp,$ $pk,sk)\rangle\rightarrow b$: 
The deposit request is $\mathsf{ReqDep} = (\textit{deposit}, i, k_i, px_i)$ on asset $i$ with amount $k_i$, and price $px_i$.  
The input record set $\{Rd\}$ only has his registration record $\mathsf{RdReg}=(usk, rid, \textit{cp}_1, \textit{cp}_2, \sigma_{\textit{reg}})$. 
The user chooses randomness $aid, r_1, r_2\sample \mathbb{Z}_p$ and generates new commitments: %on his registration message and deposited asset information: 
$com_1=\mathsf{Com}(usk, rid, \textit{cp}_1, \textit{cp}_2; r_1),$ $com_2=\mathsf{Com}(usk,$ $aid, i, k_i, px_i; r_2)$ with the proof $\pi$ that
\begin{itemize}[noitemsep,leftmargin=*]
    \item he owns a valid signature $\sigma_{\textit{reg}}$
    %record $\mathsf{RdReg}$ 
    according to $com_1$; 
    %\item there is an identifier $aid$ in $com_2$;
    \item $com_2$ contains the correct kind $i$, amount $k_i$ and price $px_i$;
    \item $com_2$ contains an identifier $aid$ and same $usk$ as that in $com_1$. %corresponding to $\mathsf{RdReg}$.
\end{itemize}
The user sends ($\mathsf{ReqDep}$, $com_1$, $com_2$, $\pi$) to the platform.
It checks that the amount of the received asset $i$ is equal to $k_i$, $px_i$ is the current price % according to the $\textit{epp}$ 
and the proof $\pi$ is valid. 
If the check does not pass, the platform outputs $b=0$ and aborts. 
Otherwise, the platform replies with  $\hat{\sigma}_{ast_i}\leftarrow\mathsf{BlindSig}(pp, pk, sk, com_2)$. 
The user unblinds $\hat{\sigma}_{ast_i}$ and gets $\sigma_{ast_i}\leftarrow\mathsf{BlindRcv}(pp,pk,\hat{\sigma}_{ast_i},r_2)$.
If $\mathsf{Vfry}(pp, pk, (usk, aid, i, k_i, px_i),\sigma_{ast_i})$=1, it outputs $\{Rd\}'=\mathsf{RdAsset_i}=(usk$, $aid,i,k_i, px_i,\sigma_{ast_i})$. 
Otherwise %the deposit operation fails and 
outputs 0.

\iffalse
\begin{remark}
The user deposit asset using his registration record $\mathsf{RdReg}$, so that the asset record $\mathsf{RdAsset_i}$ inherits the same $usk$ obliviously. %, and $\mathsf{RdReg}$ needs not to be updated since it does not make profit and the $rid$ is not revealed. 
\end{remark}
\fi


% 
\iffalse
\noindent$Rd_{exc}\leftarrow\langle\mathsf{Exchange}(epp,pk,usk,req_{exc},\{Rd\}), \mathsf{Update}(epp,pk,sk)\rangle\rightarrow b$:
The user's exchange request is $req_{exc}=(\textit{Exchange}, i, k_i, j, k_j)$ and uses $\textit{record}=(\textbf{a}, cred)$.
The platform receives the identifier $id$ and checks that $id\notin\mathsf{ID}$.
If the check does not pass, the platform output $b=0$ and aborts. 
Otherwise, the two parties interact to run
$\textit{cred}'\leftarrow\mathsf{UpdRcv}_{\mathrm{ouac}}(\textit{cp}p,pk,\psi^*,\alpha,\textit{record})\leftrightarrow \mathsf{Update}_{\mathrm{ouac}}(\textit{cp}p,pk,\mathcal{F},sk)\rightarrow b$.
The hidden parameter $\alpha=(id', i, k_i, j, k_j)$ where $id'$ is randomly chosen from $\mathbb{Z}_p$.
The update function $\psi^*$ is
$$\psi^*(\textbf{a},\alpha) = \begin{cases}
\textbf{a}', \ \mathrm{if} \ \psi^*_{chk}  \\
\bot, \ \mathrm{otherwise} \\
\end{cases}$$
%where $\mathbf{\textit{cp}}^*=f(\mathsf{exchange},\mathbf{w},\mathbf{\textit{cp}},i,k_i)$, 
$\psi^*_{chk}$ is true if and only if
\begin{itemize}
    \item the revealed $id$ is the identifier of $\textit{token}$;
    \item $\psi^*\in\mathcal{F}$;
    \item an old record of asset $i$ is chosen from \textbf{a} with enough value $v_i\geq k_i$;
    \item the new record of asset $j$ with value $k_j$ is added to $\textbf{a}'$;
    \item this exchange is fair: $k_i\cdot px_i=k_j\cdot px_j$;
    \item the compliance information is updated correctly in $\textbf{a}'$;
    %\item the $\textit{token}$ shares the same \textit{usk} with the $\textit{record}_i$,
    \item there is a new identifier $id'$ in the credential.
%    \item the $\mathbf{q^*}$ is well-formed.
\end{itemize}

If the platform outputs $b=0$, the exchange operation fails, and the user output $\bot$. 
Otherwise, the user outputs the $Rd_{exc} = \textit{record}'=(\textbf{a}', cred')$ for the new attributes $\textbf{a}'$, and the platform adds $id$ to the spent identifiers set $\mathsf{ID}$.

\fi


%%merge multiple updates into one

%\tian{private and anonymous exchange by updating multiple credentials and just UAC, updatable \textit{multiple} anonymous credentials}

\iffalse

\item \noindent$Rd_{exc}\leftarrow\langle\mathsf{Exchange}(epp,pk,usk,\{Rd\},\mathsf{ReqExc}), \mathsf{Update}(epp,pk,sk)\rangle\rightarrow b$:
The user chooses its records $\{Rd\}=\{\mathsf{RdReg}, \mathsf{RdAsset}\}$ and $\mathsf{ReqExc}=(\textit{Exchange}, i, k_i, j, k_j)$, where 
$\mathsf{RdReg}=(usk, rid, \textit{cp}_1, \textit{cp}_2, \sigma_{reg}), \mathsf{RdAsset}=(usk, aid_i, i, v_i, px_i, \sigma_{coin_i})$.
The platform receives the identifiers $rid$, $aid_i$ and checks that $rid \notin \mathsf{ID}$ and $aid_i \notin \mathsf{ID}$. 
If any of the checks does not pass, the platform output $b=0$ and aborts. 
Otherwise, the two parties interact to update $\mathsf{RdReg}$ and  $\mathsf{RdAsset}_i$, and to issue $\mathsf{RdAsset}_j$ by\\
$\mathsf{RdAsset}_i'\leftarrow\mathsf{UpdRcv}_{uacs}(\textit{cp}p,pk,\psi_0,\alpha_0,\mathsf{RdAsset}_i)\leftrightarrow \mathsf{Update}_{uacs}(\textit{cp}p,pk,\psi_0,sk)\rightarrow b_0$,
$\mathsf{RdReg}'\leftarrow\mathsf{UpdRcv}_{uacs}(\textit{cp}p,pk,\psi_1,\alpha_1,\mathsf{RdReg})\leftrightarrow \mathsf{Update}_{uacs}(\textit{cp}p,pk,\psi_1,sk) \rightarrow b_1$,
$\mathsf{RdAsset}_j\leftarrow\mathsf{Receive}_{uacs}(\textit{cp}p,pk,\psi_2,\alpha_2)\leftrightarrow \mathsf{Issue}_{uacs}(\textit{cp}p,pk,\psi_2,sk)\rightarrow b_2$.

The hidden parameters $\alpha_0=(aid^*,i,k_i), \alpha_1=(rid^*,i, k_i,px_i,\overline{px}_i), \alpha_2=(usk,aid_j, i, \overline{px}_i, j, \overline{px}_j, k_j)$, where $aid_i^*,rid^*,aid_j$ are randomly chosen from $\mathbb{Z}_p$. 
%\yanan{Seems $\alpha_1$ includes the information of two kinds of assets, $\alpha_2$ only includes the information of asset $j$?}
%and $open_0^*, open_1^*$ are randomnesses. 

The update functions $\psi_0, \psi_1, \psi_2$ are 
$$\psi_0((usk, aid_i, i, v_i, px_i), \alpha_0) = \begin{cases}
(usk, aid_i^*, i,v_i-k_i,px_i), \ \mathrm{if} \ \psi_{chk0}  \\
\bot, \ \mathrm{otherwise} \\
\end{cases}$$

%The update function $\psi_1$ is
$$\psi_1((usk, rid, {\textit{cp}_1}, \textit{cp}_2),\alpha_1) = \begin{cases}
(usk, rid^*, {\textit{cp}}_1+\textit{pf}_1, \textit{cp}_2+\textit{pf}_2), \ \mathrm{if} \ \psi_{chk1}  \\
\bot, \ \mathrm{otherwise} \\
\end{cases}$$
%where ${\textit{cp}}^*=\textit{cp}+\textit{pf}$,

%The update funtion $\psi_2$ is
$$\psi_2(\bot,\alpha_2) = \begin{cases}
(usk, aid_j, j, k_j, \overline{px}_j), \ \mathrm{if} \ \psi_{chk2}  \\
\bot, \ \mathrm{otherwise} \\
\end{cases}$$

$\psi_{chk0}\wedge\psi_{chk1}\wedge\psi_{chk2}$ is true if and only if
\begin{itemize}
    \item $\mathsf{RdAsset}_i$ and $\mathsf{RdReg}$ are valid;
    \item the revealed $aid_i$ and $rid$ are identifiers of $\mathsf{RdCoin}_i$ and $\mathsf{RdReg}$;
    \item $\mathsf{RdAsset}_i$ has the same \textit{usk} with the $\mathsf{RdReg}$;
    \item the $i$th asset in $\mathsf{RdAsset}_i$ is enough, i.e., $v_i\geq k_i$;
    \item the new updated and issued records $\mathsf{RdAsset}'_i$, $\mathsf{RdReg}'$, $\mathsf{RdAsset}_j$ share the same $usk$;
    \item there are new identifiers $aid_i^*, rid^*, aid_j$ in the new records;
    \item the $\textit{cp}_1, \textit{cp}_2$ in $\mathsf{RdReg}$ are updated correctly to $\textit{cp}_1+\textit{pf}_1, \textit{cp}_2+\textit{pf}_2$ and $\textit{pf}_1=k_i\cdot px_i$, $\textit{pf}_2=k_i\cdot\overline{px}_i$ where $\overline{px}_i$ is the current price of the asset $i$ ({proof details are shown below});
    \item the new issued record $\mathsf{RdAsset}_j$ is correct: the exchange is fair: $\overline{px}_i\cdot k_i = \overline{px}_j\cdot k_j$ where $\overline{px}_j$ is the current price of the asset $j$.
\end{itemize}

If the platform outputs $b=0$, the exchange operation fails, and the user output $\bot$. 
Otherwise, the user outputs the $Rd_{exc} = (\mathsf{RdReg}', \mathsf{RdAsset}'_i, \mathsf{RdAsset}_j)$. 
%which consists of updated record token $\textit{record}_i'$ on attributes $(usk,dsid^*,\mathbf{w}^*)$, the updated global token $\textit{token}'$ on attributes $(usk,id^*,\mathbf{\textit{cp}}^*)$, and a new record token $\textit{record}_j$ on attributes $(usk,dsid',\mathbf{w}')$, and 
The platform adds $aid, rid$ to the set $\mathsf{ID}$.

\fi


\item %$\mathsf{RdExc}
$\{Rd\}'\leftarrow\langle\mathsf{Exchange}$ $(epp,$ $pk,usk,\{Rd\}, \mathsf{ReqExc}), \mathsf{Update}(epp,$ $pk,$ $sk)\rangle\rightarrow b$:
%The user's exchange request is 
Let $\mathsf{ReqExc}=(\textit{exchange},$ $i, k_i,$ $j, k_j)$. 
The user chooses records $\{Rd\}=\{\mathsf{RdReg}, \mathsf{RdAsset_i}\}$, price tokens $\mathsf{px}(i),$ $\mathsf{px}(j)$ and randomness $aid^*, rid^*,$ 
%r_1, r_2, r_3, r_4, r_5, r_6,$ 
$\{r_u\}_{u=1}^7\sample\mathbb{Z}_p$, where 
$\mathsf{RdReg} = (usk, rid, \textit{cp}_1, \textit{cp}_2, \sigma_{\textit{reg}})$, $\mathsf{RdAsset_i}=(usk, aid_i, i,$ $v_i,$ $px_i,$ $\sigma_{\textit{ast}_i})$, $\mathsf{px}(i)=(au, i, \overline{px}_i,\sigma_i), \mathsf{px}(j)=(au, j,$ $\overline{px}_j,\sigma_j)$.
%The two parties interact to generate new records $\mathsf{RdReg}^*$,  $\mathsf{RdAsset_i^*}$ and $\mathsf{RdAsset_j}$.
The user computes the commitments: 

$com_1=\mathsf{Com}(usk, rid, \textit{cp}_1, \textit{cp}_2; r_1)$, 

$com_2=\mathsf{Com}(usk, aid_i, i, v_i, px_i; r_2)$, %\\

$com_3=\mathsf{Com}(usk, rid^*, \textit{cp}_1^*, \textit{cp}_2^*; r_3)$, %\\

$com_4=\mathsf{Com}(usk, aid_i^*, i, v_i^*, px_i; r_4)$, %\\

$com_5=\mathsf{Com}(usk, aid_j, j, v_j, \overline{px}_j; r_5)$, %\\

$com_6=\mathsf{Com}(au, i, \overline{px}_i; r_6)$, 
$com_7=\mathsf{Com}(au, j, \overline{px}_j; r_7)$ \\
and the proof $\pi$ proving that:

\iffalse


by\\
$\mathsf{RdAsset}_i'\leftarrow\mathsf{UpdRcv}_{uacs}(\textit{cp}p,pk,\psi_0,\alpha_0,\mathsf{RdAsset}_i)\leftrightarrow \mathsf{Update}_{uacs}(\textit{cp}p,pk,\psi_0,sk)\rightarrow b_0$,
$\mathsf{RdReg}'\leftarrow\mathsf{UpdRcv}_{uacs}(\textit{cp}p,pk,\psi_1,\alpha_1,\mathsf{RdReg})\leftrightarrow \mathsf{Update}_{uacs}(\textit{cp}p,pk,\psi_1,sk) \rightarrow b_1$,
$\mathsf{RdAsset}_j\leftarrow\mathsf{Receive}_{uacs}(\textit{cp}p,pk,\psi_2,\alpha_2)\leftrightarrow \mathsf{Issue}_{uacs}(\textit{cp}p,pk,\psi_2,sk)\rightarrow b_2$.

The hidden parameters $\alpha_0=(aid^*,i,k_i), \alpha_1=(rid^*,i, k_i,px_i,\overline{px}_i), \alpha_2=(usk,aid_j, i, \overline{px}_i, j, \overline{px}_j, k_j)$, where $aid_i^*,rid^*,aid_j$ are randomly chosen from $\mathbb{Z}_p$. 
%\yanan{Seems $\alpha_1$ includes the information of two kinds of assets, $\alpha_2$ only includes the information of asset $j$?}
%and $open_0^*, open_1^*$ are randomnesses. 

The update functions $\psi_0, \psi_1, \psi_2$ are 
$$\psi_0((usk, aid_i, i, v_i, px_i), \alpha_0) = \begin{cases}
(usk, aid_i^*, i,v_i-k_i,px_i), \ \mathrm{if} \ \psi_{chk0}  \\
\bot, \ \mathrm{otherwise} \\
\end{cases}$$

%The update function $\psi_1$ is
$$\psi_1((usk, rid, {\textit{cp}_1}, \textit{cp}_2),\alpha_1) = \begin{cases}
(usk, rid^*, {\textit{cp}}_1+\textit{pf}_1, \textit{cp}_2+\textit{pf}_2), \ \mathrm{if} \ \psi_{chk1}  \\
\bot, \ \mathrm{otherwise} \\
\end{cases}$$
%where ${\textit{cp}}^*=\textit{cp}+\textit{pf}$,

%The update funtion $\psi_2$ is
$$\psi_2(\bot,\alpha_2) = \begin{cases}
(usk, aid_j, j, k_j, \overline{px}_j), \ \mathrm{if} \ \psi_{chk2}  \\
\bot, \ \mathrm{otherwise} \\
\end{cases}$$

$\psi_{chk0}\wedge\psi_{chk1}\wedge\psi_{chk2}$ is true if and only if
\fi

\iffalse
    \noindent $-$ \ he owns a valid record $\mathsf{RdReg}$ according to $com_1$ and a valid asset record $\mathsf{RdAsset_i}$ according to $com_2$;\\
    \noindent $-$ \ $rid$ and $aid_i$ are identifiers in $com_1$ and $com_2$;\\
    \noindent $-$ \ there are new identifiers $aid_i^*, rid^*, aid_j$ in $com_3$, $com_4$, $com_5$;\\
    \noindent $-$ \ all these commitments share the same $usk$;\\
    \noindent $-$ \ the $i$-th asset in $com_2$ is enough, i.e., $v_i - k_i\geq 0$ and it is equal to the $v_i^*$ in $com_4$;\\
    \noindent $-$ \ $com_2$ and $com_4$ share the same asset kind $i$ and price $px_i$;\\
    \noindent $-$ \ the $\textit{cp}_1^*, \textit{cp}_2^*$ in $com_3$ are computed correctly as $\textit{cp}_1^*=\textit{cp}_1+\textit{pf}_1, \textit{cp}_2^*=\textit{cp}_2+\textit{pf}_2$ and $\textit{pf}_1=k_i\cdot px_i$, $\textit{pf}_2=k_i\cdot\overline{px}_i$ where $\overline{px}_i$ is the current price of the asset $i$ ({proof details are shown below});\\
    \noindent $-$ \ $com_5$ contains an asset kind $j\in[n]$, number $v_j=k_j$ and price $\overline{px}_j$ satisfying   $\overline{px}_i\cdot k_i = \overline{px}_j\cdot k_j$. %where $\overline{px}_j$ is the current price of the asset $j$.
\fi
%\iffalse

\begin{itemize}[noitemsep,leftmargin=*]
    \item he owns valid platform's signatures w.r.t. $com_1, com_2, com_6, com_7$;
    %valid  $\mathsf{RdReg}$, $\mathsf{RdAsset_i}$,  according to $com_1$ and a valid asset record $\mathsf{RdAsset_i}$ according to $com_2$;
    \item $rid$ and $aid_i$ are identifiers in $com_1$ and $com_2$;
    \item there are identifiers $aid_i^*, rid^*, aid_j$ in $com_3$, $com_4$, $com_5$;
    \item $\{\textit{com}_u\}_{u=1}^5$ share the same $usk$;
    \item the $i$-th asset in $com_2$ is enough, i.e., $k_i\geq 0$ and $v_i - k_i = v_i^*\geq 0$; %and it is equal to the $v_i^*$ in $com_4$;
    \item $com_2, com_4$ and $com_6$ share the same asset kind $i$;
    \item $com_2$ and $com_4$ share the same price $px_i$;
    \item $com_5$ and $com_7$ share the same kind $j$ and price $\overline{px}_j$;
    \item $com_3$ contains 
    %compliance correctness 
    %the $\textit{cp}_1^*, \textit{cp}_2^*$ in $com_3$ are computed correctly as 
    $\textit{cp}_1^*=\textit{cp}_1+k_i\cdot px_i, \textit{cp}_2^*=\textit{cp}_2+k_i\cdot\overline{px}_i$; 
    %where $\overline{px}_i$ is the price in $com_6$;
    \item fairness: $\textit{com}_5$ contains 
    %an asset kind $j\in[n]$ which is same with $com_7$, 
    number $v_j=k_j>0$ and price $\overline{px}_j$ satisfying $\overline{px}_i\cdot k_i = \overline{px}_j\cdot k_j$, which also implies $k_i>0$. %where $\overline{px}_j$ is the price in $com_7$. %where $\overline{px}_j$ is the current price of the asset $j$.
\end{itemize}
%\fi


He sends $(rid, aid, \{\textit{com}_u\}_{u=1}^7, \pi)$
%$(rid, aid, com_1, com_2, com_3, com_4, com_5, com_6,$ $com_7, \pi)$ 
to the platform.
It checks that $rid \notin \mathsf{ID}$ and $aid_i \notin \mathsf{ID}$ and proof $\pi$ is valid. 
If any of the checks does not pass, the platform output $b=0$ and aborts. 
Otherwise, the platform replies with blind signatures $\hat{\sigma}_{\textit{reg}}, \hat{\sigma}_{\textit{ast}_i},\hat{\sigma}_{\textit{ast}_j}$ on $\textit{com}_3,\textit{com}_4, \textit{com}_5$ respectively.
%:\\ $\hat{\sigma}_{reg}\leftarrow\mathsf{BlindSig}(pp, pk, sk, com_3)$,\\ $\hat{\sigma}_{ast_i}\leftarrow\mathsf{BlindSig}(pp, pk, sk, com_4)$,\\ $\hat{\sigma}_{ast_j}\leftarrow\mathsf{BlindSig}(pp, pk, sk, com_5)$. \\
The user unblinds them and gets ${\sigma}^*_{\textit{reg}}, {\sigma}^*_{\textit{ast}_i},{\sigma}^*_{\textit{ast}_j}$.

\iffalse
\\ $\sigma^*_{reg}\leftarrow\mathsf{BlindRcv}(pp,pk,\hat{\sigma}_{reg},r_3)$,\\ 
$\sigma^*_{ast_i}\leftarrow\mathsf{BlindRcv}(pp,pk,\hat{\sigma}_{ast_i},r_4)$,\\ 
$\sigma^*_{ast_j}\leftarrow\mathsf{BlindRcv}(pp,pk,\hat{\sigma}_{ast_j},r_5)$.
\fi


If $\mathsf{Vfry}(pp, pk, (usk, rid^*, \textit{cp}_1^*, \textit{cp}_2^*),\sigma^*_{\textit{reg}})=1$ %\\
$\wedge\mathsf{Vfry}(pp, pk, (usk, aid_i^*,$ $i, v_i^*, px_i),\sigma^*_{\textit{ast}_i})=1$  %\\
$\wedge\mathsf{Vfry}(pp, pk, (usk, aid_j, j, k_j, px_j),\sigma^*_{\textit{ast}_j})$=1,  
he outputs $\{Rd\}' = \{\mathsf{RdReg}^*, \mathsf{RdAsset_i^*}, \mathsf{RdAsset_j}\}$, 
$\mathsf{RdReg}^*=(usk, rid^*, \textit{cp}_1^*, \textit{cp}_2^*,\sigma^*_{\textit{reg}})$,
$\mathsf{RdAsset_i^*}=(usk, aid_i^*, i, v_i^*, px_i,\sigma^*_{\textit{ast}_i})$,  
$\mathsf{RdAsset_j}= (usk, aid_j, j, k_j, px_j,\sigma^*_{\textit{ast}_j})$.
The platform adds $aid, rid$ to  $\mathsf{ID}$.
%$Rd_{exc}=(\mathsf{RdAsset}_i=(usk$, $aid,i,k_i, px_i,\sigma)$. Otherwise the deposit operation fails and outputs 0.
Otherwise, user outputs $\bot$. 

%Otherwise, the user outputs the $Rd_{exc} = (\mathsf{RdReg}', \mathsf{RdAsset}'_i, \mathsf{RdAsset}_j)$. 

%which consists of updated record token $\textit{record}_i'$ on attributes $(usk,dsid^*,\mathbf{w}^*)$, the updated global token $\textit{token}'$ on attributes $(usk,id^*,\mathbf{\textit{cp}}^*)$, and a new record token $\textit{record}_j$ on attributes $(usk,dsid',\mathbf{w}')$, and 



\iffalse
\item \noindent$Rd_{wit}\leftarrow\langle\mathsf{Withdraw}(epp,pk,usk,\{Rd\},\mathsf{ReqWit}), \mathsf{Deduct}(epp,pk,sk)\rangle\rightarrow b$:
The user's exchange request is $\mathsf{ReqWit}=(\textit{Withdraw}, i, k_i)$ and uses $\{\textit{Rd}\}=(\mathsf{RdReg}, \mathsf{RdAsset}_i)$.
The platform receives the identifiers $aid, rid$ and checks that $aid, rid\notin\mathsf{ID}$.
If the check does not pass, the platform output $b=0$ and aborts. 
Otherwise, the two parties interact to update $\mathsf{RdReg}$ and  $\mathsf{RdAsset}_i$ by\\
$\mathsf{RdAsset}_i'\leftarrow\mathsf{UpdRcv}_{uacs}(\textit{cp}p,pk,\psi_0,\alpha_0,\mathsf{RdAsset}_i)\leftrightarrow \mathsf{Update}_{uacs}(\textit{cp}p,pk,\psi_0,sk)\rightarrow b_0$,
$\mathsf{RdReg}'\leftarrow\mathsf{UpdRcv}_{uacs}(\textit{cp}p,pk,\psi_1,\alpha_1,\mathsf{RdReg})\leftrightarrow \mathsf{Update}_{uacs}(\textit{cp}p,pk,\psi_1,sk) \rightarrow b_1$.

The hidden parameters $\alpha_0=(aid^*), \alpha_1=(rid^*,px_i),$ %\alpha_2=(usk,aid_j, i, \overline{px}_i, j, \overline{px}_j, k_j)$, 
where $aid_i^*,rid^*$ are randomly chosen from $\mathbb{Z}_p$. 
%and $open_0^*, open_1^*$ are randomnesses. 

The update function $\psi_0, \psi_1$ are 
$$\psi_0((usk, aid_i, i, v_i, px_i), \alpha_0) = \begin{cases}
(usk, aid_i^*, i,v_i-k_i,px_i), \ \mathrm{if} \ \psi_{chk0}  \\
\bot, \ \mathrm{otherwise} \\
\end{cases}$$

%The update function $\psi_1$ is
$$\psi_1((usk, rid, {\textit{cp}_1}, \textit{cp}_2 ),\alpha_1) = \begin{cases}
(usk, rid^*, {\textit{cp}}_1+\textit{pf}_1, {\textit{cp}}_2+\textit{pf}_2), \ \mathrm{if} \ \psi_{chk1}  \\
\bot, \ \mathrm{otherwise} \\
\end{cases}$$
%where ${\textit{cp}}^*=\textit{cp}+\textit{pf}$,


$\psi_{chk0}\wedge\psi_{chk1}$ is true if and only if
\begin{itemize}
    \item $\mathsf{RdAsset}_i$ and $\mathsf{RdReg}$ are valid;
    \item the revealed $aid$ and $rid$ are identifiers of $\mathsf{RdAsset}_i$ and $\mathsf{RdReg}$;
    \item $\mathsf{RdAsset}_i$ shares the same \textit{usk} with the $\mathsf{RdReg}$;
    \item the $i$th asset in $\mathsf{RdAsset}_i$ is enough, i.e., $v_i\geq k_i$;
    %\item the new updated and issued records $\mathsf{RdCoin}'_i$, $\mathsf{RdReg}'$, $\mathsf{RdCoin}_j$ share the same $usk$;
    \item there are new identifiers $aid_i^*, rid^*$ in the new records;
    \item the $\textit{cp}_1, \textit{cp}_2$ in $\mathsf{RdReg}$ are updated correctly to $\textit{cp}_1+\textit{pf}_1, \textit{cp}_2+\textit{pf}_2$ and $\textit{pf}_1=k_i\cdot px_i$, $\textit{pf}_2=k_i\cdot\overline{px}_i$ where $\overline{px}_i$ is the current price of the asset $i$.
    %\item the new issued record $\mathsf{RdCoin}_j$ is correct, the exchange is fair: $\overline{px}_i\cdot k_i = \overline{px}_j\cdot k_j$ where $\overline{px}_j$ is the current price of the asset $j$.
\end{itemize}




If the platform outputs $b=0$, the exchange operation fails, and the user output $\bot$. 
Otherwise, the user outputs the $Rd_{wit} = (\mathsf{RdCoin}_i, \mathsf{RdReg})$, and the platform adds $aid, rid$ to the spent identifiers set $\mathsf{ID}$.
\fi

\item %$\mathsf{RdWit}
$\{Rd\}'\leftarrow\langle\mathsf{Withdraw}(epp,$ $pk,usk,\{Rd\},\mathsf{ReqWit}),\mathsf{Deduct}$ $(epp,$ $pk,sk)\rangle\rightarrow b$:
The user sets $\mathsf{ReqWit}=(\textit{withdraw}, i, k_i)$,
chooses $\{Rd\}=\{\mathsf{RdReg}, \mathsf{RdAsset_i}\}$ and randomnesses $aid^*, rid^*, r_1, r_2,$ $r_3, r_4 \sample \mathbb{Z}_p$, where 
$\mathsf{RdReg}$ $ = (usk, rid, \textit{cp}_1, \textit{cp}_2, \sigma_{\textit{reg}})$, $\mathsf{RdAsset_i}=(usk, aid_i, i, v_i, px_i, \sigma_{ast_i})$.
%The two parties interact to produce new records $\mathsf{RdReg}^*$ and  $\mathsf{RdAsset_i^*}$.
He computes the commitments: \\
$com_1=\mathsf{Com}(usk, rid, \textit{cp}_1, \textit{cp}_2; r_1)$, \\
$com_2=\mathsf{Com}(usk, aid_i, i, v_i, px_i; r_2)$, \\
$com_3=\mathsf{Com}(usk, rid^*, \textit{cp}_1^*, \textit{cp}_2^*; r_3)$,\\
$com_4=\mathsf{Com}(usk, aid_i^*, i, v_i^*, px_i; r_4)$\\ 
and the proof $\pi$ proving that:

\begin{itemize}[noitemsep,leftmargin=*]
    \item he owns valid platform's signatures
    %records $\mathsf{RdReg}$, $\mathsf{RdAsset_i}$ 
    w.r.t. $com_1$, $com_2$;
    \item $rid$ and $aid_i$ are identifiers in $com_1$ and $com_2$;
    \item there are new identifiers $aid_i^*, rid^*$ in $com_3$, $com_4$;
    \item all these commitments share the same $usk$;
    \item the $i$-th asset in $com_2$ is enough, i.e., $k_i\geq 0$ and $v_i - k_i = v_i^*\geq 0$; % and it is equal to the $v_i^*$ in $com_4$;
    \item $com_2$ and $com_4$ share the same asset kind $i$ and price $px_i$;
    \item %the $\textit{cp}_1^*, \textit{cp}_2^*$ in $com_3$ are computed correctly as 
    $com_3$ contains $\textit{cp}_1^*=\textit{cp}_1+k_i\cdot px_i, \textit{cp}_2^*=\textit{cp}_2+k_i\cdot\overline{px}_i$. %where $\overline{px}_i$ is the current price of the asset $i$;
\end{itemize}

He sends $(rid, aid, com_1, com_2, com_3, com_4, \pi)$ to the platform.
It checks that $rid \notin \mathsf{ID}$ and $aid_i \notin \mathsf{ID}$. 
If any of the checks does not pass, the platform output $b=0$ and aborts. 
Otherwise, the platform replies with blind signatures $\hat{\sigma}_{reg}, \hat{\sigma}_{ast_i}$ on $com_3, com_4$.\\ %$\hat{\sigma}_{reg}\leftarrow\mathsf{BlindSig}(pp, pk, sk, com_3)$,\\ $\hat{\sigma}_{ast_i}\leftarrow\mathsf{BlindSig}(pp, pk, sk, com_4)$,\\ 
The user unblinds them and gets $\sigma^*_{reg},\sigma^*_{ast_i}$. %$\sigma^*_{reg}\leftarrow\mathsf{BlindRcv}(pp,pk,\hat{\sigma}_{reg},r_3)$,\\ 
%$\sigma^*_{ast_i}\leftarrow\mathsf{BlindRcv}(pp,pk,\hat{\sigma}_{ast_i},r_4)$.
If they are valid,
%$\mathsf{Vfry}(pp, pk, (usk, rid^*, \textit{cp}_1^*, \textit{cp}_2^*), \sigma^*_{reg})=1\wedge$ \\
%$\mathsf{Vfry}(pp, pk, (usk, aid_i^*, i, v_i^*, px_i),\sigma^*_{ast_i})=1$, 
he outputs $\{Rd\}' = \{\mathsf{RdReg}^*, \mathsf{RdAsset_i^*}\}$. 
$\mathsf{RdReg}^*=(usk, rid^*, \textit{cp}_1^*,$ $\textit{cp}_2^*,$ $\sigma^*_{\textit{reg}})$,
$\mathsf{RdAsset_i^*}=(usk, aid_i^*, i, v_i^*, px_i,\sigma^*_{\textit{ast}_i})$.
The platform adds $aid, rid$ to the set $\mathsf{ID}$.
Otherwise, user outputs $\bot$.




\iffalse
by\\
$\mathsf{RdAsset}_i'\leftarrow\mathsf{UpdRcv}_{uacs}(\textit{cp}p,pk,\psi_0,\alpha_0,\mathsf{RdAsset}_i)\leftrightarrow \mathsf{Update}_{uacs}(\textit{cp}p,pk,\psi_0,sk)\rightarrow b_0$,
$\mathsf{RdReg}'\leftarrow\mathsf{UpdRcv}_{uacs}(\textit{cp}p,pk,\psi_1,\alpha_1,\mathsf{RdReg})\leftrightarrow \mathsf{Update}_{uacs}(\textit{cp}p,pk,\psi_1,sk) \rightarrow b_1$.

The hidden parameters $\alpha_0=(aid^*), \alpha_1=(rid^*,px_i),$ %\alpha_2=(usk,aid_j, i, \overline{px}_i, j, \overline{px}_j, k_j)$, 
where $aid_i^*,rid^*$ are randomly chosen from $\mathbb{Z}_p$. 
%and $open_0^*, open_1^*$ are randomnesses. 

The update function $\psi_0, \psi_1$ are 
$$\psi_0((usk, aid_i, i, v_i, px_i), \alpha_0) = \begin{cases}
(usk, aid_i^*, i,v_i-k_i,px_i), \ \mathrm{if} \ \psi_{chk0}  \\
\bot, \ \mathrm{otherwise} \\
\end{cases}$$

%The update function $\psi_1$ is
$$\psi_1((usk, rid, {\textit{cp}_1}, \textit{cp}_2 ),\alpha_1) = \begin{cases}
(usk, rid^*, {\textit{cp}}_1+\textit{pf}_1, {\textit{cp}}_2+\textit{pf}_2), \ \mathrm{if} \ \psi_{chk1}  \\
\bot, \ \mathrm{otherwise} \\
\end{cases}$$
%where ${\textit{cp}}^*=\textit{cp}+\textit{pf}$,

$\psi_{chk0}\wedge\psi_{chk1}$ is true if and only if
\fi
\iffalse
\begin{itemize}
    \item $\mathsf{RdAsset}_i$ and $\mathsf{RdReg}$ are valid;
    \item the revealed $aid$ and $rid$ are identifiers of $\mathsf{RdAsset}_i$ and $\mathsf{RdReg}$;
    \item $\mathsf{RdAsset}_i$ shares the same \textit{usk} with the $\mathsf{RdReg}$;
    \item the $i$th asset in $\mathsf{RdAsset}_i$ is enough, i.e., $v_i\geq k_i$;
    %\item the new updated and issued records $\mathsf{RdCoin}'_i$, $\mathsf{RdReg}'$, $\mathsf{RdCoin}_j$ share the same $usk$;
    \item there are new identifiers $aid_i^*, rid^*$ in the new records;
    \item the $\textit{cp}_1, \textit{cp}_2$ in $\mathsf{RdReg}$ are updated correctly to $\textit{cp}_1^*=\textit{cp}_1+\textit{\textit{pf}}_1, \textit{cp}_2^*=\textit{cp}_2+\textit{\textit{pf}}_2$ and $\textit{\textit{pf}}_1=k_i\cdot px_i$, $\textit{\textit{pf}}_2=k_i\cdot\overline{px}_i$ where $\overline{px}_i$ is the current price of the asset $i$.
    %\item the new issued record $\mathsf{RdCoin}_j$ is correct, the exchange is fair: $\overline{px}_i\cdot k_i = \overline{px}_j\cdot k_j$ where $\overline{px}_j$ is the current price of the asset $j$.
\end{itemize}
The platform receives the identifiers $aid, rid$ and checks that $aid, rid\notin\mathsf{ID}$.
If the check does not pass, the platform output $b=0$ and aborts. 
Otherwise, 

If the platform outputs $b=0$, the exchange operation fails, and the platform replies with signed signatures $\hat{\sigma}_1\leftarrow\mathsf{BlindSig}(pp, pk, sk, com_3)$, $\hat{\sigma}_2\leftarrow\mathsf{BlindSig}(pp, pk, sk, com_4)$. 
The user unblinds them and gets $\sigma_1\leftarrow\mathsf{BlindRec}(pp,pk,\hat{\sigma}_1,r_3)$, 
$\sigma_2\leftarrow\mathsf{BlindRec}(pp,pk,\hat{\sigma}_2,r_4)$.

If $\mathsf{Vfry}(pp, pk, (usk, rid^*, \textit{cp}_1^*, \textit{cp}_2^*),\sigma_1)$=1, 
$\mathsf{Vfry}(pp, pk, (usk, aid_i^*, i, v_i^*, px_i),\sigma_2)$=1,   
it outputs $Rd_{wit} = (\mathsf{RdReg}', \mathsf{RdAsset}'_i)$. 
The platform adds $aid, rid$ to the set $\mathsf{ID}$.
%$Rd_{exc}=(\mathsf{RdAsset}_i=(usk$, $aid,i,k_i, px_i,\sigma)$. Otherwise the deposit operation fails and outputs 0.
Otherwise, user output $\bot$. 
\fi

\iffalse
\begin{remark}
The withdrawal can be seemed as a special exchange where the exchange content is public and there is only asset deduction. No new asset generates. 
Here the user just updates the profits and asset amount in his records.
\end{remark}
\fi

\item %$\mathsf{RdFil}
$\{Rd\}'\leftarrow \langle\mathsf{File}(epp, pk, usk, \{Rd\}, \mathsf{ReqFil}),
\mathsf{Sign}(epp,pk,$ $sk)\rangle\rightarrow b$: 
The user %interacts with the platform to generate the compliance document $\mathit{doc}$. He 
chooses $\{Rd\}=\mathsf{RdReg}$ and $\mathsf{ReqFil}=(\textit{file}, upk)$,
computes the commitments: %\\
$com_1=\mathsf{Com}(usk, rid, \textit{cp}_1, \textit{cp}_2; r_1)$, %\\
$com_2=\mathsf{Com}(usk, rid^*, \textit{cp}_1^*, \textit{cp}_2^*; r_2)$, %\\
$com_3=\mathsf{Com}(upk, \textit{cp}_1, \textit{cp}_2,$ $au; r_3)$ %\\ 
and the proof $\pi$ that:
\iffalse
the two parties run\\ $\mathsf{RdReg}'\leftarrow\mathsf{UpdRcv}_{\mathrm{uacs}}(\textit{cp}p,pk,\psi^*,\alpha,\textit{record})\leftrightarrow \mathsf{Update}_{\mathrm{uacs}}(\textit{cp}p,pk,\psi^*,sk) \rightarrow b$. 
The hidden parameter $\alpha=(rid', r)$ where $rid',r$ are chosen randomly by the user. 
The update function $\psi^*$ is 
$$\psi^*((usk, rid, \textit{cp}_1, \textit{cp}_2),\alpha) = \begin{cases}
(usk, rid', 0, 0),\ \mathrm{if} \ \psi^*_{chk}  \\
\bot, \ \mathrm{otherwise} \\
\end{cases}$$
%where $\mathbf{\textit{cp}^*}=f(\mathsf{File}, \mathbf{\textit{cp}})$.
$\psi^*_{chk}$ is true if and only if
\fi
\begin{itemize}[noitemsep,leftmargin=*]
    \item he owns a valid platform's signature w.r.t. 
    %record $\mathsf{RdReg}$ according to 
    $\textit{com}_1$;
    \item the revealed $\textit{rid}$ is the identifier in $\textit{com}_1$;
    %\item %the $usk$ in the $com_1$ is matched with the user's public key, i.e., 
    %$upk=\mathsf{ComputPK}(epp,usk)$.
    \item  $com_1$, $com_2$ share the same $usk$ and $upk=\mathsf{ComputPK}(epp,usk)$;
    \item $com_2$ contains an identifier $rid^*$ and $(\textit{cp}^*_1, \textit{cp}^*_2)=(0,0)$;
    \item $com_3$ contains $\textit{cp}_1, \textit{cp}_2$ which are the same as that in $com_1$; 
    \item $com_3$ contains the public $au$ and  $upk$ in $\mathsf{ReqFil}$. %the public auxiliary information $au$.
\end{itemize}
He sends $(\mathsf{ReqFil}, rid, au, com_1, com_2, com_3, \pi)$ to the platform.
If $upk\notin\mathsf{UPK}$ or $rid\in \mathsf{ID}$ or $au$ is not correct, the platform outputs $b=0$ and aborts. 
Otherwise, it replies with blind signatures $\hat{\sigma}_{\textit{reg}}, \hat{\sigma}_{\textit{cp}}$ on $\textit{com}_2, \textit{com}_3$. %$\hat{\sigma}_{reg}\leftarrow\mathsf{BlindSig}(pp, pk, sk, com_2)$, $\hat{\sigma}_{com}\leftarrow\mathsf{BlindSig}(pp, pk, sk, com_3)$. 
The user unblinds them and gets $\sigma_{\textit{reg}}^*, \sigma_{\textit{cp}}$. 
%$\sigma_{reg}^*\leftarrow\mathsf{BlindRcv}(pp,pk,\hat{\sigma}_1,r_2)$, 
%$\sigma_{cp}\leftarrow\mathsf{BlindRcv}(pp,pk,\hat{\sigma}_2,r_3)$.
If $\mathsf{Vfry}(pp, pk, (usk, \textit{rid}^*, \textit{cp}_1^*, \textit{cp}_2^*),\sigma_{\textit{reg}}^*)=1$ $\wedge$
$\mathsf{Vfry}(pp, pk, (upk,$ $ \textit{cp}_1, \textit{cp}_2),\sigma_{cp})=1$,   
it outputs $\{Rd\}' = \{\mathsf{RdReg}^*,$ $\mathit{doc}=(upk, \textit{cp}_1,$ $\textit{cp}_2, au,  \sigma_{cp})\}$. 
The platform adds $rid$ to $\mathsf{ID}$.
Otherwise, output $\bot$. 


\iffalse
If the platform outputs $b=0$, the operation fails and the user outputs $\bot$. 
Otherwise, the platform completes the above update protocol and runs $\mathsf{BlindSign}_{sig}(pp, pk, sk, c)$ and the user runs $\mathsf{BlindRcv}_{sig}(pp, pk, (upk, \textit{cp}_1, \textit{cp}_2), r)$ and outputs a signature $\sigma$.
It checks if $\mathsf{Vrfy}_{sig}(pp, pk, (upk,\textit{\textit{cp}}_1, \textit{cp}_2),\sigma)=1$.
If yes, it means $\sigma$ is a valid signature on $(upk,\textit{cp}_1, \textit{cp}_2)$ and $(upk,\textit{cp}_1, \textit{cp}_2, \sigma)$ is denoted by $Doc$.
In the end, the user output the compliance record $Rd_{com}$. 
It can be parsed to  $(\mathsf{RdReg}',Doc)$. 
%The updated global token $\textit{token}^*=(usk,id^*,\mathbf{\textit{cp}}^*,cred^*)$ where $cred^*$ is a credential on $(usk,id^*,\mathbf{\textit{cp}}^*)$.
%The compliance token $\textit{comp}=(upk,\mathbf{\textit{cp}},\sigma)$ where $\sigma$ is a signature on $(upk,\mathbf{\textit{cp}})$.
\fi

\item \noindent$\mathsf{Verify}(epp, pk, \mathit{doc}, au')\rightarrow b$: 
The public auxiliary information is $au'$ and the authority receives $\mathit{doc}=(upk, \textit{cp}_1, \textit{cp}_2, au, \sigma)$. %from some user. 
If $au=au'$ and $\mathsf{Vrfy}(pk,(upk,\textit{cp}_1,\textit{cp}_2, au),\sigma)\rightarrow 1$, then it outputs $b=1$ indicating the verification succeeds. 
Otherwise, it fails.
%and $\mathsf{check}(\textit{cp}_1, \textit{cp}_2,{au})\rightarrow b_1$. 
%$\textsf{check}$ is a public check algorithm and ${au}$ is the auxiliary information, which both are specified according to regulations. 
%The output $b=b_0\wedge b_1=0$  
\end{itemize}

\fi
%%%%%%%%%%%%%%%%%%%%%scheme%%%%%%%









%\yanan{how to put the verify algorithm? It is the algorithm beyond the two parties, and is not in the platform, but is necessary for compliance.}

% Given the platform's public key $pk$, the user's \textit{upk}, its compliance information \textbf{\textit{cp}}, a signature $\sigma$  and some auxiliary information \textbf{au}. Anyone can check the validness of the user's compliance information by running $\mathsf{Verify}(pk,upk,\textbf{\textit{cp}},\sigma,\textbf{au})$. It outputs a bit \textit{b} indicating if the user's compliance information \textbf{\textit{cp}} is valid according to the auxiliary information \textbf{au}. If \textit{b}=0, it is invalid. Otherwise, it is valid.

\begin{comment}
\iffalse
The update function $\psi_1$ is
$$\psi_1((usk, id, \mathbf{\textit{cp}} ),\alpha_1) = \begin{cases}
(usk, id^*, \mathbf{\textit{cp}}^*), \ \mathrm{if} \ \psi_{chk1}  \\
\bot, \ \mathrm{otherwise} \\
\end{cases}$$
where $\mathbf{\textit{cp}}^*=f(\mathsf{exchange},\mathbf{w},\mathbf{\textit{cp}},i,k_i)$, %and $\mathbf{q^*}=f(\mathsf{exchange}, \mathbf{q}, i, k_i)$.
$\psi_{chk1}$ is true if and only if
\begin{itemize}
    \item the revealed $id$ is the identifier of $\textit{token}$,
    \item the $\textit{token}$ shares the same \textit{usk} with the $\textit{record}_i$,
    \item there is a new identifier $id^*$ in the credential.
%    \item the $\mathbf{q^*}$ is well-formed.
\end{itemize}
The update funtion $\psi_2$ is
$$\psi_2(\bot,\alpha_2) = \begin{cases}
(usk, dsid', \mathbf{w}'), \ \mathrm{if} \ \psi_{chk2}  \\
\bot, \ \mathrm{otherwise} \\
\end{cases}$$
where $\mathbf{w}'=(j,k_j,px_j)$, $\psi_{chk2}$ is true if and only if
\begin{itemize}
    \item the user's secret key in the attributes is the same as the \textit{usk} in the attributes of $\textit{record}_i$,
    \item there is an identifier $dsid'$ in the attributes. 
\end{itemize}
 
\noindent$\bullet$ \textbf{Enroll}\quad Users are enrolled in the exchange system when they obtaining a token from the platform authority. 
A token \textit{token} = $(id, \mathbf{px}, cred)$ consists of its identifier \textit{id}, its current value vector $\mathbf{v}$, its current compliance information vector $\mathbf{px}$ and a credential \textit{cred} on the attributes $(usk, id, \mathbf{px})$. 
In order to request the platform issue the credential, the user sends its $upk$ to the platform.
His hidden parameter is $\alpha=(usk, id)$ where $id$ is chosen randomly from $\mathbb{Z}_p$. 
The update function is
$$\psi(\bot,\alpha) = \begin{cases}
(usk, id, \mathbf{0}), \ \mathrm{if} \ \psi_{chk}  \\
\bot, \ \mathrm{otherwise} \\
\end{cases}$$
where $\psi_{chk}$ is true if and only if
\begin{itemize}
    \item The user's secret in the attributes/credential is consistent with the user's public key, i.e., $upk=\mathsf{ComputePK}(pp, usk)$,
    \item there is an identifier $id$ in the attributes/credential 
\end{itemize}

The platform interacts with the user by running $\langle\mathsf{Issue}_{\mathrm{uacs}}(\textit{cp}p, pk, \psi, sk), \mathsf{Receive}_{\mathrm{uacs}}(\textit{cp}p, pk, \psi, \alpha)\rangle$. % and outputs a $cred$ which is hidden from the exchange. 
The user outputs his token $token=(id,\mathbf{px}=\mathbf{0},cred)$.
The exchange records the new enrolled user with its $upk$. 





 
\noindent$\bullet$ \textbf{Deposit}
The user deposits the $i$-th kind of asset with number of $k_i$ and price $px_i$ in the system.
%Here the update function is $$\psi((usk, id, \mathbf{v}, \mathbf{px}),\cdot) = \begin{cases}
%(usk, id, \mathbf{v^*}, \mathbf{px^*}), \ \mathrm{if} \ \psi_{\textit{chk}}  \\
%\bot, \ \mathrm{otherwise} \\
%\end{cases}$$
%where $\mathbf{v^*}=(v_1,\dots,v_i+k,\dots,v_n)$ and $\mathbf{px^*}=f(\mathsf{deposit}, \mathbf{px}, i, k)$. $\psi_{\textit{chk}}$ is true if and only if the $\mathbf{px^*}$ is well-formed. The exchange interacts with the user by running $\mathsf{Update}_{\mathrm{uacs}}(\textit{cp}p, pk, \psi,sk)\leftrightarrow\mathsf{UpdRcv}_{\mathrm{uacs}}(\textit{cp}p, pk, \psi, \alpha)$ and outputs a $cred^*$ which is hidden from the exchange. The user outputs his new token $token^*=(id, \mathbf{v^*},\mathbf{px^*},cred^*)$.

The user obtains an anonymous record describing details of this deposited asset 
\textit{record}$ = (rid, \mathbf{w}, cred)$
consists of the identifier \textit{rid}, the public detail $\mathbf{w}=(i, k_i, px_i)$ for this
deposited asset and a credential \textit{cred} on attributes $(usk, rid, \mathbf{w})$. 

The user designs the update function as follows.
The hidden parameter is $\alpha=(usk, rid)$ where $rid$ is chosen randomly from $\mathbb{Z}_p$. 
%The update function is
$$\psi(\bot,\alpha) = \begin{cases}
(usk, rid, \mathbf{w}), \ \mathrm{if} \ \psi_{chk}  \\
\bot, \ \mathrm{otherwise} \\
\end{cases}$$
where $\psi_{chk}$ is true if and only if
\begin{itemize}
    \item The user's secret key in the attributes is consistent with the user's public key, i.e., $upk=\mathsf{ComputePK}(pp, usk)$,
    \item there is an identifier $rid$ in the attributes. 
\end{itemize}

The platform interacts with the user by running $\langle\mathsf{Issue}_{\mathrm{uacs}}(\textit{cp}p, pk, \psi, sk), \mathsf{Receive}_{\mathrm{uacs}}(\textit{cp}p, pk, \psi, \alpha)\rangle$. %and outputs a $cred$ which is hidden from the exchange. 
The user outputs this anonymous record $record=(rid, \mathbf{w}, cred)$.
%$\mathbf{w}$ is the detail for this deposit that is public. 

 

\noindent$\bullet$ \textbf{Exchange}:
The user requests to exchange one asset $i$ to another $j$ with the \textit{record} for that asset $i$ and its latest \textit{token}.
The platform deducts value $v_i$ by $k_i$ of the \textit{record} and updates the compliance information $\mathbf{\textit{cp}}$ in $token$ to $f(\mathsf{exchange}, \mathbf{w}, \mathbf{\textit{cp}}, i, k_i)$. 
%To update the token compliance information $\mathbf{px}$, it also needs the details $\mathbf{w}$ of that asset.
%Then it is updated to $f(\mathsf{exchange}, \mathbf{w}, \mathbf{px}, i, k_i)$.
Afterwards, the user gets the updated $\textit{token}'$, $\textit{record}'$ and a new $\textit{record}^*$ with $(j, k_j, px_j)$ for this new obtained asset. 
During the interaction, the user shows the identifiers $id, rid$ and they run\\ $\mathsf{Exchange}(epp, pk, f, i, j, k_i, k_j, usk, token, record) \leftrightarrow \mathsf{Update}(epp, pk, f, i, j, k_i, k_j, sk)$. 
%It consists of updating \textit{token} and \textit{record} for asset \textit{i} and generating $\textit{record}'$ for asset \textit{j}. 
It works as follows.

The user updates his \textit{record}.
He shows an identifier $rid$ and run a credential update protocol with the exchange on his \textit{record}: $\mathsf{Update}_{\mathrm{uacs}}(\textit{cp}p, pk, \psi, sk)\leftrightarrow\mathsf{UpdRcv}_{\mathrm{uacs}}(\textit{cp}p, pk, \psi, \alpha)$.
%It includes a check whether the data sent by the user is formed correctly.
The hidden parameter is $\alpha=(usk, rid')$ where $rid'$ is chosen randomly by the user. The update function is 

$$\psi((usk, rid, \mathbf{w}, ),\alpha) = \begin{cases}
(usk, rid', \mathbf{w'}, ), \ \mathrm{if} \ \psi_{chk}  \\
\bot, \ \mathrm{otherwise} \\
\end{cases}$$
where $\mathbf{w'}=(i,v_i-k_i,px_i)$ %and $\mathbf{q^*}=f(\mathsf{exchange}, \mathbf{q}, i, k_i)$.
$\psi_{chk}$ is true if and only if
\begin{itemize}
    \item the revealed $rid$ is the identifier in the credential,
    \item the \textit{record} shares the same \textit{usk} with the \textit{token},
    \item the $i$th asset in this record is enough, i.e., $v_i\geq k_i$,
    \item there is a new identifier $rid'$ in the credential,
%    \item the $\mathbf{q^*}$ is well-formed.
\end{itemize}
The user outputs a $cred'$ and its new token $record'=(rid^*, \mathbf{w'}, cred')$.

In this exchange, the user gets new asset $j$ like in the deposit transaction, and he also generates a record for it: 
${record}^* = (rid^*, \mathbf{w^*}, cred^*)$.
It consists of an identifier ${rid}^*$, the detail vector $\mathbf{w}^*$ and a credential ${cred}^*$ on attributes $(usk, rid^*, \mathbf{w^*})$. 

Here \textit{usk} is user's secret key and he proves that it is the same as the attribute in that \textit{token}.
$\mathbf{w^*}=(j, k_j, px_j)$ is the detail of that asset \textit{j} which is public for the issuer.  %$\mathbf{q}$ is the compliance information and is initialized to zeroes.
His hidden parameter is $\alpha=(usk, rid^*)$ where $rid^*$ is chosen randomly from $\mathbb{Z}_p$. 
The update function is
$$\psi(\bot,\alpha) = \begin{cases}
(usk, rid^*, \mathbf{w^*}), \ \mathrm{if} \ \psi_{chk}  \\
\bot, \ \mathrm{otherwise} \\
\end{cases}$$
where $\psi_{chk}$ is true if and only if
\begin{itemize}
    \item the user's secret key in the attributes is the same as the \textit{usk} in the attributes of that $record$,
    \item there is an identifier $rid^*$ in the attributes. 
\end{itemize}
The platform interacts with the user by running $\mathsf{Issue}_{\mathrm{uacs}}(\textit{cp}p, pk, \psi, sk)\leftrightarrow\mathsf{Receive}_{\mathrm{uacs}}(\textit{cp}p, pk, \psi, \alpha)$ and outputs a $cred^*$ which is hidden from the exchange. 
The user outputs this record $record^*=(rid^*, \mathbf{w^*}, cred^*)$.

The user updates his current \textit{token}. He shows an identifier $id$ and runs a credential update protocol with the exchange on the his \textit{token} $\langle\mathsf{Update}_{\mathrm{uacs}}(\textit{cp}p, pk, \psi, sk), \mathsf{UpdRcv}_{\mathrm{uacs}}(\textit{cp}p, pk, \psi, \alpha\rangle$.
%It includes a check whether the data sent by the user is formed correctly.
The hidden parameter is $\alpha=(usk, id^*, \mathbf{w})$ where $id'$ is chosen randomly by the user, $\mathbf{w}$ is the history details of asset $i$. The update function is 

$$\psi((usk, id, \mathbf{\textit{cp}}),\alpha) = \begin{cases}
(usk, id', \mathbf{\textit{cp}}), \ \mathrm{if} \ \psi_{chk}  \\
\bot, \ \mathrm{otherwise} \\
\end{cases}$$
where %$\mathbf{v^*}=(v_1,\dots,v_i-k_i,\dots,v_j+k_j, \dots, v_n)$ and 
$\mathbf{\textit{cp}^*}=f(\mathsf{exchange}, \mathbf{w}, \mathbf{\textit{cp}}, i, k_i)$.
$\psi_{chk}$ is true if and only if
\begin{itemize}
    \item the revealed $id$ is the identifier in the credential,
    %\item the $i$th asset is enough, i.e., $v_i\geq k_i$, 
    %\item this exchange is consistent with the record $\mathbf{w}$, e.g., the record value is enough, $w_i\geq k_i$,
    \item there is a new identifier $id'$ in the credential,
    \item the $\mathbf{\textit{cp}'}$ is well-formed.
\end{itemize}
The user outputs a $cred'$ and his new token $token'=(id', \mathbf{v'}, \mathbf{\textit{cp}'}, cred')$.

\noindent{$Rd_{wit}\leftarrow\langle\mathsf{Withdraw}(epp,pk,usk,req_{wit},\{Rd\}), \mathsf{Deduct}(epp,pk,sk)\rangle\rightarrow b$}:



The user chooses the records $\{Rd\}=\{\textit{token},\textit{record}_i\}$ and a withdraw request $req_{wit}=(\textit{withdraw},i,k_i)$. 
The platform receives the deduct request $req_{ded}=(\textit{Deduct}, i, k_i, id, dsid)$ and checks that $id\notin \mathsf{ID}$ and $dsid \notin \mathsf{ID}$. 
If any of the checks does not pass, the platform outputs $b=0$ and aborts. 
Otherwise, the two parties updates the record token $\textit{record}_i$ and the global token \textit{token} by $\textit{record}_i'\leftarrow\mathsf{UpdRcv}_{uacs}(\textit{cp}p,pk,\psi_0,\alpha_0,\textit{record}_i)\leftrightarrow \mathsf{Update}_{uacs}(\textit{cp}p,pk,\psi_0,sk)\rightarrow b_0$,
$\textit{token}'\leftarrow\mathsf{UpdRcv}_{uacs}(\textit{cp}p,pk,\psi_1,\alpha_1,\textit{token})\leftrightarrow \mathsf{Update}_{uacs}(\textit{cp}p,pk,\psi_1,sk) \rightarrow b_1$, where the hidden parameters $\alpha_0=(dsid^*,open_0^*), \alpha_1=(id^*, open_1^*)$ where $dsid^*,id^*$ are randomly chosen from $\mathbb{Z}_p$ and $open_0^*, open_1^*$ are randomnesses. 
The update function $\psi_0$ and $\psi_1$ are the same as them described in $\langle\mathsf{Exchange},\mathsf{Update}\rangle$ protocol.

If the platform outputs $b_0\wedge b_1=0$, the withdraw operation fails, and the user output $\bot$. 
Otherwise, the user outputs $Rd_{wit}=(\textit{token}',\textit{record}_i')$ consists of the updated record token $\textit{record}_i'$ on attributes $(usk,dsid^*,\mathbf{w}^*)$, and the updated global token $\textit{token}'$ on attributes $(usk,id^*,\mathbf{\textit{cp}}^*)$,  and the platform adds $id, dsid$ to the set $\mathsf{ID}$.

\fi


\iffalse
Otherwise, the two parties interact to run
$\textit{cred}'\leftarrow\mathsf{UpdRcv}_{\mathrm{ouac}}(\textit{cp}p,pk,\psi^*,\alpha,\textit{record})\leftrightarrow \mathsf{Update}_{\mathrm{ouac}}(\textit{cp}p,pk,\mathcal{F},sk)\rightarrow b$.
The hidden parameter $\alpha=(id')$ where $id'$ is randomly chosen from $\mathbb{Z}_p$.
The update function $\psi^*$ is
$$\psi^*(\textbf{a},\alpha) = \begin{cases}
\textbf{a}', \ \mathrm{if} \ \psi^*_{chk}  \\
\bot, \ \mathrm{otherwise} \\
\end{cases}$$
%where $\mathbf{\textit{cp}}^*=f(\mathsf{exchange},\mathbf{w},\mathbf{\textit{cp}},i,k_i)$, 
$\psi^*_{chk}$ is true if and only if
\begin{itemize}
    \item the revealed $id$ is the identifier of $\textit{token}$;
    \item $\psi^*\in\mathcal{F}$;
    \item an old record of asset $i$ is chosen from \textbf{a} with enough value $v_i\geq k_i$ and it is updated to $v_i-k_i $;
    %\item the new record of asset $j$ with value $k_j$ is added to $\textbf{a}'$;
    \item the compliance information is updated correctly in $\textbf{a}'$;
    %\item the $\textit{token}$ shares the same \textit{usk} with the $\textit{record}_i$,
    \item there is a new identifier $id'$ in the credential.
\end{itemize}
\fi



\iffalse
 
\noindent$\bullet$ \textbf{Withdraw}:
The user wants to withdraw one asset $i$ to the real world with his latest \textit{token} and the \textit{record} for that asset $i$.
If it successes, the user gets the updated $token^*$, $record^*$.
During the interaction, the user shows the identifiers $id, rid$ and they run $\langle\mathsf{Withdraw}(epp, pk, f, i, k, usk, token, record), \mathsf{Deduct}(epp, pk, f, i, k, id, rid, sk)\rangle$. 
It consists of updating \textit{token} and \textit{record} for asset \textit{i}. %It works as follows.

The user updates the \textit{record} used in withdrawing.
He shows an identifier $rid$ and run a credential update protocol with the platform on the \textit{record}: $\mathsf{Update}_{\mathrm{uacs}}(\textit{cp}p, pk, \psi, sk)\leftrightarrow\mathsf{UpdRcv}_{\mathrm{uacs}}(\textit{cp}p, pk, \psi, \alpha)$.
It includes a check whether the data sent by the user is formed correctly.
The hidden parameter is $\alpha=(rid',open')$ where $id', open'$ are chosen randomly by the user. The update function is 

$$\psi((usk, rid, \mathbf{w}),\alpha) = \begin{cases}
(usk, rid', \mathbf{w'}), \ \mathrm{if} \ \psi_{chk}  \\
\bot, \ \mathrm{otherwise} \\
\end{cases}$$
where $\mathbf{w'}=(i,v_i-k,px_i)$ 
%and $\mathbf{q^*}=f(\mathsf{withdraw}, \mathbf{q}, i, k)$.
$\psi_{chk}$ is true if and only if
\begin{itemize}
    \item the revealed $rid$ is the identifier in the credential,
    \item the \textit{record} shares the same \textit{usk} with that \textit{token},
    \item the record value is enough, i.e., $v_i\geq k_i$,
    \item there is a new identifier $rid'$ in the credential,
    %\item the $\mathbf{q^*}$ is well-formed.
\end{itemize}
The user outputs a $cred'$ and the updated $record'=(rid', \mathbf{w'}, cred')$.


The user updates his current \textit{token}. He shows an identifier $id$ and runs a credential update protocol with the platform on the \textit{token}: $\mathsf{Update}_{\mathrm{uacs}}(\textit{cp}p, pk, \psi, sk)\leftrightarrow\mathsf{UpdRcv}_{\mathrm{uacs}}(\textit{cp}p, pk, \psi, \alpha)$.
It includes a check whether the data sent by the user is formed correctly.
The hidden parameter is $\alpha=(id', open', px_i)$ where $id', open'$ are chosen randomly by the user, $px_i$ is the buying price of asset $i$ in \textit{record}. The update function is 

$$\psi((usk, id, \mathbf{px}),\alpha) = \begin{cases}
(usk, id', \mathbf{px'}), \ \mathrm{if} \ \psi_{chk}  \\
\bot, \ \mathrm{otherwise} \\
\end{cases}$$
where %$\mathbf{v^*}=(v_1,\dots,v_i-k,\dots, v_n)$ and 
$\mathbf{px'}=f(\mathsf{withdraw}, px_i, \mathbf{px}, i, k_i)$.
$\psi_{chk}$ is true if and only if
\begin{itemize}
    \item the revealed $id$ is the identifier in the credential,
    %\item the $i$th asset is enough, i.e., $v_i\geq k$, 
    \item this withdraw is consistent with the record $\mathbf{w}$, e.g., the record value is enough, $v_i\geq k_i$, 
    \item there is a new identifier $id^*$ in the credential,
    \item the $\mathbf{px'}$ is well-formed.
\end{itemize}
The user outputs a $cred'$ which is hidden from the exchange and his new token $token'=(id', \mathbf{\textit{cp}'}, cred')$.

 
\noindent$\bullet$ \textbf{Request}:
The user also needs to request the platform to authenticate the compliance information of its token. %The user shows the token $id$, $upk$  and interacts with the platform.
%The exchange verifies the correctness of these data and update his token.
These parties run $\mathsf{File}(epp, pk, f, id, upk, id^*, usk, token)\leftrightarrow \mathsf{Sign}(epp, pk, f, id, upk, sk)$. 
It works as follows.

The user shows an identifier $id$, its $upk$. 
It runs a credential update protocol with the platform on the its current \textit{token} $\mathsf{Update}_{\mathrm{uacs}}(\textit{cp}p, pk, \psi, sk)\leftrightarrow\mathsf{UpdRcv}_{\mathrm{uacs}}(\textit{cp}p, pk, \psi, \alpha)$.
It includes a check whether the data sent by the user is formed correctly.
The hidden parameter is $\alpha=(id^*,open^*)$ where $id^*, open^*$ are chosen randomly by the user. The update function is 

$$\psi((usk, id,  \mathbf{\textit{cp}}),\alpha) = \begin{cases}
(usk, id^*, \mathbf{\textit{cp}^*}), \ \mathrm{if} \ \psi_{chk}  \\
\bot, \ \mathrm{otherwise} \\
\end{cases}$$
where $\mathbf{\textit{cp}^*}=f(\mathsf{reveal}, \mathbf{\textit{cp}})$.
$\psi_{chk}$ is true if and only if
\begin{itemize}
    \item the revealed $id$ is the identifier in the credential,
    \item there is compliance attributes \textbf{\textit{cp}} in the credential;% satisfies some check function:...,
    \item there is a new identifier $id^*$ in the credential,
    \item the $\mathbf{\textit{cp}^*}$ is well-formed.
\end{itemize}

The user outputs a $cred^*$ which is hidden from the exchange and his new token $token^*=(id^*, \mathbf{\textit{cp}^*},cred^*)$.
\fi
\end{comment}


\iffalse
\begin{remark}
%\tian{add security intuitions and high level proof outline}

In the exchange transaction, the exchange content is concealed and the user needs to prove the exchange is fair and the profit is calculated correctly according to the prices of the involved assets. 
Otherwise, the overdraft prevention and compliance properties cannot be guaranteed. 
%To make sure the user uses
%The fairness and correctness rely on
Note that the related prices should also be hidden. %which requires additional proofs.
An intuitive idea is using one-out-of-many style proof\cite{Groth2015} but it is still heavy (linear parameter, logarithmic proof size and superlinear generation time and linear verification time).
To improve it, we add authentication on the price and achieves constant proof size and verification time.
The user proves that the exchange is fair and the profit is computed correctly and prices bind with the assets and these binding relationships have been authenticated by the platform.
\end{remark}
\fi


 
\noindent{\bf Extended compliance support.}\ 
Our construction also easily supports other regulation policies. 
We just give sketches here due to the page limitation.
For example, AML requires that users cannot exchange or withdraw too many times in a time period.
It can be achieved by adding a counter in the registration record.
In each exchange or withdraw transaction, the user proves that the counter in his latest registration record is smaller than some value and the counter is credited by one in the newly issued record. 
Other rules are similar, such as transaction amounts, and (total) value of exchanged assets.

We can also enforce tax filing by prohibiting users who have not filed tax last year from exchanging and withdrawing. 
It can be achieved by adding a year number in the registration record indicating the year when the user filed tax last time.
In each exchange or withdraw transaction, the user shows the year number in his latest registration record and this number is credited by one when the user has filed his tax.








\vspace{-0.3cm}	

\subsection{Security analysis}

%\tian{move the formal security proofs from App. XI to Sec. VI.B.}

In this section, we analyze the security of our construction. 



\begin{theorem}[Interaction indistinguishability]
    {If $\Pi_{bs}$ has perfect message privacy and the underlying $\mathsf{ZKAoK}$ is zero-knowledge, then $\Pi_{\mathsf{\name}}$ has interaction indistinguishability.}
\end{theorem}
\vspace{-0.3cm}	

\begin{proof}
We describe a simulation $\mathsf{G}_{\mathrm{sim}}$ in which the adversary $\mathcal{A}$ interacts with the challenger $\mathcal{C}$ as in the $\mathsf{IND}$ experiment.
It differs from $\mathsf{IND}$ that all answers sent to $\mathcal{A}$ are independent with the bit $b$, which means $\mathcal{A}$'s advantage in $\mathsf{G}_{\mathrm{sim}}$ is 0.
Then we will show that $\mathcal{A}$'s advantage in $\mathsf{IND}$ is at most negligibly different from its advantage in $\mathsf{G}_{\mathrm{sim}}$.
\yanan{use $\mathsf{Trans}$. didn't understand why need it?}

\tian{no need Trans}

\noindent$\mathsf{G}_{\mathrm{sim}}$: The simulation $\mathsf{G}_{\mathrm{sim}}$ works as follows.
$\mathcal{C}$ samples $b\in\{0,1\}$ randomly and generates $pp\leftarrow\mathsf{Setup}(1^{\lambda})$ and zero-knowledge trapdoor $\textit{td}\leftarrow\mathsf{Sim}(1^{\lambda})$.
$\mathcal{C}$ sends $pp$ to $\mathcal{A}$ and initializes two sets of oracles $\mathcal{O}^0_{\mathsf{IND}}$ and $\mathcal{O}^1_{\mathsf{IND}}$.
$\mathsf{G}_{\mathrm{sim}}$ proceeds in steps and at each step 
%$\mathcal{C}$ provides 
$\mathcal{A}$ has two transcript lists ($\mathsf{Trans}^{0}$, $\mathsf{Trans}^{1}$).
%, where the left one $\mathsf{Trans}_{L} := \mathsf{Trans}_{b}$ and the right one $\mathsf{Trans}_{R} := \mathsf{Trans}_{1-b}$.
Then each time $\mathcal{A}$ invokes an oracle, it sends $\mathcal{C}$ a pair of queries $(Q^0, Q^1)$.
$\mathcal{C}$ first checks that $Q^0, Q^1$ are \textit{publicly consistent}, then acts differently to simulate different oracles.

\setlist{nolistsep}
\begin{itemize}[noitemsep,leftmargin=*]
    \item[-] For $\mathcal{O}_\mathsf{UKeyGen}$ oracle, $Q^0=Q^1=(u)$. $\mathcal{C}$ generates $(upk, usk) \leftarrow \mathsf{UserKeyGen}(epp)$ and chooses an identity $u$, then $\mathcal{C}$ stores $(usk,u)$ and returns $(u, upk)$ as the answer for $Q^0$ and $Q^1$ to $\mathcal{A}$.
    \item[-] For $\mathcal{O}_\mathsf{Join}$ oracle, $Q^0=(u, upk, \{\mathit{ref}^0\})$ and $Q^1=(u, upk, \{\mathit{ref}\}^1)$. 
To answer $Q^0$, $\mathcal{C}$ behaves as in $\mathsf{IND}$ experiment except the following modification.
It produces commitment $com^0$ on a randomness $r$ and simulates the $\mathsf{ZKAoK}$ proof $\pi$ using $\textit{td}$.
So $\mathit{ts}^0=(com^0,\pi^0)$.
To answer $Q^1$, $\mathcal{C}$ does the same with a fresh randomness $r'$ and produces $\mathit{ts}^1$.
$\mathcal{C}$ replies $\mathcal{A}$ with $(\mathit{ts}^{0}, \mathit{ts}^{1})$. 
If $\mathcal{A}$ accepts the proofs, it runs $\hat{\sigma}^0\leftarrow\mathsf{BlindSign}(pp,pk,com^0)$ and $\hat{\sigma}^{1}\leftarrow\mathsf{BlindSign}(pp,pk,com^{1})$ and sends them to $\mathcal{C}$. 
$\mathcal{C}$ unblinds the signatures and outputs $a^0, a^{1}$ after verifying them indicating whether they are valid signatures.
If $a^0\neq a^1$, outputs $\bot$.% otherwise, adds
%$\mathit{ts}'^0=(\mathit{ts}^0,\hat{\sigma}^0, a^0$) to $\mathsf{Trans}^0$ and $\mathit{ts}'^1=(\mathit{ts}^1,\hat{\sigma}^1,a^1$) to $\mathsf{Trans}^1$.
\item[-] For $\mathcal{O}_{\mathsf{Deposit}}$ oracle, $Q^0=(u, \mathit{req_{dep}}, \{\mathit{ref}\}^{\mathsf{old0}}, \{\mathit{ref}\}^{\mathsf{new}0})$ and $Q^1=(u, \mathit{req_{dep}}, \{\mathit{ref}\}^{\mathsf{old}1}, \{\mathit{ref}\}^{\mathsf{new}1})$. 
To answer $Q^0$, $\mathcal{C}$ behaves as in $\mathsf{IND}$ experiment except the following modification:
It produces commitments $\{com^0\}$ on random inputs and
%sets $(id, usk, cp_1, cp_2)=(0,0,0,0)$ and commits them as $c_1$, sets $(aid, usk, i, v_i, px_i)=(0,0,0,0,0)$ and commits it as $c_2$, 
simulates the $\mathsf{ZKAoK}$ using $\textit{td}$:  $\pi^0_{dep}\leftarrow\mathsf{Sim}(\textit{td}, x)$. %where $x=(c_1, c_2)$
So $\mathit{ts}^0=(\{com^0\}, \pi_{dep}^0)$.
To answer $Q^1$, $\mathcal{C}$ does the same with fresh randomness  and produces $\mathit{ts}^1$.
$\mathcal{C}$ replies $\mathcal{A}$ with $(\mathit{ts}^0, \mathit{ts}^1)$. 
If $\mathcal{A}$ accepts the proofs, it runs the $\mathsf{BlindSign}$ algorithm and sends the respective blinded signatures to $\mathcal{C}$. %$\hat{\sigma}_b\leftarrow\mathsf{BlindSign}_{\mathrm{sig}}(pp,pk,c_b)$ and $\hat{\sigma}_{1-b}\leftarrow\mathsf{BlindSign}_{\mathrm{sig}}(pp,pk,c_{1-b})$ and sends them to $\mathcal{C}$. 
$\mathcal{C}$ unblinds the signatures and outputs $a^0, a^1$ after verifying them.
If $a^0\neq a^1$, outputs $\bot$. %otherwise, adds
%runs $\sigma_b\leftarrow\mathsf{BlindRcv}_{\mathrm{sig}}(pp,pk,\hat{\sigma}_b,0,0,0,r)$ and $a_b \leftarrow\mathsf{Vrfy}_{\mathrm{sig}}(pp,pk,0,0,0,\sigma_b)$, where $a_b=a_{1-b}$.
%It sends $b$ to $\mathcal{A}$.
%$\mathit{ts}'^0=(\mathit{ts}^0$,$\hat{\sigma}^0$, $a^0$) to $\mathsf{Trans}^0$ and $\mathit{ts}'^1=(\mathit{ts}^1$,$\hat{\sigma}^1$, $a^1$) to $\mathsf{Trans}^1$.
\item[-] For $\mathcal{O}_{\mathsf{Exchange}}$ oracle, $Q^0=(u, \mathit{req_{exc}}, \{\mathit{ref}\}^{\mathsf{old0}},$ $\{\mathit{ref}\}^{\mathsf{new0}})$ and $Q^1=(u', \mathit{req_{exc}}', \{\mathit{ref}\}^{\mathsf{old1}},$ 
$\{\mathit{ref}\}^{\mathsf{new1}})$. 
To answer $Q^0$, $\mathcal{C}$ behaves as in $\mathsf{IND}$ experiment except the following modification:
It chooses $rid$ and $aid$ randomly and produces commitments $\{com\}^0$ on random inputs and simulates the $\mathsf{ZKAoK}$ using $\textit{td}$:  $\pi_{exc}^0\leftarrow\mathsf{Sim}(\textit{td}, x)$. 
So $\mathit{ts}^0=(rid^0, aid^0, \{com\}^0, \pi_{exc}^0)$.
To answer $Q^1$, $\mathcal{C}$ does the same with fresh randomnesses and produces $\mathit{ts}^1$.
$\mathcal{C}$ replies $\mathcal{A}$ with $(\mathit{ts}^0, \mathit{ts}^1)$. 
If $\mathcal{A}$ accepts the proofs, it runs the $\mathsf{BlindSign}$ algorithm and sends the blinded signatures to $\mathcal{C}$.  
$\mathcal{C}$ unblinds the signatures and generates $a^0, a^1$ by verifying them.
If $a^0\neq a^1$, outputs $\bot$. %otherwise, adds $\mathit{ts}'^0$=($\mathit{ts}^0$, $\hat{\sigma}^0$ ,$a^0$) to $\mathsf{Trans}^0$ and $\mathit{ts}'^1$=($\mathit{ts}^1$, $\hat{\sigma}^1$ ,$a^1$) to $\mathsf{Trans}^1$.
\item[-] For $\mathcal{O}_{\mathsf{Withdraw}}$ oracle, $Q^0=(u^0, \mathit{req_{wit}}, \{\mathit{ref}\}^{\mathsf{old0}},$ $\{\mathit{ref}\}^{\mathsf{new0}})$ and $Q^1=(u^1, \mathit{req_{wit}}, \{\mathit{ref}\}^{\mathsf{old1}}, \{\mathit{ref}\}^{\mathsf{new1}})$. 
To answer $Q^0$, $\mathcal{C}$ behaves as in $\mathsf{IND}$ experiment except the following modification:
It chooses $rid^0$ and $aid^0$ randomly and produces commitments $\{com\}^0$ on random inputs and
%sets $(rid, usk, cp_1, cp_2)=(0,0,0,0)$ and commits them as $c_1$, sets $(aid, usk, i, v_i, px_i)=(0,0,0,0,0)$ and commits it as $c_2$, sets $(rid, usk, cp_1, cp_2)=(0,0,0,0)$ and commits them as $c_3$, sets $(aid, usk, i, v_i, px_i)=(0,0,0,0,0)$ and commits it as $c_4$, 
simulates the $\mathsf{ZKAoK}$ using $\textit{td}$:  $\pi_{wit}^0\leftarrow\mathsf{Sim}(\textit{td}, x)$. %where $x=(c_1, c_2)$
So $\mathit{ts^0}=(rid^0, aid^0, \{com\}^0, \pi_{wit}^0)$.
To answer $Q^1$, $\mathcal{C}$ does the same with fresh randomnesses and produces $\mathit{ts}^1$.
$\mathcal{C}$ replies $\mathcal{A}$ with $(\mathit{ts}^0, \mathit{ts}^1)$. 
If $\mathcal{A}$ accepts the proofs, it runs the $\mathsf{BlindSign}$ algorithm and sends the blinded signatures to $\mathcal{C}$.  
$\mathcal{C}$ unblinds the signatures and generates $a^0, a^1$ by verifying them.
If $a^0\neq a^1$, outputs $\bot$. % otherwise, adds $\mathit{ts}'^0$=($\mathit{ts}^0$, $\hat{\sigma}^0$ ,$a^0$) to $\mathsf{Trans}^0$ and $\mathit{ts}'^1$=($\mathit{ts}^1$, $\hat{\sigma}^1$ ,$a^1$) to $\mathsf{Trans}^1$.
\item[-] For $\mathcal{O}_{\mathsf{File}}$ oracle, $Q^0=(u, \{\mathit{ref}\}^{\mathsf{old0}}, \{\mathit{ref}\}^{\mathsf{new0}})$ and $Q^1=(u,  \{\mathit{ref}\}^{\mathsf{old1}},$ $\{\mathit{ref}\}^{\mathsf{new1}})$. 
To answer $Q^0$, $\mathcal{C}$ behaves as in $\mathsf{IND}$ experiment except the following modification:
It chooses $rid^0$ randomly and produces commitments $\{com\}^0$ on random inputs and
%sets $(rid, usk, cp_1, cp_2)=(0,0,0,0)$ and commits them as $c_1$, sets $(upk, cp_1, cp_2)=(0,0,0)$ and commits it as $c_2$, sets $(rid, usk, cp_1, cp_2)=(0,0,0,0)$ and commits them as $c_3$,  
simulates the $\mathsf{ZKAoK}$ using $\textit{td}$:  $\pi_{fil}\leftarrow\mathsf{Sim}(\textit{td}, x)$. %where $x=(c_1, c_2)$
So $\mathit{ts}^0=(rid^0, aid^0, \{com\}^0, \pi_{fil}^0)$.
To answer $Q^1$, $\mathcal{C}$ does the same with fresh randomnesses and produces $\mathit{ts}^1$.
$\mathcal{C}$ replies $\mathcal{A}$ with $(\mathit{ts}^0, \mathit{ts}^1)$. 
If $\mathcal{A}$ accepts the proofs, it runs the $\mathsf{BlindSign}$ algorithm and sends the blinded signatures to $\mathcal{C}$.  
$\mathcal{C}$ unblinds the signatures and generates $a^0, a^1$ by verifying them.
If $a^0\neq a^1$, outputs $\bot$. % otherwise, adds $\mathit{ts}'^0$=($\mathit{ts}^0$, $\hat{\sigma}^0$ ,$a^0$) to $\mathsf{Trans}^0$ and $\mathit{ts}'^1$=($\mathit{ts}^1$, $\hat{\sigma}^1$ ,$a^1$) to $\mathsf{Trans}^1$.
   
\end{itemize}




In each of the above cases, the response to $\mathcal{A}$ is independent of $b$. 
Thus, when $\mathcal{A}$ outputs a guess $\hat{b}$, its advantage in $\mathsf{G}_{\mathrm{sim}}$ is 0 since all transcripts $\mathit{ts}^0, \mathit{ts}^1$ are independent of $b$.

Then we describe a sequence of hybrid experiments $(\mathsf{G}_{\mathrm{real}}, \mathsf{G}_{\mathrm{1}},
%\mathsf{G}_{\mathrm{2}}, 
%\mathsf{G}_{\mathrm{3}}, 
\mathsf{G}_{\mathrm{sim}})$ as follows.\\
\noindent$\mathsf{G}_{\mathrm{real}}$: It is the original $\mathsf{IND}$ experiment.\\
\noindent$\mathsf{G}_{1}$:
This experiment modifies $\mathsf{G}_{\mathrm{real}}$ by simulating the $\mathsf{ZKAoK}$ proof. 
It works as follows:
at the beginning, $\mathcal{C}$ generates the zero-knowledge trapdoor $\textit{td}\leftarrow\mathsf{Sim}(1^{\lambda})$.
In the following oracle queries, $\mathcal{C}$ generates proof using $\textit{td}$: $\pi\leftarrow\mathsf{Sim}(\textit{td}, x)$.\\
\noindent$\mathsf{G}_{\mathrm{sim}}$: It has been described above.
This experiment modifies $\mathsf{G}_{1}$ by replacing the original commitments by commitments on random strings.

In the real $\mathsf{IND}$ experiment, the adversary $\mathcal{A}$ wins if it can distinguish the transcripts with overwhelming probability. 
Due to that the blind signature has perfect message privacy and the underlying $\mathsf{ZKAoK}$ is zero-knowledge, each adjacent experiments can be distinguished with only negligible probability.
Thus $\mathsf{G}_{\mathrm{sim}}$ can be distinguished from ${\mathsf{IND}}$ experiment with only negligible probability.
Since $\mathcal{A}$ wins in $\mathsf{G}_{\mathrm{sim}}$ with probability 1/2, its advantage in ${\mathsf{IND}}$ is negligible.
\end{proof}


\iffalse
\noindent\textit{Proof sketch.} 
In the interaction of join, deposit, exchange, withdraw and file, the user sends committed messages with zero-knowledge proof to the platform for blind signature.
He only shows some unused identifiers which are randomly chosen before. 
Since the blind signature has perfect message privacy and the underlying $\mathsf{ZKAoK}$ is zero-knowledge, the interaction does not leak any other things except for the public information, so the adversary cannot distinguish when the public information are the same.
\fi

\iffalse
\begin{proof}
We describe a simulation $\mathsf{G}_{\mathrm{sim}}$ in which the adversary $\mathcal{A}$ interacts with the challenger $\mathcal{C}$ as in the $\mathsf{IND}$ experiment.
It differs from $\mathsf{IND}$ that all answers sent to $\mathcal{A}$ are independent with the bit $b$, which means $\mathcal{A}$'s advantage in $\mathsf{G}_{\mathrm{sim}}$ is 0.
Then we will show that $\mathcal{A}$'s advantage in $\mathsf{IND}$ is at most negligibly different from its advantage in $\mathsf{G}_{\mathrm{sim}}$.

\noindent$\mathsf{G}_{\mathrm{sim}}$: The simulation $\mathsf{G}_{\mathrm{sim}}$ works as follows.
$\mathcal{C}$ samples $b\in\{0,1\}$ randomly and generates $pp\leftarrow\mathsf{Setup}(1^{\lambda})$ and zero-knowledge trapdoor $td\leftarrow\mathsf{Sim}(1^{\lambda})$.
$\mathcal{C}$ sends $pp$ to $\mathcal{A}$ and initializes two sets of oracles $\mathcal{O}^0$ and $\mathcal{O}^1$.
$\mathsf{G}_{\mathrm{sim}}$ proceeds in steps and at each step $\mathcal{C}$ provides $\mathcal{A}$ with two transcript lists ($\mathsf{Trans}_{L}$, $\mathsf{Trans}_{R}$), where the left one $\mathsf{Trans}_{L} := \mathsf{Trans}_{b}$ and the right one $\mathsf{Trans}_{R} := \mathsf{Trans}_{1-b}$.
Then each time $\mathcal{A}$ invokes a kind of oracle, it sends $\mathcal{C}$ a pair of queries $(Q, Q')$.
$\mathcal{C}$ first checks that $Q, Q'$ are \textit{publicly consistent}, then acts differently on different oracles.
%forwards $Q$ to the oracle in $\mathcal{O}^0$ and forwards $Q'$ to the oracle in $\mathcal{O}^1$. The oracles' outputs are the transcripts $\mathsf{ts}^0,\mathsf{ts}^1$. $\mathcal{C}$ replies $\mathcal{A}$ with $\mathsf{ts}^b,\mathsf{ts}^{1-b}$.

For \textbf{UserKeyGen} oracle, $Q=Q'=(u)$. 

$\mathcal{C}$ generates $(upk, usk) \leftarrow \mathsf{UserKeyGen}(epp)$ and chooses an identity $u$, then $\mathcal{C}$ stores $(usk,u)$ and returns $(u, upk)$ as the answer for $Q$ and $Q'$ to $\mathcal{A}$.

For \textbf{Join} oracle, $Q=(u, upk, \{\mathsf{idx}\})$ and $Q'=(u, upk, \{\mathsf{idx}\}')$. 

To answer $Q$, $\mathcal{C}$ behaves as in $\mathsf{IND}$ experiment except the following modification.
It sets $(id, usk, \textit{cp}_1, \textit{cp}_2)=(0,0,0)$ and commits them as $c=\mathsf{Com}_{\mathrm{sig}}(pp,pk,0,0,0,r)$ with random $r$ and simulates the $\mathsf{ZKAoK}$ proof $\pi$ using $td$.
So $ts_0=(c,\pi)$.
To answer $Q'$, $\mathcal{C}$ does the same with a fresh randomness $r'$ and produces $ts_1$.
$\mathcal{C}$ replies $\mathcal{A}$ with $(ts_b, ts_{1-b})$. 
If $\mathcal{A}$ accepts the proofs, it runs $\hat{\sigma}_b\leftarrow\mathsf{BlindSign}_{\mathrm{sig}}(pp,pk,c_b)$ and $\hat{\sigma}_{1-b}\leftarrow\mathsf{BlindSign}_{\mathrm{sig}}(pp,pk,c_{1-b})$ and sends them to $\mathcal{C}$. 
$\mathcal{C}$ runs $\sigma_b\leftarrow\mathsf{BlindRcv}_{\mathrm{sig}}(pp,pk,\hat{\sigma}_b,0,0,0,r)$ and $a_b \leftarrow\mathsf{Vrfy}_{\mathrm{sig}}(pp,pk,0,0,0,\sigma_b)$, where $a_b=a_{1-b}$.
%It sends $b$ to $\mathcal{A}$.
Finally, $ts_b'$=($ts_b$, $a_b$) are added to $\mathsf{Trans}_{L}$.


For \textbf{Deposit} oracle, $Q=(u, req_{dep}, \{\mathsf{idx}\}^{\mathsf{old}}, \{\mathsf{idx}\}^{\mathsf{new}})$ and $Q'=(u, req_{dep}, \{\mathsf{idx}\}^{\mathsf{old}'}, \{\mathsf{idx}\}^{\mathsf{new}'})$ 

To answer $Q$, $\mathcal{C}$ behaves as in $\mathsf{IND}$ experiment except the following modification:
It sets $(id, usk, \textit{cp}_1, \textit{cp}_2)=(0,0,0,0)$ and commits them as $c_1$, sets $(aid, usk, i, v_i, px_i)=(0,0,0,0,0)$ and commits it as $c_2$, simulates the $\mathsf{ZKAoK}$ using $td$:  $\pi_{dep}\leftarrow\mathsf{Sim}(td, x)$. %where $x=(c_1, c_2)$
So $ts_0=(c_1, c_2, \pi_{dep})$.
To answer $Q'$, $\mathcal{C}$ does the same with a fresh randomness $r'$ and produces $ts_1$.
$\mathcal{C}$ replies $\mathcal{A}$ with $(ts_b, ts_{1-b})$. 
If $\mathcal{A}$ accepts the proofs, it runs the $\mathsf{BlindSign}$ algorithm and sends the blinded signatures to $\mathcal{C}$. %$\hat{\sigma}_b\leftarrow\mathsf{BlindSign}_{\mathrm{sig}}(pp,pk,c_b)$ and $\hat{\sigma}_{1-b}\leftarrow\mathsf{BlindSign}_{\mathrm{sig}}(pp,pk,c_{1-b})$ and sends them to $\mathcal{C}$. 
$\mathcal{C}$ unblinds the signatures and generates $a_b, a_{1-b}$ by verifying them.
If $a_b\neq a_{1-b}$, outputs $\bot$, otherwise, adds
%runs $\sigma_b\leftarrow\mathsf{BlindRcv}_{\mathrm{sig}}(pp,pk,\hat{\sigma}_b,0,0,0,r)$ and $a_b \leftarrow\mathsf{Vrfy}_{\mathrm{sig}}(pp,pk,0,0,0,\sigma_b)$, where $a_b=a_{1-b}$.
%It sends $b$ to $\mathcal{A}$.
$ts'_b$=($ts_b$, $a_b$) to $\mathsf{Trans}_{L}$ and $ts'_{1-b}$=($ts_{1-b}$, $a_{1-b}$) to $\mathsf{Trans}_{R}$.

% If $\mathcal{A}$ accepts, it runs $\hat{\sigma}\leftarrow\mathsf{BlindSign}_{\mathrm{sig}}(pp,pk,c_2)$ and sends it to $\mathcal{C}$. 
% $\mathcal{C}$ runs $\sigma\leftarrow\mathsf{BlindRcv}_{\mathrm{sig}}(pp,pk,\hat{\sigma},0,0,0,r)$ and $b \leftarrow\mathsf{Vrfy}_{\mathrm{sig}}(pp,pk,0,0,0,\sigma)$.
% %It sends $b$ to $\mathcal{A}$.
% Finally, ($c_1, c_2$, $\hat{\sigma}, \pi$, $b$) are added to $\mathsf{Trans}_{L}$.
% To answer $Q'$, $\mathcal{C}$ does the same.




For \textbf{Exchange} oracle, $Q=(u, req_{exc}, \{\mathsf{idx}\}^{\mathsf{old}}, \{\mathsf{idx}\}^{\mathsf{new}})$ and $Q'=(u', req'_{exc}, \{\mathsf{idx}\}^{\mathsf{old}'}, \{\mathsf{idx}\}^{\mathsf{new}'})$ 

%To answer $Q$, $\mathcal{C}$ behaves as in IND experiment except that it chooses an identifier $id$ randomly and runs $\mathcal{S}_{\mathrm{UpdRcv}}(td, pk)$.

%To answer $Q'$, $\mathcal{C}$ chooses another $id'$ and does the same.

To answer $Q$, $\mathcal{C}$ behaves as in $\mathsf{IND}$ experiment except the following modification:
It chooses $rid$ and $aid$ randomly and sets $(rid, usk, \textit{cp}_1, \textit{cp}_2)=(0,0,0,0)$ and commits them as $c_1$, sets $(aid, usk, i, v_i, px_i)=(0,0,0,0,0)$ and commits it as $c_2$, sets $(rid, usk, \textit{cp}_1, \textit{cp}_2)=(0,0,0,0)$ and commits them as $c_3$, sets $(aid, usk, i, v_i, px_i)=(0,0,0,0,0)$ and commits it as $c_4$, sets $(aid, usk, j, v_j, px_j)=(0,0,0,0,0)$ and commits it as $c_5$, simulates the $\mathsf{ZKAoK}$ using $td$:  $\pi_{dep}\leftarrow\mathsf{Sim}(td, x)$. %where $x=(c_1, c_2)$
So $ts_0=(rid, aid, c_1, c_2, c_3, c_4, c_5, \pi_{dep})$.
To answer $Q'$, $\mathcal{C}$ does the same with fresh randomnesses and produces $ts_1$.
$\mathcal{C}$ replies $\mathcal{A}$ with $(ts_b, ts_{1-b})$. 
If $\mathcal{A}$ accepts the proofs, it runs the $\mathsf{BlindSign}$ algorithm and sends the blinded signatures to $\mathcal{C}$.  
$\mathcal{C}$ unblinds the signatures and generates $a_b, a_{1-b}$ by verifying them.
If $a_b\neq a_{1-b}$, outputs $\bot$, otherwise, adds $ts'_b$=($ts_b$, $a_b$) to $\mathsf{Trans}_{L}$ and $ts'_{1-b}$=($ts_{1-b}$, $a_{1-b}$) to $\mathsf{Trans}_{R}$.



For \textbf{Withdraw} oracle, $Q=(u, req_{wit}, \{\mathsf{idx}\}^{\mathsf{old}}, \{\mathsf{idx}\}^{\mathsf{new}})$ and $Q'=(u', req_{wit}, \{\mathsf{idx}\}^{\mathsf{old}'}, \{\mathsf{idx}\}^{\mathsf{new}'})$ 


To answer $Q$, $\mathcal{C}$ behaves as in $\mathsf{IND}$ experiment except the following modification:
It chooses $rid$ and $aid$ randomly and sets $(rid, usk, \textit{cp}_1, \textit{cp}_2)=(0,0,0,0)$ and commits them as $c_1$, sets $(aid, usk, i, v_i, px_i)=(0,0,0,0,0)$ and commits it as $c_2$, sets $(rid, usk, \textit{cp}_1, \textit{cp}_2)=(0,0,0,0)$ and commits them as $c_3$, sets $(aid, usk, i, v_i, px_i)=(0,0,0,0,0)$ and commits it as $c_4$, simulates the $\mathsf{ZKAoK}$ using $td$:  $\pi_{dep}\leftarrow\mathsf{Sim}(td, x)$. %where $x=(c_1, c_2)$
So $ts_0=(rid, aid, c_1, c_2, c_3, c_4, \pi_{dep})$.
To answer $Q'$, $\mathcal{C}$ does the same with fresh randomnesses and produces $ts_1$.
$\mathcal{C}$ replies $\mathcal{A}$ with $(ts_b, ts_{1-b})$. 
If $\mathcal{A}$ accepts the proofs, it runs the $\mathsf{BlindSign}$ algorithm and sends the blinded signatures to $\mathcal{C}$.  
$\mathcal{C}$ unblinds the signatures and generates $a_b, a_{1-b}$ by verifying them.
If $a_b\neq a_{1-b}$, outputs $\bot$, otherwise, adds $ts'_b$=($ts_b$, $a_b$) to $\mathsf{Trans}_{L}$ and $ts'_{1-b}$=($ts_{1-b}$, $a_{1-b}$) to $\mathsf{Trans}_{R}$.


%To answer $Q$, $\mathcal{C}$ behaves as in IND experiment except that it chooses an identifier $id$ randomly and runs $\mathcal{S}_{\mathrm{UpdRcv}}(td, pk)$.

%To answer $Q'$, $\mathcal{C}$ does the same.



For \textbf{Request} oracle, $Q=(u, \{\mathsf{idx}\}^{\mathsf{old}}, \{\mathsf{idx}\}^{\mathsf{new}})$ and $Q'=(u,  \{\mathsf{idx}\}^{\mathsf{old}'}, \{\mathsf{idx}\}^{\mathsf{new}'})$ 

%To answer $Q$, $\mathcal{C}$ behaves as in IND experiment except that it chooses a uniformly random identifier $id$ and generates a commitment $\mathsf{cm}$ on a random input and runs $\mathcal{S}_{\mathrm{UpdRcv}}(td, pk)$.

%To answer $Q'$, $\mathcal{C}$ does the same except that chooses another uniformly random identifier $id'$ and generates a commitment $\mathsf{cm}'$ on another random input.


To answer $Q$, $\mathcal{C}$ behaves as in $\mathsf{IND}$ experiment except the following modification:
It chooses $rid$ randomly and sets $(rid, usk, \textit{cp}_1, \textit{cp}_2)=(0,0,0,0)$ and commits them as $c_1$, sets $(upk, \textit{cp}_1, \textit{cp}_2)=(0,0,0)$ and commits it as $c_2$, sets $(rid, usk, \textit{cp}_1, \textit{cp}_2)=(0,0,0,0)$ and commits them as $c_3$,  simulates the $\mathsf{ZKAoK}$ using $td$:  $\pi_{dep}\leftarrow\mathsf{Sim}(td, x)$. %where $x=(c_1, c_2)$
So $ts_0=(rid, aid, c_1, c_2, c_3, \pi_{dep})$.
To answer $Q'$, $\mathcal{C}$ does the same with fresh randomnesses and produces $ts_1$.
$\mathcal{C}$ replies $\mathcal{A}$ with $(ts_b, ts_{1-b})$. 
If $\mathcal{A}$ accepts the proofs, it runs the $\mathsf{BlindSign}$ algorithm and sends the blinded signatures to $\mathcal{C}$.  
$\mathcal{C}$ unblinds the signatures and generates $a_b, a_{1-b}$ by verifying them.
If $a_b\neq a_{1-b}$, outputs $\bot$, otherwise, adds $ts'_b$=($ts_b$, $a_b$) to $\mathsf{Trans}_{L}$ and $ts'_{1-b}$=($ts_{1-b}$, $a_{1-b}$) to $\mathsf{Trans}_{R}$.



In each of the above cases, the response to $\mathcal{A}$ is computed independently of the bit $b$. 
Thus, when $\mathcal{A}$ outputs a guess $b'$, its advantage in $\mathsf{G}_{\mathrm{sim}}$ is 0.

Then we describe a sequence of hybrid experiments $(\mathsf{G}_{\mathrm{real}}, \mathsf{G}_{\mathrm{1}},\mathsf{G}_{\mathrm{2}}, \mathsf{G}_{\mathrm{3}}, \mathsf{G}_{\mathrm{sim}})$.
In each experiment, the challenger $\mathcal{C}$ modifies them one by one.
%Here the $\mathsf{G}_{\mathrm{real}}$ is the original $\mathsf{IND}$ experiment and $\mathsf{G}_{\mathrm{sim}}$ 


\noindent$\mathsf{G}_{\mathrm{real}}$: It is the original $\mathsf{IND}$ experiment.

\noindent$\mathsf{G}_{1}$:
This experiment modifies $\mathsf{G}_{\mathrm{real}}$ by simulating the $\mathsf{ZKAoK}$ proof. 
It works as follows:
at the beginning, $\mathcal{C}$ generates the zero-knowledge trapdoor $td\leftarrow\mathsf{Sim}(1^{\lambda})$.
for \textbf{Join} and 
for \textbf{Deposit} oracles.


\noindent$\mathsf{G}_{2}$:
This experiment modifies $\mathsf{G}_{1}$ by choosing an identifier $id$ randomly and simulating the $\Pi_{\mathrm{ouac}}$ in \textbf{Exchange} and \textbf{Withdraw} oracles.


\noindent$\mathsf{G}_{\mathrm{sim}}$: It has been described above.
This experiment modifies $\mathsf{G}_{2}$ replacing the commitment in \textbf{Request} oracle by commitments on random strings.

In the real $\mathsf{IND}$ experiment, the adversary $\mathcal{A}$ wins if it can distinguish the transcripts with overwhelming probability. 

%In the challenge phase, the adversary can also query the request oracle. 

%For X = $\mathsf{Deposit}$: due to the simulation anonymity of $\Pi_{\mathrm{uacs}}$, everything that $\mathcal{A}$ sees perfectly hides the user’s secret \textit{usk} and \textit{id}.

%Due to the simulation privacy of $\Pi_{\mathrm{ouac}}$, the user’s secret \textit{usk}, $\textit{record}$ and the update function $\phi^*$ are hidden from $\mathcal{A}$. It gets nothing except the public information.


%the deduct request $req_{ded}=(\textit{Deduct}, i, k_i, id, dsid)$ additionally which is independent of $b$.
%The $id, dsid$ are hidden in the past update operation of $\Pi_{uacs}$.

When $\mathcal{A}$ queries the \textbf{Request} oracle and generates signature on the user's compliance information.
However, they run a blind signature protocol to compute such signature. 
%and it just gets the commitment of the compliance value.
Due to the perfect message privacy of the blind signature, $\mathcal{A}$ cannot get any information of the compliance information, thus it does not help to distinguish.

\end{proof}
\fi

\iffalse
\begin{theorem}[Withdraw Anonymity]
    {If $\Pi_{\mathrm{uacs}}$ has simulation anonymity and the blind signature has perfect message privacy, then $\Pi_{\mathrm{\name}}$ has withdraw anonymity.}

\end{theorem}

\begin{proof}
In the withdraw anonymity experiment of $\Pi_{\mathrm{\name}}$, the adversary $\mathcal{A}$ wins if it can distinguish the users $u_0$ and $u_1$ with overwhelming probability. 


Due to the simulation anonymity of $\Pi_{\mathrm{uacs}}$, the user’s secret \textit{usk} and the new $\textit{id}^*, \textit{dsid}^*$ are hidden from the adversary $\mathcal{A}$. 
It only gets the deduct request $req_{ded}=(\textit{Deduct}, i, k_i, id, dsid)$ additionally which is independent of $b$.
The $id, dsid$ are hidden in the past update operation of $\Pi_{uacs}$.

In the challenge phase, $\mathcal{A}$ can also query the request oracle and generates signature on the user's compliance information.
However, they run a blind signature protocol to get such signature.
Due to the perfect message privacy of the blind signature, $\mathcal{A}$ cannot get any information of the compliance information, thus it does not help to distinguish.

%For X = $\mathsf{Withdraw}$: everything that the adversary $\mathcal{A}$ sees perfectly hides the user’s secret \textit{usk} and \textit{id}. $\mathcal{A}$ only gets the old \textit{id} additionally which is independent of $b$.

\end{proof}

\fi



\begin{theorem}[Overdraft prevention]
    If the underlying $\mathsf{ZKAoK}$ has proof of knowledge, the commitment is binding and  $\Pi_{bs}$ is unforgeable, then $\Pi_{\mathsf{\name}}$ has overdraft prevention.
\end{theorem}

\vspace{-0.3cm}	


\begin{proof}
In the overdraft prevention experiment, the adversary $\mathcal{A}$ wins if it 
%is infeasible to extract a consistent list of transaction history and 
withdraws more asset than it has deposited or exchanged.
It means there exists at least one transaction $h_t=(u, \{Rd\}, \{Rd\}', \mathit{ts_t},\mathit{pub_t})$, where $t\in[N]$, such that one of the following events happens:\\
%\noindent(1) It is not a join transaction and the user identity has not registered: $u\notin \mathsf{RU}$ and $\mathsf{Join}\notin\mathsf{Req}$;\\
\noindent(1) The records used in this transaction were not generated from previous transactions: $\{Rd\}\not\subseteq \mathsf{RdSet}$ and $\mathsf{RdSet}\neq\emptyset$;\\
\noindent(2) The asset record is wrong in the following cases: \\
\textit{Deposit}: $\mathit{Rd_{ast}}(\textit{{kind}}) \neq \mathit{ts_t}(\mathit{kind})$ or $\mathit{Rd_{ast}}(\textit{{amt}}) \neq \mathit{ts_t}(\mathit{amt})$;\\
\textit{Exchange}: $\mathit{Rd'_{ast_i}}(\textit{{kind}}) \neq \mathit{Rd_{ast_i}}(\mathit{kind})$ {or} $\mathit{Rd'_{ast}}(\textit{{amt}}) <0;$\\
\textit{Withdraw}: $\mathit{Rd_{ast}}(\textit{{kind}}) \neq \mathit{ts_{t}}(\mathit{kind}) \ \mathrm{or}\ \mathit{Rd'_{ast}}(\textit{{amt}}) <0$ or  $\mathit{Rd_{ast}(amt)}-\mathit{Rd'_{ast}(amt)}<\mathit{ts_{t}(amt)}$;\\
\noindent(3) It is an unfair exchange:
\vspace{-0.2cm}
$$(\mathit{Rd_{ast_i}}(\textit{amt})-\mathit{Rd'_{ast_i}}(\textit{amt}))\cdot \mathit{pub_t(i)} \neq \mathit{Rd_{ast_j}}(\textit{amt})\cdot \mathit{pub_t(j)}$$


The security of our scheme can be reduced to the underlying cryptographic building blocks. 
This includes standard primitives like commitment, blind signature, and non-interactive $\mathsf{ZKAoK}$.
We elaborate it case by case. \\
\noindent(1) 
Suppose that Pr[$\mathcal{A}$ wins and violates condition 1] is non-negligible. In this case, it leads to at least one of the following contradictions: 
\vspace{-0.2cm}
\setlist{nolistsep}
\begin{itemize}[noitemsep,leftmargin=*]
    \item $\mathcal{A}$ does not know the $usk$ of $u$ in the commitments but generates a valid proof, which breaks the soundness of underlying $\mathsf{ZKAoK}$; 
    \item The records in $\{Rd\}$ are valid but were not generated via querying oracles, which breaks the unforgeability of the blind signature; 
    \item The asset record in $\{Rd\}$ has been used before, in this case, since the used identifier would be detected, the revealed identifiers must be different $aid \neq aid'$ which means one commitment produces two different openings. This contradicts the binding property of the commitment scheme. 
\end{itemize}
%$\mathcal{A}$ violates condition 3: 
\vspace{-0.2cm}
\noindent(2) 
Suppose that Pr[$\mathcal{A}$ wins and violates condition 2] is non-negligible. 
In this case, \adv\ generates a valid transaction but gets asset records with wrong attributes.
\iffalse
with an asset record where in the commitment
$\mathsf{Req.in.kind}\neq \mathsf{RdAsset.kind}$ or $\mathsf{Req.in.amt}> \mathsf{RdAsset.amt}$. But it generates a valid proof that $\mathsf{Req.in.kind} = \mathsf{RdAsset.kind}$ and $\mathsf{RdAsset.amt} > \mathsf{Req.in.amt}$. 
\fi
It leads to at least one of the following contradictions:
\vspace{-0.2cm}
\setlist{nolistsep}
\begin{itemize}[noitemsep,leftmargin=*]
    \item $\mathcal{A}$ does not have the correct witness (a valid asset record) but generates a proof, which breaks the soundness of underlying $\mathsf{ZKAoK}$; 
    \item[$\bullet$] $\mathcal{A}$ opens the asset kind and amount in commitment $\mathsf{Com}(usk, aid_i, i, v_i, px_i; r)$ to values $i'\neq i$ and $v_i'\neq v_i$ such that $i'=\mathit{ts_t(kind)}$ and $v_i' > \mathit{ts_t(amt)}$ and generates the proof. It means one commitment produces two different openings which contradicts the binding property of the commitment scheme. 
\end{itemize}
\vspace{-0.2cm}

\noindent(3) 
Suppose that Pr[$\mathcal{A}$ wins and violates condition 3] is non-negligible. 
In this exchange transaction, \adv\ uses an asset record and a price tokens as the exchange input w.r.t. a commitments $\mathsf{Com}(usk, aid_i, i, v_i, px_i; r_2)$ and $\mathsf{Com}(au, i, v_i, \overline{px}_i; r_6)$, $\mathsf{Com}(au, i, v_i, \overline{px}_j; r_7)$ and produces the exchange results of commitments
$\mathsf{Com}(usk, aid_i^*, i, v_i^*, px_i; r_4)$ and $\mathsf{Com}(usk, aid_j, j, v_j, \overline{px}_j; r_5)$
where $\overline{px}_i\times(v_i-v_i^*)\neq\overline{px}_j\times v_j$,
%it leads to the contradiction that  
%$\mathsf{ReqExc.in.amt}\times\mathsf{RdAsset.price}\neq \mathsf{ReqExc.out.amt}\times\mathsf{RdAsset'.price}$ 
but it generates a valid proof that they are equal. %$\mathsf{ReqExc.in.amt}\times\mathsf{RdAsset.price}= \mathsf{ReqExc.out.amt}\times\mathsf{RdAsset'.price}$. 
It leads to at least one of the following contradictions:
\vspace{-0.2cm}
\setlist{nolistsep}
\begin{itemize}[noitemsep,leftmargin=*]
    \item $\mathcal{A}$ uses the incorrect witness to generate a valid proof, which breaks the soundness of underlying $\mathsf{ZKAoK}$; 
    \item $\mathcal{A}$ opens the commitment to different values and generates the proof. It means one commitment produces two different openings which contradicts the binding property of the commitment scheme. 
\end{itemize}
\vspace{-0.6cm}
\end{proof}



\iffalse
\noindent\textit{Proof sketch.} 
In each exchange and withdraw transaction, the user shows an unused identifier and proves that he owns a valid token (signature on some message) containing that identifier and enough asset amount.
He also commits on some messages as the transaction result and proves their well-formness to request new blind signatures. 
If $\mathcal{A}$ wins in the overdraft prevention experiment, the soundness of underlying $\mathsf{ZKAoK}$, or the binding property of the commitment, or unforgeability of blind signature is broken.


\fi


\iffalse
\begin{theorem}[Overdraft prevention]
    If $\Pi_{\mathrm{ouac}}$ is sound, then $\Pi_{\mathrm{\name}}$ has overdraft prevention property.
\end{theorem}
\fi

\iffalse
\begin{proof}
In the overdraft prevention experiment, the adversary $\mathcal{A}$ wins if it is infeasible to extract a consistent list of transaction history and withdraws more asset than it has deposited.
It means one of the following events happens:

%\noindent$\bullet$ 
For $t=1$ to $N$, check each $h_t=(u, \mathsf{Req}, \{Rd\}, \{Rd\}')$, %\textbf{returns 1} if any of the following conditions is true:
\begin{itemize}
    \item $\{Rd\}\not\subseteq \{Rd\}_{u}$ and $\{Rd\}_{u}\neq\emptyset$
    \item The $\mathsf{RdAsset}$ in $\{Rd\}$ is not enough to satisfy the request $\mathsf{Req}$: \\
    $\mathsf{Req}.\mathsf{in}.\mathsf{kind} \neq \mathsf{RdAsset}.\mathsf{kind}$ or
    $\mathsf{Req}.\mathsf{in}.\mathsf{amt} > \mathsf{RdAsset}.\mathsf{amt}$ %for the asset record $\mathsf{Rd}_{\mathrm{asset}}\in\{Rd\}$.
    \item $\mathsf{Req}$ is an exchange request $\mathsf{ReqExc}$ and it is unfair:\\ $\mathsf{ReqExc}.\mathsf{in}.\mathsf{amt}\times\mathsf{RdAsset}.\mathsf{price}\neq\mathsf{ReqExc}.\mathsf{out}.\mathsf{amt}\times\mathsf{RdAsset'}.\mathsf{price}$ for $\mathsf{RdAsset}\in\{\mathsf{Rd}\}$ and $\mathsf{RdAsset'}\in\{\mathsf{Rd}\}'$.
    \item The $\mathsf{RdAsset}$ in $\{Rd\}$ has been used before.
\end{itemize}

$\mathcal{A}$ violates condition 1: Suppose that Pr[$\mathcal{A}$ wins and violates condition 1] is non-negligible. In this case, it leads to the contradiction that $\mathcal{A}$ does not know the $usk$ of $u$ but generates a valid proof, which breaks the soundness of underlying $\mathsf{ZKAoK}$.

$\mathcal{A}$ violates condition 2: Suppose that Pr[$\mathcal{A}$ wins and violates condition 2] is non-negligible. 
In this case, it leads to the contradiction that  $\mathsf{Req.in.kind}\neq \mathsf{RdAsset.kind}$ or $\mathsf{Req.in.amt}> \mathsf{RdAsset.amt}$ but the proof is valid, which breaks the binding property of the commitment scheme or the soundness of underlying $\mathsf{ZKAoK}$.

$\mathcal{A}$ violates condition 3: Suppose that Pr[$\mathcal{A}$ wins and violates condition 3] is non-negligible. 
In this case, it leads to the contradiction that 
$\mathsf{ReqExc.in.amt}\times\mathsf{RdAsset.price}\neq \mathsf{ReqExc.out.amt}\times\mathsf{RdAsset'.price}$
but the proof is valid, which breaks the binding property of the commitment scheme or the soundness of underlying $\mathsf{ZKAoK}$.

$\mathcal{A}$ violates condition 4: Suppose that Pr[$\mathcal{A}$ wins and violates condition 4] is non-negligible. 
In this case, there are two valid transactions using the same asset record.
Since the used identifier would be detected, the revealed identifiers must be different $aid\neq aid'$.
It means one commitment produces two different openings.
This contradicts the binding property of the commitment scheme.


\iffalse
Here we construct $\mathcal{B}$ as an attacker of the soundness of the $ \Pi_{\mathrm{ouac}} $. 
It responds $ \mathcal{A}  $'s queries by querying $ \textbf{Issue}_{\mathrm{ouac}}  $ and $ \textbf{Update}_{\mathrm{ouac}}  $ oracles in the soundness experiment of $\Pi_{\mathrm{ouac}}$ and it owns the secret key of the blind signature.  
Thus $ \mathcal{B}  $  simulates $ \mathcal{A}  $'s view perfectly. % except with some error events. 
It remains to prove that if $ \mathcal{A}  $ wins, then $ \mathcal{B}  $ can update a credential not obtained by the issuer.   

Errors: (1) there are two same identifiers in two transactions of exchange or withdraw;
(2) the exchange is unfair according to the public prices. \tian{no}
These errors happen with negligible probability since the platform can check the $req_{upd}$ and $req_{ded}$ with the $\mathsf{ID}$ set and the public prices and reject the errors.

If no errors happen and $\mathcal{A}$ wins, it means the extracted transaction history $\mathcal{H}$ is not consistent and at least one of the following things happens:

(1) for one $h_t=(usk,\{Rd\}, req, Rd)$, $\{Rd\}\not\subseteq\{Rd\}_{usk}$, it means the records used in this transaction do not belong to that user.
Thus, there must be an instance in the $\mathcal{L}$ where the attribute vector w.r.t $(usk, \{Rd\})$ is not the result of any earlier issue or update operation $\mathbf{A}_s\notin E_{s-1}$.
So $\mathcal{B}$ wins.

(2) for one $h_t=(usk,\{Rd\}, req, Rd)$, if the records used in this transaction do not satisfy the request, there must be an instance in the $\mathcal{L}$ where the attribute vector w.r.t $(usk, \{Rd\})$ cannot fulfill the update function $\psi$, i.e. $\psi(\mathbf{A}_s,\alpha_{s})=\bot$.
So $\mathcal{B}$ wins.


\fi


\iffalse
If $ \mathcal{A}  $ withdraws more asset than it has deposited, then 
(1) it can update a credential not issued by the platform in a withdraw or exchange operation or 
(2) it can update a credential more than once.
For the second case, due to the identifiers $ id, dsid $ shown in the exchange, withdraw operations, this kind of behavior would be detected at once by the platform with the $ \mathsf{ID}  $ set.
Therefore, $ \mathcal{A}  $ can only win in the first case which can be utilized by $ \mathcal{B}  $ to break the soundness of $ \Pi_{\mathrm{uacs}} $. 
\fi


\end{proof}
\fi


\begin{theorem}[Compliance]\label{thmcomp}
    If the underlying $\mathsf{ZKAoK}$ is secure with proof of knowledge, the commitment is binding, and $\Pi_{bs}$ is unforgeable, then $\Pi_{\mathsf{\name}}$ has compliance property w.r.t. MR-LCR-platform-compliance and tax-report-client-compliance.
    %If $\Pi_{\mathrm{ouac}}$ is sound and the blind signature $\Pi_{\mathrm{bs}}$ is unforgeable, then $\Pi_{\mathrm{\name}}$ has compliance property.
\end{theorem}
\vspace{-0.3cm}	
%\yanan{Which compliance does Theorem 3 prove? Probably specify it satisfy the tax-report-client-compliance property.}
\begin{proof}
{%We prove that $\Pi_{\mathsf{\name}}$ is compliant by showing it has tax-report-client-compliance and MR-LCR-compliance properties.
Firstly, since the net inflow of assets and monthly outflow are publicly and immutably recorded on the blockchain. For fiat money transactions via bank transfer, we assume banks do not collude with the platform and provide correct transfer information to the authority.
So, the authority can check the platform's proofs of minimal reserve and appropriate liquidity using available data.
Thus, it satisfies the MR-LCR-platform-compliance of minimal reserve and liquidity.
Then we only need to prove the tax-report-client-compliance.}

In this experiment, $\mathcal{A}$ wins if it outputs $\mathit{doc}$ with the $upk$ and can be verified under the public key $pk$ and auxiliary information $au$, but the accumulated cost or gain in $\mathit{doc}$ is inconsistent with that of this user's transaction history. 
%, i.e., $cp\neq cp^*$ where $cp\in \mathit{doc}$, $cp^*$ is computed from $\{cp\}_{u^*}$ denoted its real compliance information.

%\noindent$\bullet$ 
For $t=1$ to $N$, obtain $h_t=(u, \{Rd\}, \{Rd\}', \mathit{ts_t},\mathit{pub_t})$, 
$\mathcal{A}$ wins if one of the following events happens:\\
\noindent(1) It is not a join transaction and the user identity has not registered: $u\notin \mathsf{RU}$;\\
(2) The user identities in all records are not the same;\\
(3) The buying price was wrong for the new asset record in each kind of transaction:\\ 
${\textit{Deposit}}$:
$\mathit{Rd_{ast}}(\mathit{acp})\neq\mathit{pub_t(Rd_{ast}(kind))}$;\\
${\textit{Exchange}}$: 
$\mathit{Rd'_{ast_i}}(\mathit{acp})\neq\mathit{Rd_{ast_i}}(\mathit{acp})$ or $\mathit{Rd'_{ast_j}}(\mathit{acp})\neq\mathit{pub_{t}}(j)$;\\
${\textit{Withdraw}}$: 
$\mathit{Rd'_{ast_i}}(\mathit{acp})\neq\mathit{Rd_{ast_i}}(\mathit{acp})$; \\
(4) $\mathit{doc}$ was obtained by interacting with $\mathcal{O}_{\mathsf{Sign}}$ oracle and the inconsistency happens due to that the compliance information was updated incorrectly in some exchange or withdraw transaction;\\    
(5) $\mathit{doc}$ was not obtained by querying oracle and the compliance information was recorded correctly for each previous transaction.

\iffalse
\begin{enumerate}
    \item It is not a join transaction and the user identity has not registered: $u\notin \mathsf{RU}$;
    \item The user identities in all records are not the same;
    \item The buying price was wrong for the new asset record in each kind of transaction:\\ 
${\textit{deposit}}$:
$\mathit{Rd_{ast}}(\mathit{acp})\neq\mathit{pub_t(Rd_{ast}(kind))}$\\
${\textit{exchange}}$: 
$\mathit{Rd'_{ast_i}}(\mathit{acp})\neq\mathit{Rd_{ast_i}}(\mathit{acp})$ or $\mathit{Rd'_{ast_j}}(\mathit{acp})\neq\mathit{pub_{t}}(j)$\\
${\textit{withdraw}}$: 
$\mathit{Rd'_{ast_i}}(\mathit{acp})\neq\mathit{Rd_{ast_i}}(\mathit{acp})$ 
    \item $\mathit{doc}$ was obtained by interacting with $\mathcal{O}_{\mathsf{Sign}}$ oracle and the inconsistency happens due to that the compliance information was updated incorrectly in some exchange or withdraw transaction;    
    \item $\mathit{doc}$ was not obtained by querying oracle and the compliance information was recorded correctly for each previous transaction.

\end{enumerate} 
\fi


We reduce the security of our scheme to the security of the underlying cryptographic building blocks. 
This includes standard primitives like commitment, blind signature, and non-interactive $\mathsf{ZKAoK}$.
We elaborate it case by case. \\
\noindent(1) Suppose that Pr[$\mathcal{A}$ wins and violates condition 1] is non-negligible. 
%Recall that a transaction is valid if and only if it convinces that the user has some valid records from the platform.
In this case, $u$ has not registered but generates a valid transaction which leads to at least one of the following contradictions:
\vspace{-0.2cm}
\setlist{nolistsep}
\begin{itemize}[noitemsep,leftmargin=*]
    \item \adv\ forges a registration record in which the $\sigma_{\textit{reg}}$ should be issued by the platform via a blind signature scheme, so \adv\ breaks the unforgeability of the blind signature;
    \item[$\bullet$] \adv\ does not have the $\sigma_{\textit{reg}}$ but generates a valid proof in the deposit, exchange or withdraw protocol, so it breaks the soundness of the underlying $\mathsf{ZKAoK}$.
\end{itemize} 
\vspace{-0.2cm}
\noindent(2) Suppose that Pr[$\mathcal{A}$ wins and violates condition 2] is non-negligible. 
%Recall that a transaction is valid if and only if it convinces that the user has some valid records from the platform.
In this case, a valid transaction is generated but the records belong to different users. 
However, the user needs to prove that all records belong to himself by proving they contain the same $usk$ which is a contradiction.
So it breaks the soundness of the underlying $\mathsf{ZKAoK}$.

\vspace{-0.2cm}
%$\mathcal{A}$ violates condition 1: 
\noindent(3) Suppose that Pr[$\mathcal{A}$ wins and violates condition 3] is non-negligible. 
In this case, \adv\ generates a commitment for its new asset containing its secret key $\textit{usk}$, asset identifier \textit{aid}, kind \textit{i}, amount $\textit{k}_i$ and price $\textit{px}_i$. 
Here $\textit{px}_i$ is different from the real price w.r.t the output of $\mathcal{O}_{\mathsf{Public}}$.
It leads to at least one of the following contradictions:
\vspace{-0.2cm}
\setlist{nolistsep}
\begin{itemize}[noitemsep,leftmargin=*]
    \item $\mathcal{A}$ uses the incorrect witness to generate a valid proof, which breaks the soundness of underlying $\mathsf{ZKAoK}$; 
    \item[$\bullet$] $\mathcal{A}$ opens the commitment to different values and generates the proof. It means one commitment produces two different openings which contradicts the binding property of the commitment scheme. 
\end{itemize}

\iffalse
it leads to the contradiction that 
the buying price is incorrect  %$\mathsf{Req.in.kind}\neq \mathsf{RdAsset.kind}$ or $\mathsf{Req.in.amt}> \mathsf{RdAsset.amt}$ 
but the proof is valid, which breaks the binding property of the commitment scheme or the soundness of underlying $\mathsf{ZKAoK}$.
\fi


\vspace{-0.2cm}
%$\mathcal{A}$ violates condition 2: 
\noindent(4) Suppose that Pr[$\mathcal{A}$ wins and violates condition 4] is non-negligible. 
In this case, for at least one exchange or withdraw transaction
%it leads to the contradiction that 
the new compliance information $\textit{cp}_1^*, \textit{cp}_2^*$ was incorrect but the proof is valid.
It leads to at least one of the following contradictions:
\vspace{-0.2cm}
\setlist{nolistsep}
\begin{itemize}[noitemsep,leftmargin=*]
    \item[$\bullet$] When computing $\textit{cp}_1^*, \textit{cp}_2^*$, $\mathcal{A}$ uses some incorrect selling prices different from the output of $\mathcal{O}_{\mathsf{Public}}$.
    Its success implies that it forges a price token which breaks the unforgeability of the blind signature, or breaks the soundness of underlying $\mathsf{ZKAoK}$, or breaks the binding property of the commitment scheme.
    \item[$\bullet$] When proving the correctness of $\textit{cp}_1^*, \textit{cp}_2^*$, $\mathcal{A}$ just uses the incorrect witness to generate a valid proof, which breaks the soundness of underlying $\mathsf{ZKAoK}$; 
    \item[$\bullet$] $\mathcal{A}$ opens the commitment to different compliance information values and generates the proof. It means one commitment produces two different openings which contradicts the binding property of the commitment scheme.
\end{itemize}

\vspace{-0.2cm}
\noindent(5) %$\mathcal{A}$ violates condition 3: 
Suppose that Pr[$\mathcal{A}$ wins and violates condition 5] is non-negligible. 
In this case, $\mathcal{A}$ works honestly for each transaction but sends a forged $\mathit{doc}$ to the authority with incorrect $\textit{cp}_1, \textit{cp}_2$. 
It breaks the unforgeability of the blind signature.
\end{proof}


\iffalse
\noindent\textit{Proof sketch.} 
In the compliance experiment, the adversary $\mathcal{A}$ wins if it outputs a compliance document $\mathit{doc}$ with the $upk$ and can be verified under the public key $pk$ and auxiliary information $au$, but its compliance information is inconsistent with that of the user's transaction history.
%It implies that at least one of $Doc_1, Doc_2$ is false and contains the incorrect compliance information. 
%for this user and its transaction history.
%Without loss of generality, we assume $Doc_1$ is the false one.
If it was generated from the blind signature protocol, $\mathcal{A}$ breaks the binding property of commitment or the soundness of the underlying $\mathsf{ZKAoK}$.
If not, then $\mathcal{A}$ breaks the unforgeability of the blind signature.
\fi


